Quark correlation functions at three-loop order and extraction of splitting functions

We present the first complete next-to-next-to-next-to-leading-order calculation of the matching coefficients that link unpolarized flavor non-singlet parton distribution functions with lattice QCD computable correlation functions. By using this high-order result, we notice a reduction in theoretical uncertainties compared to relying solely on previously known lower-order matching coefficients. Furthermore, based on this result we have extracted the three-loop unpolarized flavor non-singlet splitting function, which is in agreement with the state-of-the-art result. Due to the simplicity of our method, it has the potential to advance the calculation of splitting functions to the desired four-loop order.

==> attachedfiles/A1 <==
{(-2.5`50.*I)*CF - (1.5`50.*I)*CF*L, 
 -0.8333333333333333333333333333333333333333333333333333333333333333333333333\
3333`50.*CF + 2.8333333333333333333333333333333333333333333333333333333333333\
3333333333333333`50.*CF*L, (-1.625`50.*I)*CF + 
  (1.791666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CF*L, 0.87129629629629629629629629629629629629629629629629629629\
62962962962962962963`50.*CF - 0.686111111111111111111111111111111111111111111\
11111111111111111111111111111111`50.*CF*L, 
 (0.2886574074074074074074074074074074074074074074074074074074074074074074074\
0741`50.*I)*CF - (0.188888888888888888888888888888888888888888888888888888888\
88888888888888888889`50.*I)*CF*L, 
 -0.0702552910052910052910052910052910052910052910052910052910052910052910052\
9101`50.*CF + 0.0406349206349206349206349206349206349206349206349206349206349\
2063492063492063`50.*CF*L, 
 (-0.013589175485008818342151675485008818342151675485008818342151675485008818\
34215`50.*I)*CF + (0.00717757936507936507936507936507936507936507936507936507\
936507936507936507936`50.*I)*CF*L, 
 0.00218646969369758485404743908145268689486376561206493179282294928553431954\
793`50.*CF - 0.00107575900730662635424540186444948349710254472159234063995968\
757873519778282`50.*CF*L, 
 (0.0003015697267663679228305078645214699636468343951337148616060180686031026\
1671`50.*I)*CF - (0.000140050233056185437137818090199042579994960947341899722\
85210380448475686571`50.*I)*CF*L, 
 -0.0000364270028913857124153588418306651278852505021985159719265707339949382\
4454`50.*CF + 0.0000161178505259193089880920568751256581944412632243320074007\
904695735383566`50.*CF*L, 
 (
    -3.91587166019354018010270634777227537788552317820815343281119715150117435`\
50.*^-6*I)*CF + 
  (
    1.66230680450257169833889410608987328564048140767717487294206870926447646`\
50.*^-6*I)*CF*L, 
 3.7935283217412687402907753878465599538070971292765264919987435460311683`50.\
*^-7*CF - 
  1.5532335006841981348955855930362904869879376853883828390802897777404752`50.\
*^-7*CF*L, 
 (
    3.345296610241248479838137379213871709315623710957057709355880605470806`50.\
*^-8*I)*CF - 
  (
    1.326670517337103837023670276836863336783170036336622836542669795836382`50.\
*^-8*I)*CF*L, 
 -2.70761941883414155703203809027731627471003027154400081589784596263419`50.*^\
-9*CF + 
  1.04357492243525962893015593401627120994173694559728279095331795717829`50.*^\
-9*CF*L, 
 (
    -2.0253530906459488102873461062534055321851824452041855974063621074983`50.*^\
-10*I)*CF + 
  (
    7.607732645935734734061627626616429700470879750154267524022989016549`50.*^\
-11*I)*CF*L, 
 1.408380699624965684267833115875431379841797327520045410740567452206`50.*^-11\
*CF - 
  5.1677861715721502647582757603110387235346897187978263419749692235`50.*^-12*
   CF*L, 
 (9.1502984074083024224846209785135880218817733107482671036135844482`50.*^-13*
    I)*CF - 
  (3.286290742406611658568678966408981319201644921503787954624526843`50.*^-13*
    I)*CF*L, 
 -5.578919830634866786410242803273570698292507041582003031785952916`50.*^-14*
   CF + 
  1.964447328708669008902678661661125704974467829512247749538595109`50.*^-14*
   CF*L, 
 (-3.20431723105732718681553776144960529794287846918663925304582026`50.*^-15*
    I)*CF + 
  (1.10784656774943491065604986329235257693286372070707778975770855`50.*^-15*
    I)*CF*L, 
 1.7396820340296404257319577306766204131346806835528693529433252`50.*^-16*
   CF - 
  5.91318379263235747179330485679556274324786157757435542613758`50.*^-17*CF*
   L, (8.95511031027227894182678047432216189396043111131275441286912`50.*^-18*
    I)*CF - (2.99582674635688576409121506611921725701793886124816598507400851\
2366569318501639`50.*^-18*I)*CF*L, 
 -4.3824870067430304703992462181649627359222033431377123733735876257735474282\
2945`50.*^-19*CF + 1.44441458743266227884586417791255146681253090383997005016\
906713255571624078334`50.*^-19*CF*L, 
 (-2.044020397711990766952588282990150660518326316871204540526495543780034248\
8778`50.*^-20*I)*CF + 
  (6.643030776976632777176361657624308474866120481843429646040941004926394579\
94`50.*^-21*I)*CF*L, 
 9.10608173440008426908534663110763829116942950048656839645747109074046672687`\
50.*^-22*CF - 
  2.9205650627185834394350114637867593354222451568050307439396394302414591918\
3`50.*^-22*CF*L, 
 (
    3.8827583797663424097072355890078178064145449165407771703311996959083316825`\
50.*^-23*I)*CF - 
  (1.229816673337038919869145107545774497141678479619141239249924201951653273\
4`50.*^-23*I)*CF*L, 
 -1.587513574586805970187347972345711885831400408726669457997264553235278216`\
50.*^-24*CF + 
  4.96893208813156199304726670683474891222234992282357287085067344876219438`5\
0.*^-25*CF*L, 
 (
    -6.2345162866808218020781185430817871616878689108131166006069698772764251`\
50.*^-26*I)*CF + 
  (
    1.9295203358492462422220321058534459631268410965933417023497056928194755`\
50.*^-26*I)*CF*L, 
 2.355473789810139655933462712931490486478119709713503608487726667976872`50.*^\
-27*CF - 
  7.21205317650072689766931943966698238581847334407281320702133103764199`50.*^\
-28*CF*L, 
 (
    8.573823195215497218015135887799197989332477105925130764667990439852`50.*^\
-29*I)*CF - 
  (
    2.5983801315776465823567591356172678153890796746379054141363705829531`50.*^\
-29*I)*CF*L, 
 -3.01076076522339763828057019722259730201296275522112552328519766067`50.*^-30\
*CF + 
  9.03541511146762036362102993089561749684181312592069264766293064692`50.*^-31\
*CF*L, 
 (
    -1.02123860799966024420459331194025706373349780352505447156199894474`50.*^\
-31*I)*CF + 
  (
    3.0361528739253095118235600951516702646948860104177895989803866181`50.*^-32\
*I)*CF*L, 
 3.349920012649549134424666581342562325563458259828232584752308704`50.*^-33*
   CF - 
  9.87012364282790472902645815629014523076784954160306349599930708`50.*^-34*
   CF*L, 
 (1.06382868832648859862316442823002025910715344245373057862956819`50.*^-34*
    I)*CF - 
  (3.1074674793598611356434871333006000956334030670249740771950072`50.*^-35*
    I)*CF*L, 
 -3.274031178584635672211011506839466854499739118900297221633766`50.*^-36*
   CF + 
  9.48436992206126687156726905688876903748716312706866492569405`50.*^-37*CF*
   L, (-9.7742702818272990518031890411232942420630991519679621265385794563674\
9995569195`50.*^-38*I)*CF + (2.8088915642897910185415334237036093929469468360\
3931332061535129265600454237407`50.*^-38*I)*CF*L, 
 2.83314020615151527328754818420385234585600095130790333867200846295883832302\
53`50.*^-39*CF - 
  8.0792103916404450839743014252092659869388383326709183502949059830989050864\
24`50.*^-40*CF*L, 
 (7.9800039924763377475599374284024632341408862552013874689788715443751060769\
6`50.*^-41*I)*CF - 
  (2.258766651165124445300988667743889121241817643263135593083657983128654367\
59`50.*^-41*I)*CF*L, 
 -2.1859381349438839037094487502702878946865522281949474982593557674480954986`\
50.*^-42*CF + 
  6.14304049681604205036089027472949511682350090561294378204910624051091537`5\
0.*^-43*CF*L, 
 (
    -5.82776074078830953226442751373921391299896185055820749627178088043666104`\
50.*^-44*I)*CF + 
  (
    1.62640099455640198628956693712404276906400855278220379412774069249924792`\
50.*^-44*I)*CF*L, 
 1.5132354789257486097318796338340898885128972202865219592759019180362608`50.\
*^-45*CF - 
  4.194786638982712001856646480129235506392528486097774824575228501242157`50.\
*^-46*CF*L, 
 (
    3.82955220398927018905662310949587133488518883594962230755468349813891`50.*^\
-47*I)*CF - 
  (
    1.05467884010332845520539556519689578539250688825582600499594326706579`50.\
*^-47*I)*CF*L, 
 -9.451635270962908813853342184819006774301087750006505708267787325369`50.*^-\
49*CF + 
  2.586630302548104682514934517543020112344928080595214882901943793941`50.*^-\
49*CF*L, 
 (
    -2.2764094706823951532501462099300328978639912175205736813718025692`50.*^-50\
*I)*CF + 
  (6.191765708387860920532345697902611820876588624547792523310142745`50.*^-51*
    I)*CF*L, 
 5.353433994652650359660700699079427240624768333690562299828635928`50.*^-52*
   CF - 
  1.447473087550733194780413729009228524071746734645294911077287214`50.*^-52*
   CF*L, 
 (1.22997253809807564623264540598795344628356945907313862892524122`50.*^-53*
    I)*CF - 
  (3.3064391248342208755545297882434683539399597513902804615768649`50.*^-54*
    I)*CF*L, 
 -2.762297378349711863006008548452605632806294618667249551803002`50.*^-55*
   CF + 
  7.38400599267844913085242433977968590065972210211753114067715`50.*^-56*CF*
   L, (-6.0670603179046197218533475390884558865126819366881609188180721651917\
26698236509`50.*^-57*I)*CF + (1.612955453469353934149082915997936390287143718\
97934652469491377315669178272897`50.*^-57*I)*CF*L, 
 1.30385772095425098196580518093070099359019890298776082979430000556983522481\
38`50.*^-58*CF - 3.4479380615431419794372846662133957588742254226151098950699\
713441120812030514`50.*^-59*CF*L, 
 (2.7430151175070318393350612268513177892579673584461780204483962997591640759\
99`50.*^-60*I)*CF - 
  (7.216097488837113342656605326693824785084767036027323236070836193862233888\
15`50.*^-61*I)*CF*L, 
 -5.6515286074060003202425685697048571550805047111740290408732987203782616192`\
50.*^-62*CF + 
  1.4792514871508977971548726971153235525780999563475253860663256889762521713`\
50.*^-62*CF*L, 
 (
    -1.140851353127059391322913254298949892560501105150412490027139877468014389`\
50.*^-63*I)*CF + 
  (
    2.97140185278243336826502333003594693273268407776374439611056973690600679`\
50.*^-64*I)*CF*L, 
 2.257333857898212226952164481259872359411863701568092740005973824043828`50.*^\
-65*CF - 
  5.851083314838198833770383684301420953896746182872730929761994726013448`50.\
*^-66*CF*L, 
 (
    4.37962879929201592244926344980534497798898661862122982792140096800769`50.*^\
-67*I)*CF - 
  (
    1.12988848621072405459949948434154219800183949099186369307188936258651`50.\
*^-67*I)*CF*L, 
 -8.3352404886878894883300924954640771262361429485891671620767670057`50.*^-69*
   CF + 
  2.140531911425947651351440089455100561135336237495594873097297631174`50.*^-\
69*CF*L, 
 (
    -1.55667015415451675766059853575814081388821468784270055184800863722`50.*^\
-70*I)*CF + 
  (
    3.9797056858895704319905297988319391801983560243421074621180308845`50.*^-71\
*I)*CF*L, 
 2.853810356959868631410810938257693478280735951450770882450066888`50.*^-72*
   CF - 
  7.2639669435998830954924778020891664170737790713196427750384727`50.*^-73*CF*
   L, 
 (5.1374843445687554431419622744190360054309317976805222941628097`50.*^-74*I)*
   CF - 
  (1.3020734650272962451660215074172615394022583428154571144149435`50.*^-74*
    I)*CF*L, -9.0847792321572363792172102431236221988504033661951749031556719\
50280820319764752`50.*^-76*CF + 2.2928505482878242647739703084774145499143624\
66626818909205443946467491176152424`50.*^-76*CF*L, 
 (-1.578531645161163796637283441286772842960247783788068200833891998253551525\
28603`50.*^-77*I)*CF + (3.967616110490708360696616533309891870986466308843040\
8740791745594676443567483`50.*^-78*I)*CF*L, 
 2.69587100292461657803728404409931820618858329508399796927543753290074542928\
9`50.*^-79*CF - 
  6.7488153569147185975285234152293088409356657594552882953667492495917893869\
8`50.*^-80*CF*L, 
 (
    4.5266736466720994170495965937522471353480200725072231507905979173119788565`\
50.*^-81*I)*CF - 
  (1.128743882610120233076441096393815861509073782224446964872698881748139767\
2`50.*^-81*I)*CF*L, 
 -7.47509341339697839084752820129331741616771688520001245423971192737413857`5\
0.*^-83*CF + 
  1.85675672565914763347601701597415400866310807630837079888928622924474373`5\
0.*^-83*CF*L, 
 (
    -1.2143125173770727044152811221499037050429772432511391445048574642246677`\
50.*^-84*I)*CF + 
  (
    3.004859175854905831475171132087910424693910844397876140299940198514848`50.\
*^-85*I)*CF*L, 
 1.94104640552682985804106548744267628407332463188054386604188786380748`50.*^\
-86*CF - 
  4.7853836529787541848355777674084971541542040428252217100826819690726`50.*^\
-87*CF*L, 
 (
    3.053827372874203229482306888563931442775357395046158410366325532354`50.*^\
-88*I)*CF - 
  (
    7.5014170285114327208898189444279414219668349841846110928936874623`50.*^-89\
*I)*CF*L, 
 -4.7300331970627037403865480187309566690562854396266342307551340054`50.*^-90*
   CF + 
  1.1577391427848611766178058855368296681663830087564805886616827985`50.*^-90*
   CF*L, 
 (-7.21439172081666507706135646197123893209291947088335683182786717`50.*^-92*
    I)*CF + 
  (1.75963523059564134591688213584908596499176265791371674740922852`50.*^-92*
    I)*CF*L, 
 1.0838085626321792958693998884562390102324399008042021100446064`50.*^-93*
   CF - 
  2.63438738465654500155987477604552878706231619112779033297997`50.*^-94*CF*
   L, (1.60406227521240268903377069319340095629235436869762698468247840136346\
9133400756`50.*^-95*I)*CF - (3.8857890874814766296344449575247794711116251261\
7219569838268272447276270839377`50.*^-96*I)*CF*L, 
 -2.3393823940660159736485001557742520069331732239874059622545533618430378228\
494`50.*^-97*CF + 
  5.6482782772713367418270808754055450600478427581531383759157038072973621770\
61`50.*^-98*CF*L, 
 (
    -3.3626783751190436772084584102169105183237092736459169574810882758110043\
6861`50.*^-99*I)*CF + 
  (8.092489804530802644520740782176345555915491568264785129675790740995399592\
8`50.*^-100*I)*CF*L, 
 4.765008553128784362607025379355873964181823032552494168797366712999784425`5\
0.*^-101*CF - 
  1.143054061449875387726737090751204830541908801291038553514598525752950113`\
50.*^-101*CF*L, 
 (
    6.6576942882803745063694397217921122571758106687687192735700075956640304`50.\
*^-103*I)*CF - 
  (
    1.5920500824530488446945579058622129293552609799864560098794661381323428`\
50.*^-103*I)*CF*L, 
 -9.17383566764129177354387449193758596257632668605294720957411671899619`50.*^\
-105*CF + 
  2.18693778682645063079350922895478125092415714374207837625323434629487`50.*^\
-105*CF*L, 
 (
    -1.2468890136879460245079892589794379899192733384031897749776844144295`50.*^\
-106*I)*CF + 
  (
    2.963384311763552974631624802323585942209902324850325271712457372672`50.*^\
-107*I)*CF*L, 
 1.6719948051420492230511617971850206666244499829124929196713171528`50.*^-108*
   CF - 
  3.9617882148967183897487304630933422867116762120933467001381905029`50.*^-109\
*CF*L, 
 (2.212334167899576605954165252093294509481386522237323320332212604`50.*^-110*
    I)*CF - 
  (5.22665726277535070546214783850952657056335067348709208214844459`50.*^-111*
    I)*CF*L, 
 -2.8890265509851436329285384273441697847903607063293482567792974`50.*^-112*
   CF + 
  6.805530643538997942177133341956522078972146663007892702136228`50.*^-113*CF*
   L, 
 (-3.72401722437483695350089711929643222601407870191115132904354`50.*^-114*I)*
   CF + (8.747398774508312411591207448271957747236746321875661836783377529300\
76551707334`50.*^-115*I)*CF*L, 4.73918429217280813740594927711033790616474271\
73877805987952389716757694034596`50.*^-116*CF - 
  1.1100605925216312043161096688800431531783707934797098306193256342845116716\
401`50.*^-116*CF*L, 
 (5.9552208383279666192179111589722511947398462446464095358380708772178872654\
6`50.*^-118*I)*CF - 
  (1.391026251941408734018952174665011876200614609245186894279827878743812654\
43`50.*^-118*I)*CF*L, 
 -7.390321332685204900478744192703319668584182643340968784021774200559272891`\
50.*^-120*CF + 
  1.721524285468511536693915076798503569819327964760419074214466099759122533`\
50.*^-120*CF*L, 
 (
    -9.0587248080920091790019868230060878226596649001862024186855248005088981`\
50.*^-122*I)*CF + 
  (
    2.104489631479263070439794947639224898598066034807770541668058168383056`50.\
*^-122*I)*CF*L, 
 1.096919054103010635131659915725747413030014598720867055856606563383797`50.*^\
-123*CF - 
  2.54156509759017157253385673268462684718921134443164825509567952677622`50.*^\
-124*CF*L, 
 (
    1.3123502494733414001583922653339682189789938558951353911007872099363`50.*^\
-125*I)*CF - 
  (
    3.032773207107136191446896379360755743827610554431164978902111421559`50.*^\
-126*I)*CF*L, 
 -1.55151139382037167509999360136017360188707349402809280744124301803`50.*^-1\
27*CF + 
  3.576224815176971432274696190758868836239984909654275439258774322`50.*^-128*
   CF*L, 
 (
    -1.812805093773903173289290005989716627718957784651503169726895961`50.*^-129\
*I)*CF + 
  (4.16789096018925853757797968259307765828069805679888678780286062`50.*^-130*
    I)*CF*L, 
 2.0936190853159247984858353226380871860192385617665835362594093`50.*^-131*
   CF - 
  4.80146333728063994939249302417600280047871574335935953086853`50.*^-132*CF*
   L, 
 (2.39030184277272616928508726203833556333883099356614353308259`50.*^-133*I)*
   CF - (5.468325238463206930354152924876128244908734715725413923331197329653\
768370461663`50.*^-134*I)*CF*L, 
 -2.6981937502333581208701300465107701666811889394918594247582870553014873082\
8322`50.*^-135*CF + 6.1576488465670950812505186756041892527517987072968248826\
548074317765986654615`50.*^-136*CF*L, 
 (-3.011718200057796951103519842033700562635752319547891769012782821903586062\
451`50.*^-137*I)*CF + 
  (6.856626721014471542701401560444158091076321930058305365575736506172653044\
3`50.*^-138*I)*CF*L, 
 3.32453280206079068889137350105993753505010929405771640396671444731217108`50.\
*^-139*CF - 
  7.550835758739478149211702641974223985664439328464180078484349582652550937`\
50.*^-140*CF*L, 
 (
    3.62973630621530203658339144139693666187877173136401010388703372108693895`\
50.*^-141*I)*CF - 
  (
    8.2247216560031406107113575727300861623046955971845521815920312217690695`\
50.*^-142*I)*CF*L, 
 -3.920122274948592200812192234191159787846646250630142537245677880309231`50.\
*^-143*CF + 
  8.86218187703886477480596454079898201044508814601661541416844092707671`50.*^\
-144*CF*L, 
 (
    -4.1884664287351484956128992243874581405368311182392879205078313864858`50.*^\
-145*I)*CF + 
  (
    9.447216330733719254520544475755893968742857086705217244446607661133`50.*^\
-146*I)*CF*L, 
 4.42783134822517394792123660120380561359522166504293900257553930603`50.*^-147\
*CF - 
  9.9646082695274233140843006941452444908212516271357864498958976096`50.*^-14\
8*CF*L, 
 (4.631870193025195770400343048437192181848057227496863317483235955`50.*^-149*
    I)*CF - 
  (
    1.040059407637848843779079583045486491189776319516124245924192036`50.*^-149\
*I)*CF*L, 
 -4.7951105229457298976803718846701809919007626331855816712953891`50.*^-151*
   CF + 
  1.0743480047415260212836397316094545920260372028817378174405389`50.*^-151*
   CF*L, (-4.9132002706562770938893043166157838092749178195235740078490672368\
37706934532442`50.*^-153*I)*CF + (1.09841671347786689953720828568108582780355\
5331492327946122428651218569495620667`50.*^-153*I)*CF*L, 
 4.98310034905927789957973942316655338046791493073900863478958167231315503056\
6`50.*^-155*CF - 1.1116550666955660589848459466516002291485288189877354187352\
001893758847195826`50.*^-155*CF*L, 
 (5.0032120680425587122808327027707867974450529986134878493309464680197881505\
3`50.*^-157*I)*CF - 
  (1.113777077266167473871934931410648039809767360273589608740857511868486543\
05`50.*^-157*I)*CF*L}


==> attachedfiles/A2 <==
{(-8.467013888888888888888888888888888888888888888888888888888888888888888888\
88889`50.*I)*CA*CF - (1.16145833333333333333333333333333333333333333333333333\
333333333333333333333333`50.*I)*CF^2 - (3.3125`50.*I)*CA*CF*L - 
  (1.5625`50.*I)*CF^2*L - (0.6875`50.*I)*CA*CF*L^2 - 
  (0.5625`50.*I)*CF^2*L^2 + (1.6284722222222222222222222222222222222222222222\
2222222222222222222222222222223`50.*I)*CF*nf + (0.625`50.*I)*CF*L*nf + 
  (0.125`50.*I)*CF*L^2*nf + (0.2083333333333333333333333333333333333333333333\
3333333333333333333333333333333`50.*I)*CA*CF*irrational[Pi^2] - 
  (0.111111111111111111111111111111111111111111111111111111111111111111111111\
11111`50.*I)*CF^2*irrational[Pi^2] + 
  (0.083333333333333333333333333333333333333333333333333333333333333333333333\
33333`50.*I)*CA*CF*L*irrational[Pi^2] - 
  (0.333333333333333333333333333333333333333333333333333333333333333333333333\
33333`50.*I)*CF^2*L*irrational[Pi^2] - (1.`50.*I)*CA*CF*irrational[Zeta[3]] + 
  (4.`50.*I)*CF^2*irrational[Zeta[3]], 
 14.5133101851851851851851851851851851851851851851851851851851851851851851851\
8519`50.*CA*CF + 3.8775077160493827160493827160493827160493827160493827160493\
8271604938271604938`50.*CF^2 + 1.99768518518518518518518518518518518518518518\
518518518518518518518518518518519`50.*CA*CF*L - 
  2.0115740740740740740740740740740740740740740740740740740740740740740740740\
7407`50.*CF^2*L + 1.298611111111111111111111111111111111111111111111111111111\
11111111111111111111`50.*CA*CF*L^2 + 2.00694444444444444444444444444444444444\
444444444444444444444444444444444444444`50.*CF^2*L^2 - 
  2.4618055555555555555555555555555555555555555555555555555555555555555555555\
5556`50.*CF*nf - 0.3657407407407407407407407407407407407407407407407407407407\
4074074074074074074`50.*CF*L*nf - 0.23611111111111111111111111111111111111111\
111111111111111111111111111111111111`50.*CF*L^2*nf - 
  0.4861111111111111111111111111111111111111111111111111111111111111111111111\
1111`50.*CA*CF*irrational[Pi^2] - 0.57407407407407407407407407407407407407407\
407407407407407407407407407407407407`50.*CF^2*irrational[Pi^2] - 
  0.0833333333333333333333333333333333333333333333333333333333333333333333333\
3333`50.*CA*CF*L*irrational[Pi^2] + 0.333333333333333333333333333333333333333\
33333333333333333333333333333333333333`50.*CF^2*L*irrational[Pi^2] + 
  1.`50.*CA*CF*irrational[Zeta[3]] - 4.`50.*CF^2*irrational[Zeta[3]], 
 (10.724392361111111111111111111111111111111111111111111111111111111111111111\
11111`50.*I)*CA*CF + (3.51548635223765432098765432098765432098765432098765432\
098765432098765432098765`50.*I)*CF^2 + 
  (0.259259259259259259259259259259259259259259259259259259259259259259259259\
25926`50.*I)*CA*CF*L - (3.362123842592592592592592592592592592592592592592592\
59259259259259259259259259`50.*I)*CF^2*L + 
  (0.821180555555555555555555555555555555555555555555555555555555555555555555\
55556`50.*I)*CA*CF*L^2 + (1.6050347222222222222222222222222222222222222222222\
2222222222222222222222222223`50.*I)*CF^2*L^2 - 
  (1.563440393518518518518518518518518518518518518518518518518518518518518518\
51852`50.*I)*CF*nf - (0.07349537037037037037037037037037037037037037037037037\
037037037037037037037037`50.*I)*CF*L*nf - 
  (0.149305555555555555555555555555555555555555555555555555555555555555555555\
55556`50.*I)*CF*L^2*nf - (0.4201388888888888888888888888888888888888888888888\
8888888888888888888888888889`50.*I)*CA*CF*irrational[Pi^2] - 
  (0.395370370370370370370370370370370370370370370370370370370370370370370370\
37037`50.*I)*CF^2*irrational[Pi^2] - 
  (0.041666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CA*CF*L*irrational[Pi^2] + 
  (0.166666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CF^2*L*irrational[Pi^2] + (0.5`50.*I)*CA*CF*
   irrational[Zeta[3]] - (2.`50.*I)*CF^2*irrational[Zeta[3]], 
 -4.5892845936213991769547325102880658436213991769547325102880658436213991769\
5474`50.*CA*CF - 2.0119216853137860082304526748971193415637860082304526748971\
1934156378600823045`50.*CF^2 + 0.12987654320987654320987654320987654320987654\
320987654320987654320987654320988`50.*CA*CF*L + 1.95634375`50.*CF^2*L - 
  0.3144675925925925925925925925925925925925925925925925925925925925925925925\
9259`50.*CA*CF*L^2 - 0.706122685185185185185185185185185185185185185185185185\
18518518518518518518518`50.*CF^2*L^2 + 0.618660172325102880658436213991769547\
32510288065843621399176954732510288065844`50.*CF*nf - 
  0.0080941358024691358024691358024691358024691358024691358024691358024691358\
0247`50.*CF*L*nf + 0.05717592592592592592592592592592592592592592592592592592\
592592592592592592592`50.*CF*L^2*nf + 0.1900462962962962962962962962962962962\
962962962962962962962962962962962962963`50.*CA*CF*irrational[Pi^2] + 
  0.1596913580246913580246913580246913580246913580246913580246913580246913580\
2469`50.*CF^2*irrational[Pi^2] + 0.013888888888888888888888888888888888888888\
88888888888888888888888888888888889`50.*CA*CF*L*irrational[Pi^2] - 
  0.0555555555555555555555555555555555555555555555555555555555555555555555555\
5556`50.*CF^2*L*irrational[Pi^2] - 0.1666666666666666666666666666666666666666\
6666666666666666666666666666666666667`50.*CA*CF*irrational[Zeta[3]] + 
  0.6666666666666666666666666666666666666666666666666666666666666666666666666\
6667`50.*CF^2*irrational[Zeta[3]], 
 (-1.381301424254115226337448559670781893004115226337448559670781893004115226\
33745`50.*I)*CA*CF - (0.74316756365740740740740740740740740740740740740740740\
740740740740740740740741`50.*I)*CF^2 + 
  (0.080819830246913580246913580246913580246913580246913580246913580246913580\
24691`50.*I)*CA*CF*L + (0.697425540123456790123456790123456790123456790123456\
79012345679012345679012346`50.*I)*CF^2*L - 
  (0.086574074074074074074074074074074074074074074074074074074074074074074074\
07407`50.*I)*CA*CF*L^2 - (0.2140740740740740740740740740740740740740740740740\
7407407407407407407407407407`50.*I)*CF^2*L^2 + 
  (0.176840888631687242798353909465020576131687242798353909465020576131687242\
79836`50.*I)*CF*nf - (0.00940200617283950617283950617283950617283950617283950\
617283950617283950617284`50.*I)*CF*L*nf + 
  (0.015740740740740740740740740740740740740740740740740740740740740740740740\
74074`50.*I)*CF*L^2*nf + (0.0587962962962962962962962962962962962962962962962\
962962962962962962962962963`50.*I)*CA*CF*irrational[Pi^2] + 
  (0.045048500881834215167548500881834215167548500881834215167548500881834215\
16755`50.*I)*CF^2*irrational[Pi^2] + 
  (0.003472222222222222222222222222222222222222222222222222222222222222222222\
22223`50.*I)*CA*CF*L*irrational[Pi^2] - 
  (0.013888888888888888888888888888888888888888888888888888888888888888888888\
88889`50.*I)*CF^2*L*irrational[Pi^2] - 
  (0.041666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CA*CF*irrational[Zeta[3]] + 
  (0.166666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CF^2*irrational[Zeta[3]], 
 0.31915347729314388894887761100913028350670074026083096377880958379824592976\
521`50.*CA*CF + 0.20162871792504794812860896437184095104406085941557272946971\
683609195756911986`50.*CF^2 - 0.024908486079617031997984378936759889140841521\
79390274628369866465104560342656`50.*CA*CF*L - 0.1803180040402404347982579275\
0962818990029874383615880214519670301983227153295`50.*CF^2*L + 
  0.0186243386243386243386243386243386243386243386243386243386243386243386243\
3863`50.*CA*CF*L^2 + 0.049535903250188964474678760393046107331821617535903250\
18896447467876039304611`50.*CF^2*L^2 - 0.039477313708772750722864101548908805\
1446328090319020024235443736577523425596`50.*CF*nf + 
  0.0032314972285210380448475686570924666162761400856638951877047115142353237\
5913`50.*CF*L*nf - 0.00338624338624338624338624338624338624338624338624338624\
338624338624338624338`50.*CF*L^2*nf - 0.0137830687830687830687830687830687830\
6878306878306878306878306878306878306879`50.*CA*CF*irrational[Pi^2] - 
  0.0098810153691106072058453010833963214915595867976820357772738725119677500\
6299`50.*CF^2*irrational[Pi^2] - 0.000694444444444444444444444444444444444444\
44444444444444444444444444444444445`50.*CA*CF*L*irrational[Pi^2] + 
  0.0027777777777777777777777777777777777777777777777777777777777777777777777\
7778`50.*CF^2*L*irrational[Pi^2] + 0.0083333333333333333333333333333333333333\
3333333333333333333333333333333333333`50.*CA*CF*irrational[Zeta[3]] - 
  0.0333333333333333333333333333333333333333333333333333333333333333333333333\
3334`50.*CF^2*irrational[Zeta[3]], 
 (0.0598775668871029590187044835570912668418337352577715389506772726727375253\
4524`50.*I)*CA*CF + (0.042840837639946262647265171290654499811178355612002086\
46488745830069661189411`50.*I)*CF^2 - 
  (0.005485607123829470059628789787519946250104980263710422440581170739900898\
63106`50.*I)*CA*CF*L - (0.036673701526534886441349026383039988482165352913652\
23338012453658712162113522`50.*I)*CF^2*L + 
  (0.003289723875661375661375661375661375661375661375661375661375661375661375\
66137`50.*I)*CA*CF*L^2 + (0.0092731761975623582766439909297052154195011337868\
4807256235827664399092970522`50.*I)*CF^2*L^2 - 
  (0.007221581908421529252500529900378728798985790671353785488328194299471699\
32053`50.*I)*CF*nf + (0.00074667507821029646426471823297220122616948013773410\
598807424204249601074998`50.*I)*CF*L*nf - 
  (0.000598131613756613756613756613756613756613756613756613756613756613756613\
75661`50.*I)*CF*L^2*nf - (0.0026063023589065255731922398589065255731922398589\
0652557319223985890652557319`50.*I)*CA*CF*irrational[Pi^2] - 
  (0.001769006676744771982867220962459057697152935248173343411438649533887629\
12573`50.*I)*CF^2*irrational[Pi^2] - 
  (0.000115740740740740740740740740740740740740740740740740740740740740740740\
74074`50.*I)*CA*CF*L*irrational[Pi^2] + 
  (0.000462962962962962962962962962962962962962962962962962962962962962962962\
96296`50.*I)*CF^2*L*irrational[Pi^2] + 
  (0.001388888888888888888888888888888888888888888888888888888888888888888888\
88889`50.*I)*CA*CF*irrational[Zeta[3]] - 
  (0.005555555555555555555555555555555555555555555555555555555555555555555555\
55555`50.*I)*CF^2*irrational[Zeta[3]], 
 -0.0094474808321851567467485424909429196623204149789151808772120153580439046\
7714`50.*CA*CF - 0.0074873047944108827099115847450208209433094202376624900238\
0800079023289250243`50.*CF^2 + 0.00095975188825959053031363437007175984248294\
653938392915465225870869609846682`50.*CA*CF*L + 
  0.0061569632262991204478954781897828605047647867597717026024504218603727895\
981`50.*CF^2*L - 0.0004930562116822037456958091878726799361719996640631561266\
4819014025363231712`50.*CA*CF*L^2 - 0.001458144376669686099013385483529096529\
85238775110279267497710430439077453438`50.*CF^2*L^2 + 
  0.0011183527215581800647933215010604461387714136197421339814569887316211007\
3571`50.*CF*nf - 0.0001343509972208558124405945015670387300520835416275073619\
4928686740226170813`50.*CF*L*nf + 0.00008964658394221886285378348870412362475\
854539346602838666330729822793314856`50.*CF*L^2*nf + 
  0.0004129562704711514235323759133282942806752330561854371378180901990425799\
9496`50.*CA*CF*irrational[Pi^2] + 0.00026817566630806741665900144106241359957\
661293010247406820851013342824882255`50.*CF^2*irrational[Pi^2] + 
  0.0000165343915343915343915343915343915343915343915343915343915343915343915\
3439`50.*CA*CF*L*irrational[Pi^2] - 0.000066137566137566137566137566137566137\
56613756613756613756613756613756613757`50.*CF^2*L*irrational[Pi^2] - 
  0.0001984126984126984126984126984126984126984126984126984126984126984126984\
127`50.*CA*CF*irrational[Zeta[3]] + 0.000793650793650793650793650793650793650\
79365079365079365079365079365079365079`50.*CF^2*irrational[Zeta[3]], 
 (-0.001286622579995353875290228505823973875980098810206749914084935100984083\
77532`50.*I)*CA*CF - (0.00110968767863007025469240757290413478859574803061237\
135440708978407700571743`50.*I)*CF^2 + 
  (0.000140465266813693192346505523628224560449302197853470214266384586364430\
1538`50.*I)*CA*CF*L + (0.0008808834861696050745634423902909427630780016531495\
2534955174458947749569113`50.*I)*CF^2*L - 
  (0.000064189690150751658688166624674561182497690434198370706307214243722180\
23012`50.*I)*CA*CF*L^2 - (0.0001977098032132459097689634348742436421952672897\
495270889072854303390962499`50.*I)*CF^2*L^2 + 
  (0.000150101716659499743545567930583547647539617049349219701193530113693123\
04737`50.*I)*CF*nf - (0.00002003690363503328040994959614259185939710001186443\
615266996471330056616023`50.*I)*CF*L*nf + 
  (0.000011670852754682119761484840849920214999580078945158310237675317040396\
40547`50.*I)*CF*L^2*nf + (0.0000563443838183421516754850088183421516754850088\
1834215167548500881834215167`50.*I)*CA*CF*irrational[Pi^2] + 
  (0.000035231764685814824388772486530108097253473922660115655832461073075837\
50012`50.*I)*CF^2*irrational[Pi^2] + 
  (
    2.06679894179894179894179894179894179894179894179894179894179894179894179`\
50.*^-6*I)*CA*CF*L*irrational[Pi^2] - 
  (
    8.2671957671957671957671957671957671957671957671957671957671957671957672`\
50.*^-6*I)*CF^2*L*irrational[Pi^2] - 
  (0.000024801587301587301587301587301587301587301587301587301587301587301587\
30159`50.*I)*CA*CF*irrational[Zeta[3]] + 
  (0.000099206349206349206349206349206349206349206349206349206349206349206349\
20635`50.*I)*CF^2*irrational[Zeta[3]], 
 0.00015408085354373169827686190478672360765395961647753179632055090337620090\
714`50.*CA*CF + 0.00014287741418220811429171953328063492516485211983192520643\
488893136412568816`50.*CF^2 - 0.000017741195962371826621847617900359984848101\
08224906242878864026088347915844`50.*CA*CF*L - 0.0001098677429825423244008690\
4406290047739868396725403475902977038085951659786`50.*CF^2*L + 
  7.38734815771301661954219273443259333911891231115217005869563188787174678`5\
0.*^-6*CA*CF*L^2 + 0.00002356770477784359276911404384166777564091596326263481\
565557502554074471281`50.*CF^2*L^2 - 0.00001777255011663597055846400664707972\
612690749739754040260512904078319657142`50.*CF*nf + 
  2.56583285313550216930199675261785403260624100924306303876762812301112919`5\
0.*^-6*CF*L*nf - 
  1.34315421049327574900767140626047151620343860202766728339920579779486305`5\
0.*^-6*CF*L^2*nf - 
  6.7509251915942833050416824667265584373168147418588335695919470169911087`50.\
*^-6*CA*CF*irrational[Pi^2] - 
  4.08704363839775655081650281825376180364715247430024324695399260653720088`5\
0.*^-6*CF^2*irrational[Pi^2] - 
  2.2964432686654908877131099353321575543797766019988242210464432686654909`50.\
*^-7*CA*CF*L*irrational[Pi^2] + 
  9.1857730746619635508524397413286302175191064079952968841857730746619636`50.\
*^-7*CF^2*L*irrational[Pi^2] + 
  2.75573192239858906525573192239858906525573192239858906525573192239858906`5\
0.*^-6*CA*CF*irrational[Zeta[3]] - 0.0000110229276895943562610229276895943562\
6102292768959435626102292768959435626`50.*CF^2*irrational[Zeta[3]], 
 (0.0000164694644620818883974708659465904901742762204793322741128351653370929\
545`50.*I)*CA*CF + (0.0000162553789018515295981088488753021171114795734651274\
3335560098304187768705`50.*I)*CF^2 - 
  (
    1.97514553882662147058440555263152614850495648905547844547312647309847836`\
50.*^-6*I)*CA*CF*L - (0.00001215075178296678011136651589932323567623271774759\
063743775940197062612826`50.*I)*CF^2*L + 
  (
    7.6189061873034536173865979862452525591855397851870515009844815841288505`\
50.*^-7*I)*CA*CF*L^2 + 
  (
    2.50683302123452397928069229137355602307464084722687378115430368879447725`\
50.*^-6*I)*CF^2*L^2 - 
  (
    1.88227317854795305403536189298144654761669532405948927503297687579993838`\
50.*^-6*I)*CF*nf + 
  (
    2.8871708790866233585184240642832609361083826066227556565554840061051075`\
50.*^-7*I)*CF*L*nf - 
  (
    1.3852556704188097486157450884082277380337345063976457274517239243870637`\
50.*^-7*I)*CF*L^2*nf - 
  (
    7.2122855044665744254221620476764509686320385908863275118419151340962041`\
50.*^-7*I)*CA*CF*irrational[Pi^2] - 
  (
    4.2436728459528900318759098035866730624843372374109322835689551474256677`\
50.*^-7*I)*CF^2*irrational[Pi^2] - 
  (
    2.296443268665490887713109935332157554379776601998824221046443268665491`50.\
*^-8*I)*CA*CF*L*irrational[Pi^2] + 
  (
    9.185773074661963550852439741328630217519106407995296884185773074661963`50.\
*^-8*I)*CF^2*L*irrational[Pi^2] + 
  (
    2.7557319223985890652557319223985890652557319223985890652557319223985891`\
50.*^-7*I)*CA*CF*irrational[Zeta[3]] - 
  (
    1.10229276895943562610229276895943562610229276895943562610229276895943563`\
50.*^-6*I)*CF^2*irrational[Zeta[3]], 
 -1.58937680067131056860133906101479637791421052129472441263034634587797779`5\
0.*^-6*CA*CF - 
  1.65739600058194136763901670608104397213202352749086555185930629977605591`5\
0.*^-6*CF^2 + 
  1.9685169687809040327391162240313587781433565777666620083960817799868137`50.\
*^-7*CA*CF*L + 
  1.20741359032486363072386120348383496615077568337996524652884290663663109`5\
0.*^-6*CF^2*L - 
  7.118986878135908118271433968082998065361381058030088012451328147977178`50.\
*^-8*CA*CF*L^2 - 
  2.4075162362877817350126079289065306308177807903564483577917848206375349`50.\
*^-7*CF^2*L^2 + 
  1.8030493369302977255603287315670120176022577028645144152374870726572205`50.\
*^-7*CF*nf - 
  2.902264127283725657400510151841979652883942864711921960055687265893553`50.\
*^-8*CF*L*nf + 
  1.294361250570165112412987994196908739156614737823652365900241481450396`50.\
*^-8*CF*L^2*nf + 
  6.952523804242044849174345192730100003896166581218155158617987969706211`50.\
*^-8*CA*CF*irrational[Pi^2] + 
  3.989186158071910411246204165450668150754304423911676972513486933454937`50.\
*^-8*CF^2*irrational[Pi^2] + 
  2.08767569878680989792100903212014323125434236545347656458767569878681`50.*^\
-9*CA*CF*L*irrational[Pi^2] - 
  8.35070279514723959168403612848057292501736946181390625835070279514724`50.*^\
-9*CF^2*L*irrational[Pi^2] - 
  2.505210838544171877505210838544171877505210838544171877505210838544172`50.\
*^-8*CA*CF*irrational[Zeta[3]] + 
  1.0020843354176687510020843354176687510020843354176687510020843354176687`50.\
*^-7*CF^2*irrational[Zeta[3]], 
 (
    -1.3982151526910284578494897910837475656311184967825424551088906797008814`\
50.*^-7*I)*CA*CF - 
  (
    1.5307454052828229798711735099287911245518127892186607404839497365910566`\
50.*^-7*I)*CF^2 + 
  (
    1.777322944001762691071234991657333481906232519432982607105278696971567`50.\
*^-8*I)*CA*CF*L + 
  (
    1.0894812742010157415405871391869457400944457195029551109354687947756673`\
50.*^-7*I)*CF^2*L - 
  (
    6.08057320446172591969182210216895696025619599987618800082056989758342`50.\
*^-9*I)*CA*CF*L^2 - 
  (
    2.107672497450516018292282076241867897667249474297289041111480941616779`50.\
*^-8*I)*CF^2*L^2 + 
  (
    1.576445467949825867126624706269041471608903885237347143471293734359613`50.\
*^-8*I)*CF*nf - 
  (
    2.63906475292339277484768161764370266110273381786184804519328385357783`50.\
*^-9*I)*CF*L*nf + 
  (
    1.10555876444758653085305856403071944731930836361385236378555816319699`50.\
*^-9*I)*CF*L^2*nf + 
  (
    6.10667522906984956301502972546998088378127112663201696645227443255596`50.\
*^-9*I)*CA*CF*irrational[Pi^2] + 
  (
    3.42539181238214391712833009895438912333217026142851023141191229980451`50.\
*^-9*I)*CF^2*irrational[Pi^2] + 
  (
    1.7397297489890082482675075267667860260452853045445638038230630823224`50.*^\
-10*I)*CA*CF*L*irrational[Pi^2] - 
  (
    6.9589189959560329930700301070671441041811412181782552152922523292893`50.*^\
-10*I)*CF^2*L*irrational[Pi^2] - 
  (
    2.08767569878680989792100903212014323125434236545347656458767569878681`50.\
*^-9*I)*CA*CF*irrational[Zeta[3]] + 
  (
    8.35070279514723959168403612848057292501736946181390625835070279514724`50.\
*^-9*I)*CF^2*irrational[Zeta[3]], 
 1.130045620204897480919520107426262325506772534750611671574375831132362`50.*^\
-8*CA*CF + 
  1.292475461715661789751138450036587846520986882932584214812421032194985`50.\
*^-8*CF^2 - 
  1.46753366082281438303024183816114290284922886190108568142533178561407`50.*^\
-9*CA*CF*L - 
  9.00434822655015676685769799946512718978599352099787732440009463443013`50.*^\
-9*CF^2*L + 
  4.7830517278282732992632146975745763788996276673208794585360406370672`50.*^\
-10*CA*CF*L^2 + 
  1.69538210026970892721666712348942939413438123845074160264383694515365`50.*^\
-9*CF^2*L^2 - 
  1.26764235250598479193603084933539906825959210526961046344953629685083`50.*^\
-9*CF*nf + 
  2.1922349957228726240260634560411625571456114052039413347540038432112`50.*^\
-10*CF*L*nf - 
  8.696457686960496907751299450135593416181141213310689924610982976486`50.*^-\
11*CF*L^2*nf - 
  4.9263590725198696396614684480062292530052087758735412473013300561218`50.*^\
-10*CA*CF*irrational[Pi^2] - 
  2.7074323537578602031851016617866235914038493358937530579886753760792`50.*^\
-10*CF^2*irrational[Pi^2] - 
  1.338253653068467883282698097512912327727142541957356772171586986402`50.*^-\
11*CA*CF*L*irrational[Pi^2] + 
  5.353014612273871533130792390051649310908570167829427088686347945607`50.*^-\
11*CF^2*L*irrational[Pi^2] + 
  1.6059043836821614599392377170154947932725710503488281266059043836822`50.*^\
-10*CA*CF*irrational[Zeta[3]] - 
  6.4236175347286458397569508680619791730902842013953125064236175347286`50.*^\
-10*CF^2*irrational[Zeta[3]], 
 (
    8.447265797615417387600488780966393420925705416693313421328232295918`50.*^\
-10*I)*CA*CF + 
  (
    1.00501186962637415593874420438294805046357965596607708221139176166393`50.\
*^-9*I)*CF^2 - 
  (
    1.1167630223678967096045300875279001248110283032315740135349388118578`50.*^\
-10*I)*CA*CF*L - 
  (
    6.8657377668270283965908530963592557161725820934724077596476734883007`50.*^\
-10*I)*CF^2*L + 
  (
    3.486877462720545086444912662199196946049153218820705948510536632585`50.*^\
-11*I)*CA*CF*L^2 + 
  (
    1.2614174797733155879600583997917776452364759191409684975274027387138`50.*^\
-10*I)*CF^2*L^2 - 
  (
    9.435311319907107542299041890252152130962779057440028500325489255079`50.*^\
-11*I)*CF*nf + 
  (
    1.676934871177204428418596995825793257668035477302078200327873083463`50.*^\
-11*I)*CF*L*nf - 
  (
    6.33977720494644561171802302218035808372573312512855627001915751379`50.*^\
-12*I)*CF*L^2*nf - 
  (
    3.674881035506553359371854669563875058416909723689223968346318519311`50.*^\
-11*I)*CA*CF*irrational[Pi^2] - 
  (
    1.982277481133990895412997321669408788425054650580130182791033501479`50.*^\
-11*I)*CF^2*irrational[Pi^2] - 
  (
    9.5589546647747705948764149822350880551938752996954055155113356172`50.*^-13\
*I)*CA*CF*L*irrational[Pi^2] + 
  (
    3.82358186590990823795056599289403522207755011987816220620453424686`50.*^\
-12*I)*CF^2*L*irrational[Pi^2] + 
  (
    1.147074559772972471385169797868210566623265035963448661861360274059`50.*^\
-11*I)*CA*CF*irrational[Zeta[3]] - 
  (
    4.588298239091889885540679191472842266493060143853794647445441096234`50.*^\
-11*I)*CF^2*irrational[Zeta[3]], 
 -5.873135879232757435984030187748893264147039713956829691276111014378`50.*^-\
11*CA*CF - 
  7.243617703576452040226050000684227610149047230492778701679887399642`50.*^-\
11*CF^2 + 
  7.88288907300404678345019459709317681374670865948370333651026105432`50.*^-12\
*CA*CF*L + 
  4.859351334178257808442828567830921892959178929817144300543403246115`50.*^-\
11*CF^2*L - 
  2.36856866197056887134754305680922608162006612111567040673852756077`50.*^-12\
*CA*CF*L^2 - 
  8.73069246705439589633396405125672391539659322467000712415885104976`50.*^-12\
*CF^2*L^2 + 
  6.53664874555183299020946727471097636612562225951773212636222688171`50.*^-12\
*CF*nf - 
  1.18909115981303661565262830736492404184802075338303739348832035464`50.*^-12\
*CF*L*nf + 
  4.3064884763101252206318964669258656029455747656648552849791410196`50.*^-13*
   CF*L^2*nf + 
  2.54943377622801094242761851785292030109714792234297571819004667458`50.*^-12\
*CA*CF*irrational[Pi^2] + 
  1.35187176880186389770985799400078080676451442482936948488787516905`50.*^-12\
*CF^2*irrational[Pi^2] + 
  6.372636443183180396584276654823392036795916866463603677007557078`50.*^-14*
   CA*CF*L*irrational[Pi^2] - 
  2.5490545772732721586337106619293568147183667465854414708030228313`50.*^-13*
   CF^2*L*irrational[Pi^2] - 
  7.6471637318198164759011319857880704441551002397563244124090684937`50.*^-13*
   CA*CF*irrational[Zeta[3]] + 
  3.05886549272792659036045279431522817766204009590252976496362739749`50.*^-12\
*CF^2*irrational[Zeta[3]], 
 (
    -3.81693531054568756783474209263293747672307940447266342639718123568`50.*^\
-12*I)*CA*CF - 
  (
    4.86509877608746525395198319745897382858380329682932864901240062467`50.*^\
-12*I)*CF^2 + 
  (
    5.1896361365632656602191754051653673260153937929657467036785832809`50.*^-13\
*I)*CA*CF*L + 
  (
    3.20923969124486363559975929824133450049920230453824333427673656594`50.*^\
-12*I)*CF^2*L - 
  (
    1.5062165902696970101773111929374497713007539223559028125362414697`50.*^-13\
*I)*CA*CF*L^2 - 
  (
    5.6489999285302934330537348625602049972339541715433921264050128164`50.*^-13\
*I)*CF^2*L^2 + 
  (
    4.2351870725893884107531280718691838863215929611388274984350776417`50.*^-13\
*I)*CF*nf - 
  (7.85986982096336342354185622127897734952413388019633399736776909`50.*^-14*
    I)*CF*L*nf + 
  (2.738575618672176382140565805340817766001370767919823295520439036`50.*^-14*
    I)*CF*L^2*nf + 
  (
    1.6530475689039850274929414207270008772305909894200980928479257655`50.*^-13\
*I)*CA*CF*irrational[Pi^2] + 
  (8.627963118978867597323251071151698514070644475176644654164106504`50.*^-14*
    I)*CF^2*irrational[Pi^2] + 
  (3.98289777698948774786517290926462002299744804153975229812972317`50.*^-15*
    I)*CA*CF*L*irrational[Pi^2] - 
  (1.59315911079579509914606916370584800919897921661590091925188927`50.*^-14*
    I)*CF^2*L*irrational[Pi^2] - 
  (4.779477332387385297438207491117544027596937649847702757755667809`50.*^-14*
    I)*CA*CF*irrational[Zeta[3]] + 
  (
    1.9117909329549541189752829964470176110387750599390811031022671234`50.*^-13\
*I)*CF^2*irrational[Zeta[3]], 
 2.3285745065458137261045315093776778275120350841273796509675908064`50.*^-13*
   CA*CF + 
  3.059544723485788700747895686701933547837518132219587882075463161`50.*^-13*
   CF^2 - 
  3.201537633384625119103206984871240682872128896135851872094171369`50.*^-14*
   CA*CF*L - 
  1.9867065017169639111272692835416970852495928539415496345342511348`50.*^-13*
   CF^2*L + 
  9.00371692324806629080394386594682614779964421859780218538522759`50.*^-15*
   CA*CF*L^2 + 
  3.431541864371128974029658449878059131789275832259310032759753026`50.*^-14*
   CF^2*L^2 - 
  2.577083451179057050916432176477031950730226000825675435130189879`50.*^-14*
   CF*nf + 
  4.86632672990216672703835068439847918568924073258732521213176028`50.*^-15*
   CF*L*nf - 
  1.63703944059055750741889888471760475414538985792687312461549592`50.*^-15*
   CF*L^2*nf - 
  1.006097010295299282045884667641387271633104012123113830373474814`50.*^-14*
   CA*CF*irrational[Pi^2] - 
  5.17486232740785613297898680933718119415031763277935237693169086`50.*^-15*
   CF^2*irrational[Pi^2] - 
  2.3428810452879339693324546525086000135279106126704425283116019`50.*^-16*CA*
   CF*L*irrational[Pi^2] + 
  9.3715241811517358773298186100344000541116424506817701132464075`50.*^-16*
   CF^2*L*irrational[Pi^2] + 
  2.81145725434552076319894558301032001623349273520453103397392224`50.*^-15*
   CA*CF*irrational[Zeta[3]] - 
  1.124582901738208305279578233204128006493397094081812413589568896`50.*^-14*
   CF^2*irrational[Zeta[3]], 
 (1.338606498647899768958433157517068836957152054524094351776870204`50.*^-14*
    I)*CA*CF + 
  (1.808879424497871468844124876996644216570211331253524839872080882`50.*^-14*
    I)*CF^2 - 
  (1.85835244169852178073811525644409634428067162177604824229455208`50.*^-15*
    I)*CA*CF*L - 
  (1.157451149229078639666060511654960022635327320651367421871191025`50.*^-14*
    I)*CF^2*L + 
  (5.0776301021849100071735618734232826442756253865741065363894976`50.*^-16*
    I)*CA*CF*L^2 + 
  (1.96444675479144154815967737948176112763418011360772993151077864`50.*^-15*
    I)*CF^2*L^2 - 
  (1.47818569206232436330149558536896026600263226044089887576276584`50.*^-15*
    I)*CF*nf + 
  (2.8338820245107068288222950155258012364616347833155984548468069`50.*^-16*
    I)*CF*L*nf - 
  (9.232054731245290922133748860769604807773864339225648247980905`50.*^-17*I)*
   CF*L^2*nf - 
  (5.7697922283710733034309537349093175919678066468223479605140053`50.*^-16*
    I)*CA*CF*irrational[Pi^2] - 
  (2.9274007449887679775994762240353991116916305451612180226508641`50.*^-16*
    I)*CF^2*irrational[Pi^2] - 
  (1.30160058071551887185136369583811111862661700703913473795089`50.*^-17*I)*
   CA*CF*L*irrational[Pi^2] + 
  (5.20640232286207548740545478335244447450646802815653895180356`50.*^-17*I)*
   CF^2*L*irrational[Pi^2] + 
  (1.5619206968586226462216364350057333423519404084469616855410679`50.*^-16*
    I)*CA*CF*irrational[Zeta[3]] - 
  (6.2476827874344905848865457400229333694077616337878467421642717`50.*^-16*
    I)*CF^2*irrational[Zeta[3]], 
 -7.2751456697184548918704742070408257235558923395034812056790527`50.*^-16*CA*
   CF - 
  1.00913518958602542803852397177446575964610528111675494071326141`50.*^-15*
   CF^2 + 
  1.0186076823902643959246537983804394951625408759201055753818768`50.*^-16*CA*
   CF*L + 
  6.3684933943251228140536068941966928954147309386722571940630121`50.*^-16*
   CF^2*L - 
  2.710209238289830507905264726031299590655269889721579570313058`50.*^-17*CA*
   CF*L^2 - 
  1.0633528163108837963575769057829544715836135596015648277008827`50.*^-16*
   CF^2*L^2 + 
  8.018665448514391409337126166020541044709176496379934073119876`50.*^-17*CF*
   nf - 
  1.557911529676945755684084044149796114879626962882702468375521`50.*^-17*CF*
   L*nf + 4.92765316052696455982775404732963561937321798131196285511465396913\
1083688428468`50.*^-18*CF*L^2*nf + 
  3.12828214335588848900673091669305114398036916832697912817938`50.*^-17*CA*
   CF*irrational[Pi^2] + 
  1.567035559649015032849639061702121633283692459203536499468899`50.*^-17*
   CF^2*irrational[Pi^2] + 6.850529372186941430796651030726900624350615826521\
76177868889434780681901145855`50.*^-19*CA*CF*L*irrational[Pi^2] - 
  2.7402117488747765723186604122907602497402463306087047114755577391227276045\
83418`50.*^-18*CF^2*L*irrational[Pi^2] - 
  8.22063524662432971695598123687228074922073899182611413442668`50.*^-18*CA*
   CF*irrational[Zeta[3]] + 
  3.288254098649731886782392494748912299688295596730445653770669`50.*^-17*
   CF^2*irrational[Zeta[3]], 
 (-3.749460530477794776957367465230964130920962412766684400421055`50.*^-17*I)*
   CA*CF - 
  (5.329131806683170308309257759911416522448518293031426559978731`50.*^-17*I)*
   CF^2 + (5.2890638950448783080382587020383668401097544180829559189049099817\
7308568044675`50.*^-18*I)*CA*CF*L + 
  (3.319670801620594746171093419741616280448936606396425095966891`50.*^-17*I)*
   CF^2*L - (1.37308725874690597520847357197130790946655531140540940982558723\
4834677604313251`50.*^-18*I)*CA*CF*L^2 - 
  (5.458810435527298930083049548670291643374294232838213022210092953766125447\
100625`50.*^-18*I)*CF^2*L^2 + (4.12596511271475637089149892436619533514563965\
3445948278881640186894285109803175`50.*^-18*I)*CF*nf - 
  (8.111236991961252797176795634564330571421713276303385876049334284769745899\
37443`50.*^-19*I)*CF*L*nf + (2.4965222886307381367426792217660143808482823843\
7347165422834042697214109875136`50.*^-19*I)*CF*L^2*nf + 
  (1.608362533061222330486462090182582051385475760993584791306318801302436185\
444246`50.*^-18*I)*CA*CF*irrational[Pi^2] + 
  (7.960545193475215633910600424211262513812704791182883118037500533533365271\
71956`50.*^-19*I)*CF^2*irrational[Pi^2] + 
  (3.425264686093470715398325515363450312175307913260880889344447173903409505\
7293`50.*^-20*I)*CA*CF*L*irrational[Pi^2] - 
  (1.370105874437388286159330206145380124870123165304352355737778869561363802\
29171`50.*^-19*I)*CF^2*L*irrational[Pi^2] - 
  (4.110317623312164858477990618436140374610369495913057067213336608684091406\
87513`50.*^-19*I)*CA*CF*irrational[Zeta[3]] + 
  (1.644127049324865943391196247374456149844147798365222826885334643473636562\
750051`50.*^-18*I)*CF^2*irrational[Zeta[3]], 
 1.83734106871537810921728804609011059784849042324469410026606535153617339197\
0499`50.*^-18*CA*CF + 2.67177621883980961622257523916011007155916008571296859\
8274813527047357649814668`50.*^-18*CF^2 - 2.609026931775650061018810596229182\
05291170070363750493193401938917735850744808`50.*^-19*CA*CF*L - 
  1.6439737941720754073438851695457432268065019171527493697706847520010072455\
26711`50.*^-18*CF^2*L + 6.620233525733035444710210815432527556224099975933196\
0632748910242136994369236`50.*^-20*CA*CF*L^2 + 2.6648186054809283498732680274\
5227466475436350765384011014709147531384621714006`50.*^-19*CF^2*L^2 - 
  2.0190608479020655907651680292563379272549287196359809838548573412990189780\
7897`50.*^-19*CF*nf + 4.01111304442704262168982003781973132953688104906065329\
10745641789104542938683`50.*^-20*CF*L*nf - 1.20367882286055189903822014826045\
95556771090865333083751408892771297635339861`50.*^-20*CF*L^2*nf - 
  7.8625690102939718551648275049041911772510233465846940349144596302307275295\
533`50.*^-20*CA*CF*irrational[Pi^2] - 3.8478290396416344667410098708340862712\
671416445025792594024462263030855506567`50.*^-20*CF^2*irrational[Pi^2] - 
  1.6310784219492717692372978644587858629406228158385147092116415113825759551\
09`50.*^-21*CA*CF*L*irrational[Pi^2] + 
  6.5243136877970870769491914578351434517624912633540588368465660455303038204\
37`50.*^-21*CF^2*L*irrational[Pi^2] + 
  1.9572941063391261230847574373505430355287473790062176510539698136590911461\
31`50.*^-20*CA*CF*irrational[Zeta[3]] - 
  7.8291764253565044923390297494021721421149895160248706042158792546363645845\
24`50.*^-20*CF^2*irrational[Zeta[3]], 
 (8.5816298615661224959100684527902273142336734795591711174274695695711576957\
022`50.*^-20*I)*CA*CF + (1.27494827536828933618903024856754331661441897203439\
770839657924837624045163162`50.*^-19*I)*CF^2 - 
  (1.225788455869714332382074474117625626625363489758418943296599215445277896\
295`50.*^-20*I)*CA*CF*L - (7.754125974953772170016941310284024959466646725884\
8214353539359001111463758537`50.*^-20*I)*CF^2*L + 
  (3.044722439447623356205832426411141384313638554178238587768764627257930849\
139`50.*^-21*I)*CA*CF*L^2 + (1.2400498100164916200637647654395530865186461107\
562423473993561912298255145543`50.*^-20*I)*CF^2*L^2 - 
  (9.419203519915143632531998019534288259752166145151919201906158243731111820\
882`50.*^-21*I)*CF*nf + 
  (1.888852369055345891341888431814224435959185119585210436678063718900184185\
649`50.*^-21*I)*CF*L*nf - 
  (5.535858980813860647646968048020257062388433734869524705034117504105328816\
62`50.*^-22*I)*CF*L^2*nf - 
  (3.663589757352933327605811442120810197966699574633426984000822844724308353\
422`50.*^-21*I)*CA*CF*irrational[Pi^2] - 
  (1.773861309130162974920520346771573885898457343015186127116650151234035153\
967`50.*^-21*I)*CF^2*irrational[Pi^2] - 
  (7.413992827042144405624081202085390286093740071993248678234734142648072523\
2`50.*^-23*I)*CA*CF*L*irrational[Pi^2] + 
  (2.965597130816857762249632480834156114437496028797299471293893657059229009\
29`50.*^-22*I)*CF^2*L*irrational[Pi^2] + 
  (8.896791392450573286748897442502468343312488086391898413881680971177687027\
87`50.*^-22*I)*CA*CF*irrational[Zeta[3]] - 
  (3.558716556980229314699558977000987337324995234556759365552672388471074811\
147`50.*^-21*I)*CF^2*irrational[Zeta[3]], 
 -3.8287532799317640576885871489263344871661590292610671611209117931909881752\
73`50.*^-21*CA*CF - 
  5.8045101992233562077212607326257648287210369595861164541261519027730097182\
36`50.*^-21*CF^2 + 
  5.4978384708481348526915795380010078045221591876437409676764191823738021194`\
50.*^-22*CA*CF*L + 
  3.4914183251021195973691276001369594805329501192444113483950217163101017756\
05`50.*^-21*CF^2*L - 
  1.3385923204126840764077135875689313620685290302023057576390014055273354629\
2`50.*^-22*CA*CF*L^2 - 
  5.5127488640072433358194102514702733511064367099873977329538929602308338127\
3`50.*^-22*CF^2*L^2 + 
  4.1982256107503846285272301953262778715160536075011948747671788073270394025\
4`50.*^-22*CF*nf - 
  8.4898291323197549534810458066655187419868187271908934366484593789418852118`\
50.*^-23*CF*L*nf + 
  2.4338042189321528661958428864889661128518709640041922866163661918678826599`\
50.*^-23*CF*L^2*nf + 
  1.6306855091159344090688831521127758475124470704195916300190199176527245261\
2`50.*^-22*CA*CF*irrational[Pi^2] + 
  7.8161403588404405804046816026723462920262964881511873008397161227488174885`\
50.*^-23*CF^2*irrational[Pi^2] + 
  3.223475142192236698097426609602343602649452205214455947058580062020901097`\
50.*^-24*CA*CF*L*irrational[Pi^2] - 
  1.2893900568768946792389706438409374410597808820857823788234320248083604388`\
50.*^-23*CF^2*L*irrational[Pi^2] - 
  3.8681701706306840377169119315228123231793426462573471364702960744250813164`\
50.*^-23*CA*CF*irrational[Zeta[3]] + 
  1.5472680682522736150867647726091249292717370585029388545881184297700325265\
9`50.*^-22*CF^2*irrational[Zeta[3]], 
 (
    -1.6350621082972842553101571321747458888827780099729277316348698752596024\
7554`50.*^-22*I)*CA*CF - 
  (2.526588926338899454407583529961088254195787618539394606885638168807588595\
54`50.*^-22*I)*CF^2 + 
  (2.358946706500052327151696992181798157947750099256952339676391584312743009\
5`50.*^-23*I)*CA*CF*L + 
  (1.503853310177025733551829415040608109303903601219031326378343826806369802\
81`50.*^-22*I)*CF^2*L - 
  (
    5.63665975279476171606691507625146644523269303158773067989548592561174417`\
50.*^-24*I)*CA*CF*L^2 - 
  (2.345991489466221489142844546902482837671904998584918073477545690518568467\
7`50.*^-23*I)*CF^2*L^2 + 
  (1.791297806717630342390774849324802611783850583412635059075722368052589001\
3`50.*^-23*I)*CF*nf - 
  (
    3.649945964541794612636917947544331463223547998818586381143909637192784809`\
50.*^-24*I)*CF*L*nf + 
  (
    1.024847227780865766557620922954812080951398733015951032708270168293044395`\
50.*^-24*I)*CF*L^2*nf + 
  (
    6.947535556147285236234209250435381304780902651418346284104933376317918668`\
50.*^-24*I)*CA*CF*irrational[Pi^2] + 
  (
    3.298243080776092606714625262645036771830456580920754498599627199380059016`\
50.*^-24*I)*CF^2*irrational[Pi^2] + 
  (
    1.34311464258009862420726108733430983443727175217268997794107502584204213`\
50.*^-25*I)*CA*CF*L*irrational[Pi^2] - 
  (
    5.37245857032039449682904434933723933774908700869075991176430010336816849`\
50.*^-25*I)*CF^2*L*irrational[Pi^2] - 
  (
    1.611737571096118349048713304801171801324726102607227973529290031010450548`\
50.*^-24*I)*CA*CF*irrational[Zeta[3]] + 
  (
    6.446950284384473396194853219204687205298904410428911894117160124041802194`\
50.*^-24*I)*CF^2*irrational[Zeta[3]], 
 6.695654884647742257683036330977185009612267959664655274128067566659129666`5\
0.*^-24*CA*CF + 
  1.0535490625109998107097104641920677197015844218632462625185207884698461611`\
50.*^-23*CF^2 - 
  9.70117707104613464648011663302428185255491968905641569534271425156554608`5\
0.*^-25*CA*CF*L - 
  6.208250377823291852453013005832871460818770995567326561522110837706387348`\
50.*^-24*CF^2*L + 
  2.27742720706029924681333057396592658476857704796080423247322533068267243`5\
0.*^-25*CA*CF*L^2 + 
  9.57440534180449533396813376210064543914726122387582309652063433738596942`5\
0.*^-25*CF^2*L^2 - 
  7.33013260435654378482634463036669894556144705038863975998951914273588357`5\
0.*^-25*CF*nf + 
  1.50382763534309190221922998883984390757446299322540894784263610572187178`5\
0.*^-25*CF*L*nf - 
  4.1407767401096349942060555890289574268519582690196440590422278739684953`50.\
*^-26*CF*L^2*nf - 
  2.83850121179169057121821813502343565211869174016771171095366762915424287`5\
0.*^-25*CA*CF*irrational[Pi^2] - 
  1.33528762301984663599357620890492126106642500531311986700631811617397058`5\
0.*^-25*CF^2*irrational[Pi^2] - 
  5.372458570320394496829044349337239337749087008690759911764300103368168`50.\
*^-27*CA*CF*L*irrational[Pi^2] + 
  2.1489834281281577987316177397348957350996348034763039647057200413472674`50.\
*^-26*CF^2*L*irrational[Pi^2] + 
  6.4469502843844733961948532192046872052989044104289118941171601240418022`50.\
*^-26*CA*CF*irrational[Zeta[3]] - 
  2.57878011375378935847794128768187488211956176417156475764686404961672088`5\
0.*^-25*CF^2*irrational[Zeta[3]], 
 (
    2.63375663031816436176782634423312057671933240987163925157046002350379334`\
50.*^-25*I)*CA*CF + 
  (
    4.21592376794064960384845534986035044902460437576755081467084333862006829`\
50.*^-25*I)*CF^2 - 
  (
    3.8306434737390994130846025173961451071055213987624368069930343798218811`\
50.*^-26*I)*CA*CF*L - 
  (
    2.46065393027824439742971366390495587791208141830117434397723453281111909`\
50.*^-25*I)*CF^2*L + 
  (
    8.843634872642378610184313818494960664331355026052816135769484425422596`50.\
*^-27*I)*CA*CF*L^2 + 
  (
    3.7536844018447576252836711782898324933009087158865932701690514364926241`\
50.*^-26*I)*CF^2*L^2 - 
  (
    2.8815495357585312565779354907926589099199053964306644163948711985672508`\
50.*^-26*I)*CF*nf + 
  (
    5.948407636851354843584152894602200725600848447865564959388566809175826`50.\
*^-27*I)*CF*L*nf - 
  (
    1.607933613207705201851693421544538302605700913827784751958088077349563`50.\
*^-27*I)*CF*L^2*nf - 
  (
    1.1139916559081936462256574032971053602644363428007255738597043179603622`\
50.*^-26*I)*CA*CF*irrational[Pi^2] - 
  (
    5.194994532495847288786608390451759276155093971605084066752746174782997`50.\
*^-27*I)*CF^2*irrational[Pi^2] - 
  (
    2.06633021935399788339578628820663051451887961872721535067857696283391`50.\
*^-28*I)*CA*CF*L*irrational[Pi^2] + 
  (
    8.26532087741599153358314515282652205807551847490886140271430785133564`50.\
*^-28*I)*CF^2*L*irrational[Pi^2] + 
  (
    2.479596263224797460074943545847956617422655542472658420814292355400693`50.\
*^-27*I)*CA*CF*irrational[Zeta[3]] - 
  (
    9.918385052899189840299774183391826469690622169890633683257169421602773`50.\
*^-27*I)*CF^2*irrational[Zeta[3]], 
 -9.966765841746374124467286670716753476991892133725736319965477150642677`50.\
*^-27*CA*CF - 
  1.6216942595584088561019263649424372987715381641315431483139405264150473`50.\
*^-26*CF^2 + 
  1.454654232876716681201356930130113331261168357313416604145465857871099`50.\
*^-27*CA*CF*L + 
  9.378789232212064886787431110363685829920533679076221760609976715548624`50.\
*^-27*CF^2*L - 
  3.30552437256283316143177140984736692683346694936670605321811005891925`50.*^\
-28*CA*CF*L^2 - 
  1.415926272339769838541891589595964372147382398719126128517006662785812`50.\
*^-27*CF^2*L^2 + 
  1.089890080275594356726943454345847950476209384777271220546663971975416`50.\
*^-27*CF*nf - 
  2.26255590169754063367425902816941138592673480520489239142980923163436`50.*^\
-28*CF*L*nf + 
  6.010044313750605748057766199722485321515394453394011005851109198035`50.*^-\
29*CF*L^2*nf + 
  4.20617802707729211389408264219549778241889588765626472172064233418892`50.*^\
-28*CA*CF*irrational[Pi^2] + 
  1.94526616662983380580889137079431659337822032014027329186815527509104`50.*^\
-28*CF^2*irrational[Pi^2] + 
  7.653074886496288457021430697061594498218072661952649446957692454941`50.*^-\
30*CA*CF*L*irrational[Pi^2] - 
  3.0612299545985153828085722788246377992872290647810597787830769819761`50.*^\
-29*CF^2*L*irrational[Pi^2] - 
  9.1836898637955461484257168364739133978616871943431793363492309459285`50.*^\
-29*CA*CF*irrational[Zeta[3]] + 
  3.6734759455182184593702867345895653591446748777372717345396923783714`50.*^\
-28*CF^2*irrational[Zeta[3]], 
 (
    -3.63380591402631601766089831988426479699993304721428677672285602702275`50.\
*^-28*I)*CA*CF - 
  (
    6.00530221945508632720953972318140220242239958546623467852865398122661`50.\
*^-28*I)*CF^2 + 
  (
    5.3202782816057947694869356863610987749821515544022086812481041733913`50.*^\
-29*I)*CA*CF*L + 
  (
    3.44272339316684837960385435871665977433338350791705320057525455767101`50.\
*^-28*I)*CF^2*L - 
  (
    1.1909242269730880169135146038245810820533281842090399814791698505202`50.*^\
-29*I)*CA*CF*L^2 - 
  (
    5.1461945969623212733893617795014171105175070780272169348888613576167`50.*^\
-29*I)*CF^2*L^2 + 
  (
    3.9719515731935450143877373486066919510736997931771571751108091519746`50.*^\
-29*I)*CF*nf - 
  (
    8.287891748999436306546150992035229093251857838042881593522994175082`50.*^\
-30*I)*CF*L*nf + 
  (
    2.165316776314705485297299279681056512824233062198254511780308819127`50.*^\
-30*I)*CF*L^2*nf + 
  (
    1.530151778319677115238660776525974694136965065673500912522899701857`50.*^\
-29*I)*CA*CF*irrational[Pi^2] + 
  (
    7.020517505641311949054858539946134517802925778957863881625901823243`50.*^\
-30*I)*CF^2*irrational[Pi^2] + 
  (
    2.73324103089153159179336810609342660650645452212594623105631873391`50.*^\
-31*I)*CA*CF*L*irrational[Pi^2] - 
  (
    1.093296412356612636717347242437370642602581808850378492422527493563`50.*^\
-30*I)*CF^2*L*irrational[Pi^2] - 
  (
    3.279889237069837910152041727312111927807745426551135477267582480689`50.*^\
-30*I)*CA*CF*irrational[Zeta[3]] + 
  (
    1.3119556948279351640608166909248447711230981706204541909070329922755`50.*^\
-29*I)*CF^2*irrational[Zeta[3]], 
 1.2781311257663675766886351893904717287127788620235593001224197413578`50.*^-\
29*CA*CF + 
  2.1439056584895158688658254482095600628775304088252422002394754694016`50.*^\
-29*CF^2 - 
  1.876693542739981308673067690273155886725436868102027513453991263978`50.*^-\
30*CA*CF*L - 
  1.2187468521634511310717956162718557403997967480381804461552470498906`50.*^\
-29*CF^2*L + 
  4.14123192608932599999297205166049135271916434938031746351217654651`50.*^-31\
*CA*CF*L^2 + 
  1.804575467138842266155551803538578856084284049466377054464525974284`50.*^-\
30*CF^2*L^2 - 
  1.396585735081622367944140803815443602332105365671249583944528043941`50.*^-\
30*CF*nf + 
  2.92776837667379790809279921260124509071414602434390974395557323567`50.*^-31\
*CF*L*nf - 
  7.5295125928896836363508582757463479140348442716005772063857755391`50.*^-32*
   CF*L^2*nf - 
  5.37037524406756913604354017012852530286465712289933160039844527901`50.*^-31\
*CA*CF*irrational[Pi^2] - 
  2.44527296673156851219473956115161864681387971407557676408442064345`50.*^-31\
*CF^2*irrational[Pi^2] - 
  9.424969072039764109632303814115264160367084559054987003642478393`50.*^-33*
   CA*CF*L*irrational[Pi^2] + 
  3.7699876288159056438529215256461056641468338236219948014569913571`50.*^-32*
   CF^2*L*irrational[Pi^2] + 
  1.13099628864477169315587645769383169924405014708659844043709740713`50.*^-31\
*CA*CF*irrational[Zeta[3]] - 
  4.52398515457908677262350583077532679697620058834639376174838962854`50.*^-31\
*CF^2*irrational[Zeta[3]], 
 (
    4.34251673290451725686836271263590984872044828173298386236722472709`50.*^-31\
*I)*CA*CF + 
  (
    7.38825312409503255763367703294680532581212093787345597797263102886`50.*^\
-31*I)*CF^2 - 
  (
    6.3928131706289571001027231130599936112107666017616661953142664616`50.*^-32\
*I)*CA*CF*L - 
  (
    4.16615630125693226138183429527228861376402972064553466191883995164`50.*^\
-31*I)*CF^2*L + 
  (
    1.3915700672157668595857983769445155379851560881081535661993438666`50.*^-32\
*I)*CA*CF*L^2 + 
  (
    6.1129008775688058204962565355290943600411413811852144705731988736`50.*^-32\
*I)*CF^2*L^2 - 
  (
    4.7436380643409620825712767562440706162223975021915735801963989713`50.*^-32\
*I)*CF*nf + 
  (9.987017110792951228222400092555337632579759752726462653435422835`50.*^-33*
    I)*CF*L*nf - 
  (2.530127394937757926519633412626391887245738342014824665816988849`50.*^-33*
    I)*CF*L^2*nf - 
  (
    1.8207073652705227315045233373098210610461030942127832651162547617`50.*^-32\
*I)*CA*CF*irrational[Pi^2] - 
  (8.229689302308389028535199864507217520619030991086447817104777406`50.*^-33*
    I)*CF^2*irrational[Pi^2] - 
  (3.14165635734658803654410127137175472012236151968499566788082613`50.*^-34*
    I)*CA*CF*L*irrational[Pi^2] + 
  (1.256662542938635214617640508548701888048944607873998267152330452`50.*^-33*
    I)*CF^2*L*irrational[Pi^2] + 
  (3.769987628815905643852921525646105664146833823621994801456991357`50.*^-33*
    I)*CA*CF*irrational[Zeta[3]] - 
  (
    1.5079950515263622575411686102584422656587335294487979205827965428`50.*^-32\
*I)*CF^2*irrational[Zeta[3]], 
 -1.4267938221927181488468073888342273630306955053822433773349997008`50.*^-32*
   CA*CF - 
  2.4607909524468037959089622199998245116501154275738086039052197883`50.*^-32*
   CF^2 + 
  2.105461308748995500749658280974220965346965131277306365870714442`50.*^-33*
   CA*CF*L + 
  1.3768449493502962068525130833706727763156836738370752717257718319`50.*^-32*
   CF^2*L - 
  4.52380666962945633413712665496631656410193103990140410233301575`50.*^-34*
   CA*CF*L^2 - 
  2.002658801439195192511846444620152421688838754720622530798166429`50.*^-33*
   CF^2*L^2 + 
  1.55825216478415122773006201530554428134477441941068651066979848`50.*^-33*
   CF*nf - 
  3.29352664221876961599394494723858549412435131026952572320820444`50.*^-34*
   CF*L*nf + 
  8.2251030356899206075220484635751210256398746180025529133327559`50.*^-35*CF*
   L^2*nf + 
  5.96961199157931612588176563689932678363890370045628530195643345`50.*^-34*
   CA*CF*irrational[Pi^2] + 
  2.67937969450222497390255453923841204311489025117215877090516571`50.*^-34*
   CF^2*irrational[Pi^2] + 
  1.0134375346279316246916455714102434581039875869951598928647826`50.*^-35*CA*
   CF*L*irrational[Pi^2] - 
  4.0537501385117264987665822856409738324159503479806395714591305`50.*^-35*
   CF^2*L*irrational[Pi^2] - 
  1.21612504155351794962997468569229214972478510439419187143773915`50.*^-34*
   CA*CF*irrational[Zeta[3]] + 
  4.86450016621407179851989874276916859889914041757676748575095659`50.*^-34*
   CF^2*irrational[Zeta[3]], 
 (-4.53848369561955436416228010343290300736344219066036974442941802`50.*^-34*
    I)*CA*CF - 
  (7.93033887137828419919086136858742068049601904364882897864426508`50.*^-34*
    I)*CF^2 + 
  (6.7118413478143526290437561140063355528013810106860132600876696`50.*^-35*
    I)*CA*CF*L + 
  (4.40397197075100301625902887027359692006281357667286469728311535`50.*^-34*
    I)*CF^2*L - 
  (1.4242559280399363538365982694294417104986430723864464520477116`50.*^-35*
    I)*CA*CF*L^2 - 
  (6.3522113633603242160270570995187033057593287140210656922230973`50.*^-35*
    I)*CF^2*L^2 + 
  (4.955822137267491782176999677825103865587822454349997368238459`50.*^-35*I)*
   CF*nf - 
  (1.051230629261272671029708683324720414060376684779668127623402`50.*^-35*I)*
   CF*L*nf + 
  (2.589556232799884279702905944417166746361169222520811730995839`50.*^-36*I)*
   CF*L^2*nf + 
  (1.8949383628451769552494273654352245265017393875090079935726972`50.*^-35*
    I)*CA*CF*irrational[Pi^2] + 
  (8.447778611455690386836286373716000305653857275209448664310205`50.*^-36*I)*
   CF^2*irrational[Pi^2] + (3.16699229571228632716139241065701080657496120935\
9874665202445528075756510525259`50.*^-37*I)*CA*CF*L*irrational[Pi^2] - 
  (1.266796918284914530864556964262804322629984483743949866080978`50.*^-36*I)*
   CF^2*L*irrational[Pi^2] - 
  (3.800390754854743592593670892788412967889953451231849598242935`50.*^-36*I)*
   CA*CF*irrational[Zeta[3]] + 
  (1.5201563019418974370374683571153651871559813804927398392971739`50.*^-35*
    I)*CF^2*irrational[Zeta[3]], 
 1.3990376622416403709863913482660702434157493683658308155283383`50.*^-35*CA*
   CF + 
  2.4754646384125655722303672606396806082109325704521802265354607`50.*^-35*
   CF^2 - 
  2.073131170017489804407415432828905493523964501341585695796352`50.*^-36*CA*
   CF*L - 
  1.3647900447202696509432641213454912380589996848625110223786337`50.*^-35*
   CF^2*L + 
  4.34700288094474731613499831774068580884828309990647142427644`50.*^-37*CA*
   CF*L^2 + 
  1.95273209683669311713673950167108973214694883955833940549997`50.*^-36*CF^2*
   L^2 - 
  1.527515404777812821236817651580147310944695249786721708349545`50.*^-36*CF*
   nf + 3.2508733816028127640213903775237993222833144037011767331382520445975\
4956200123`50.*^-37*CF*L*nf - 7.903641601717722392972724214073974197905969272\
5572207714117040837089978442336`50.*^-38*CF*L^2*nf - 
  5.82947500944608667106768429489698548188265200586592430000577`50.*^-37*CA*
   CF*irrational[Pi^2] - 2.58192648563788274113497269899275559292949918153732\
2221971425562248801235183163`50.*^-37*CF^2*irrational[Pi^2] - 
  9.5969463506432919004890679110818509290150339677571959551589263530300559444\
782`50.*^-39*CA*CF*L*irrational[Pi^2] + 3.83877854025731676019562716443274037\
160601358710287838206357054121202237779129`50.*^-38*CF^2*L*irrational[Pi^2] + 
  1.1516335620771950280586881493298221114818040761308635146190711623636067133\
37387`50.*^-37*CA*CF*irrational[Zeta[3]] - 
  4.60653424830878011223475259731928844592721630452345405847628`50.*^-37*CF^2*
   irrational[Zeta[3]], 
 (4.18346330758364324159665027726291461026862887133898153843173`50.*^-37*I)*
   CA*CF + 
  (7.49198980282425638738075010932251524721379770254844660548878`50.*^-37*I)*
   CF^2 - (6.2104913011536734930793570624813225218191326831470502841371624631\
600627075888`50.*^-38*I)*CA*CF*L - 
  (4.10178327671185368095589263855811048155806058640226644604252`50.*^-37*I)*
   CF^2*L + (1.28740863363282088349820281919748763843401729985135193861536934\
246733541525478`50.*^-38*I)*CA*CF*L^2 + 
  (5.823372353660236084585097065470025119789269148323268719265641470267092758\
41079`50.*^-38*I)*CF^2*L^2 - (4.567313457235200711066008588515615349496414591\
79710119635922705531753507768187`50.*^-38*I)*CF*nf + 
  (9.749733219565747050860719024197851922382132824446677676806086746886750061\
9721`50.*^-39*I)*CF*L*nf - (2.34074297024149251545127785308634116078912236336\
60944338461260772133371186451`50.*^-39*I)*CF*L^2*nf - 
  (1.739661743632093190590872195899666245065253934027358941608310775472032792\
24405`50.*^-38*I)*CA*CF*irrational[Pi^2] - 
  (7.656776150897090572456668222906331011871096587079916944405371781230099973\
7929`50.*^-39*I)*CF^2*irrational[Pi^2] - 
  (2.822631279600968206026196444435838508533833519928587045634978339126487042\
494`50.*^-40*I)*CA*CF*L*irrational[Pi^2] + 
  (1.129052511840387282410478577774335403413533407971434818253991335650594816\
9974`50.*^-39*I)*CF^2*L*irrational[Pi^2] + 
  (3.387157535521161847231435733323006210240600223914304454761974006951784450\
9923`50.*^-39*I)*CA*CF*irrational[Zeta[3]] - 
  (1.354863014208464738892574293329202484096240089565721781904789602780713780\
39693`50.*^-38*I)*CF^2*irrational[Zeta[3]], 
 -1.2145587346318920730595460904580171028549759791223602413600539364327697610\
8102`50.*^-38*CA*CF - 2.20050052666802919655144031146171276317792361696936662\
979751827300528616997391`50.*^-38*CF^2 + 1.8060802730188407063751558520073813\
663650425277840225756395403472625876744395`50.*^-39*CA*CF*L + 
  1.1966398513046239946944895910949067167547997643069516632581256529574552328\
2142`50.*^-38*CF^2*L - 
  3.7029714295018706634882214865542469106803009024741709105518319089203314979\
44`50.*^-40*CA*CF*L^2 - 1.686205465331396971185987071238646635392799398041515\
1498790821698747305694317`50.*^-39*CF^2*L^2 + 1.32596001583323144483074262709\
35966855708598211246459830740081832110433568693`50.*^-39*CF*nf - 
  2.8384135441225829152215428605603381004272197932987997198171854457815359486\
33`50.*^-40*CF*L*nf + 
  6.7326753263670375699785845210077216557823652772257652919124216525824209053\
5`50.*^-41*CF*L^2*nf + 
  5.0407115152039315853459163269330166700517140854637401698097322538755351859\
49`50.*^-40*CA*CF*irrational[Pi^2] + 
  2.2051283039231261652366857160281339335808904263723709446695674230394392074\
02`50.*^-40*CF^2*irrational[Pi^2] + 
  8.0646607988599091600748469841023957386680957712245344160999381117899629785`\
50.*^-42*CA*CF*L*irrational[Pi^2] - 
  3.2258643195439636640299387936409582954672383084898137664399752447159851914\
2`50.*^-41*CF^2*L*irrational[Pi^2] - 
  9.6775929586318909920898163809228748864017149254694412993199257341479555742\
6`50.*^-41*CA*CF*irrational[Zeta[3]] + 
  3.8710371834527563968359265523691499545606859701877765197279702936591822297\
05`50.*^-40*CF^2*irrational[Zeta[3]], 
 (-3.426481319186219668709075899031577427536516428267199563767898933053054820\
154`50.*^-40*I)*CA*CF - 
  (6.277804614754018794130637775750665840032639328366759758929938015440776247\
033`50.*^-40*I)*CF^2 + 
  (5.103106089755748221242129082163450750610792428037335826393299538133122719\
94`50.*^-41*I)*CA*CF*L + 
  (3.391666983832998032551688218434438319996508494970155004966320575611475146\
05`50.*^-40*I)*CF^2*L - 
  (1.035268048450682037429619806049282513902499753162270480163343242267299918\
48`50.*^-41*I)*CA*CF*L^2 - 
  (4.744799792264956158206398951466618016651756280337001313825063244446477484\
32`50.*^-41*I)*CF^2*L^2 + 
  (3.740771796836567980420597432829597238656648000429494784167982268982803051\
86`50.*^-41*I)*CF*nf - 
  (8.028326279916769258571435169082720756846677473324660102876900081283625048\
9`50.*^-42*I)*CF*L*nf + 
  (1.882305542637603704417490556453240934368181369385946327569714985940545306\
3`50.*^-42*I)*CF*L^2*nf + 
  (1.419315497235815875631735928601552545102367066024358017342549091090033691\
06`50.*^-41*I)*CA*CF*irrational[Pi^2] + 
  (6.172618931833561302646452965319615597496717132744568996366218187585555411\
1`50.*^-42*I)*CF^2*irrational[Pi^2] + 
  (
    2.240183555238863655576346384472887705185582158673481782249982808830545272`\
50.*^-43*I)*CA*CF*L*irrational[Pi^2] - 
  (
    8.960734220955454622305385537891550820742328634693927128999931235322181087`\
50.*^-43*I)*CF^2*L*irrational[Pi^2] - 
  (2.688220266286636386691615661367465246222698590408178138699979370596654326\
2`50.*^-42*I)*CA*CF*irrational[Zeta[3]] + 
  (1.075288106514654554676646264546986098489079436163271255479991748238661730\
47`50.*^-41*I)*CF^2*irrational[Zeta[3]], 
 9.4009309293119785546040257427444329533795622419814741565363493404844715907`\
50.*^-42*CA*CF + 
  1.7410787577662829865372546317333883560677409232947393537274015126999541273\
4`50.*^-41*CF^2 - 
  1.4020769432448630124355213780461217851138404703406197462303613590751309118`\
50.*^-42*CA*CF*L - 
  9.3470764623412130453633230444458396501866306123455548726857214471052334966`\
50.*^-42*CF^2*L + 
  2.815560227707352606415408042584351928544104581739265900105840360234169545`\
50.*^-43*CA*CF*L^2 + 
  1.2985050366734254605395271731724095900064333050729058206263154801907630833`\
50.*^-42*CF^2*L^2 - 
  1.0263596128410596822375527125987223626664192773460105161221854447643567946`\
50.*^-42*CF*nf + 
  2.207981598153580503029836333116250378380970523114949469352014140771635393`\
50.*^-43*CF*L*nf - 
  5.11920041401336837530074189560791259735291742134411981837425520042576281`5\
0.*^-44*CF*L^2*nf - 
  3.886633995337504378255509164552056193800080245483886341869020422837733414`\
50.*^-43*CA*CF*irrational[Pi^2] - 
  1.680721082339763928277650239329052358201125912042822051824066439707729906`\
50.*^-43*CF^2*irrational[Pi^2] - 
  6.0545501492942260961522875256023992032042761045229237358107643481906629`50.\
*^-45*CA*CF*L*irrational[Pi^2] + 
  2.42182005971769043846091501024095968128171044180916949432430573927626516`5\
0.*^-44*CF^2*L*irrational[Pi^2] + 
  7.26546017915307131538274503072287904384513132542750848297291721782879548`5\
0.*^-44*CA*CF*irrational[Zeta[3]] - 
  2.90618407166122852615309801228915161753805253017100339318916688713151819`5\
0.*^-43*CF^2*irrational[Zeta[3]], 
 (
    2.510252379385054465774933279097941923690891946185278010574651578096155703`\
50.*^-43*I)*CA*CF + 
  (
    4.697753886066233908298823539249801603714403631888997774217943815289675241`\
50.*^-43*I)*CF^2 - 
  (
    3.74871588865007297271166700145523940456801609925674584992078475445949553`\
50.*^-44*I)*CA*CF*L - 
  (
    2.506603329736174175347431100865903798346244087222339109924396208194485476`\
50.*^-43*I)*CF^2*L + 
  (
    7.4543378917168424371605151284851960248767058669184340564188115072882196`\
50.*^-45*I)*CA*CF*L^2 + 
  (
    3.45872267327226613700950611194922827078661487855415203919924142242101039`\
50.*^-44*I)*CF^2*L^2 - 
  (
    2.74077297944684854345096287603635188191651337568969144049301602662274033`\
50.*^-44*I)*CF*nf + 
  (
    5.9091089759166209115862190346166800352376159302323106766159020976266587`\
50.*^-45*I)*CF*L*nf - 
  (
    1.3553341621303349885746391142700356408866737939851698284397839104160399`\
50.*^-45*I)*CF*L^2*nf - 
  (
    1.03586879975320433482826533145862977936393998796454730698726402539472246`\
50.*^-44*I)*CA*CF*irrational[Pi^2] - 
  (
    4.4548776296389581348029972882399740970031719494646262493160879659477306`\
50.*^-45*I)*CF^2*irrational[Pi^2] - 
  (
    1.593302670866901604250601980421684000843230553821822035739674828471227`50.\
*^-46*I)*CA*CF*L*irrational[Pi^2] + 
  (
    6.373210683467606417002407921686736003372922215287288142958699313884908`50.\
*^-46*I)*CF^2*L*irrational[Pi^2] + 
  (
    1.9119632050402819251007223765060208010118766645861864428876097941654725`\
50.*^-45*I)*CA*CF*irrational[Zeta[3]] - 
  (
    7.64785282016112770040288950602408320404750665834474577155043917666189`50.\
*^-45*I)*CF^2*irrational[Zeta[3]], 
 -6.5282575338606063667122724121327895164637173568416980737357297109701781`50.\
*^-45*CA*CF - 
  1.23409023166730660489651554957132560951070840506622984168654157466229296`5\
0.*^-44*CF^2 + 
  9.760732826818673589359753433200255001600992946753982454147731023543801`50.\
*^-46*CA*CF*L + 
  6.5457454973288537438133741724704085296200071339819669961279214542537719`50.\
*^-45*CF^2*L - 
  1.922610542867076334184296303392566273763242222794813461263646396402655`50.\
*^-46*CA*CF*L^2 - 
  8.973148137838627902725218412620555952147879418314805455643476901606564`50.\
*^-46*CF^2*L^2 + 
  7.128400456264270828811575565195394808361075427200427955254592046760187`50.\
*^-46*CF*nf - 
  1.540003208647386356942227450842487893226409962806360461965773874226205`50.\
*^-46*CF*L*nf + 
  3.49565553248559333488053873344102958866044040508147902047935708436846`50.*^\
-47*CF*L^2*nf + 
  2.688954441504196660582702566206193435460097170934761162246223105630906`50.\
*^-46*CA*CF*irrational[Pi^2] + 
  1.150262921952640863080947133152434008243644424968741149335219711914943`50.\
*^-46*CF^2*irrational[Pi^2] + 
  4.0853914637612861647451332831325230790852065482610821429222431499262`50.*^\
-48*CA*CF*L*irrational[Pi^2] - 
  1.63415658550451446589805331325300923163408261930443285716889725997049`50.*^\
-47*CF^2*L*irrational[Pi^2] - 
  4.90246975651354339769415993975902769490224785791329857150669177991147`50.*^\
-47*CA*CF*irrational[Zeta[3]] + 
  1.960987902605417359077663975903611077960899143165319428602676711964587`50.\
*^-46*CF^2*irrational[Zeta[3]], 
 (
    -1.654657536457859240759656713227679852207331549539850104033985411725706`50.\
*^-46*I)*CA*CF - 
  (
    3.158569637265483009899404933206035122602464993395511199912430399606486`50.\
*^-46*I)*CF^2 + 
  (
    2.47668521943061169892213500486412973405060457469069952577594544640659`50.\
*^-47*I)*CA*CF*L + 
  (
    1.665697974535229426730272480853126265137883665534040928273895651120002`50.\
*^-46*I)*CF^2*L - 
  (
    4.8339446838069220863580630071524390163823232378392025228980733073849`50.*^\
-48*I)*CA*CF*L^2 - 
  (
    2.26895322359471925683679622357013821159102229487661536931465784626099`50.\
*^-47*I)*CF^2*L^2 + 
  (
    1.8069703695585142018484554297109495665614814300648981099475380919464`50.*^\
-47*I)*CF*nf - 
  (
    3.9110616369662849141478609231457963129440574902273947898748296312129`50.*^\
-48*I)*CF*L*nf + 
  (
    8.788990334194403793378296376640798211604224068798550041632860558882`50.*^\
-49*I)*CF*L^2*nf + 
  (
    6.8030708610726087683010304415263903349692588825576652031702159313508`50.*^\
-48*I)*CA*CF*irrational[Pi^2] + 
  (
    2.8951454817699208068215701159564929310888004613217804606366512314688`50.*^\
-48*I)*CF^2*irrational[Pi^2] + 
  (
    1.021347865940321541186283320783130769771301637065270535730560787482`50.*^\
-49*I)*CA*CF*L*irrational[Pi^2] - 
  (
    4.085391463761286164745133283132523079085206548261082142922243149926`50.*^\
-49*I)*CF^2*L*irrational[Pi^2] - 
  (
    1.2256174391283858494235399849397569237255619644783246428766729449779`50.*^\
-48*I)*CA*CF*irrational[Zeta[3]] + 
  (
    4.9024697565135433976941599397590276949022478579132985715066917799115`50.*^\
-48*I)*CF^2*irrational[Zeta[3]], 
 4.0900497074586202373897929970836857788641542183570337709787691125104`50.*^-\
48*CA*CF + 
  7.8815506775904733761540304745824242613025115176257112991438760827623`50.*^\
-48*CF^2 - 
  6.128182729692731100502563862831983648804164284932471374981987774637`50.*^-\
49*CA*CF*L - 
  4.1331554804372933387571088247109265652527690377199271098461596487899`50.*^\
-48*CF^2*L + 
  1.185538888667881312819344987207217551491425370272806821330057572223`50.*^-\
49*CA*CF*L^2 + 
  5.595483966831203918873094137237433257744566193011870069516265688519`50.*^-\
49*CF^2*L^2 - 
  4.467139798025625613414802559253386999196946337809078160299002315796`50.*^-\
49*CF*nf + 
  9.68559013813387877002584338192893144863715505918840636084913387945`50.*^-50\
*CF*L*nf - 
  2.15552525212342056876244543128585009362077340049601240241828649495`50.*^-50\
*CF*L^2*nf - 
  1.678609422403845568972951188231917351677181992872580624071066559707`50.*^-\
49*CA*CF*irrational[Pi^2] - 
  7.10775598423278162921750201718214872947933361284740234902007953355`50.*^-50\
*CF^2*irrational[Pi^2] - 
  2.4910923559520037589909349287393433409056137489396842334891726524`50.*^-51*
   CA*CF*L*irrational[Pi^2] + 
  9.9643694238080150359637397149573733636224549957587369339566906096`50.*^-51*
   CF^2*L*irrational[Pi^2] + 
  2.98931082714240451078912191448721200908673649872762108018700718287`50.*^-50\
*CA*CF*irrational[Zeta[3]] - 
  1.195724330856961804315648765794884803634694599491048432074802873149`50.*^-\
49*CF^2*irrational[Zeta[3]], 
 (
    9.86568805420773679835751661693823394621059318085052700097363983095`50.*^-50\
*I)*CA*CF + 
  (
    1.918593398083686003760541883174342794286397864582609203211395176881`50.*^\
-49*I)*CF^2 - 
  (
    1.47956830141107815911954713505085736518166331441197647362598472434`50.*^\
-50*I)*CA*CF*L - 
  (
    1.000659135021985696835374298227107596529406630378656496093341350837`50.*^\
-49*I)*CF^2*L + 
  (
    2.8378926163444362552439917782053637512351031195844049065171487581`50.*^-51\
*I)*CA*CF*L^2 + 
  (
    1.3466267994428457375881205085799335417272070028986806296297079691`50.*^-50\
*I)*CF^2*L^2 - 
  (
    1.07768941042756642899955517563242734445885884947748781701977473601`50.*^\
-50*I)*CF*nf + 
  (2.340381713652107605173200012219538084968471770057696044911932128`50.*^-51*
    I)*CF*L*nf - 
  (5.159804756989884100443621414918843184063823853789827102758452288`50.*^-52*
    I)*CF*L^2*nf - 
  (4.041885972304871764937780111766323092087248628750884096857692017`50.*^-51*
    I)*CA*CF*irrational[Pi^2] - 
  (
    1.7031239203619294841222409457527381235798141411443924424165287142`50.*^-51\
*I)*CF^2*irrational[Pi^2] - 
  (5.93117227607619942616889268747462700215622321176115293687898251`50.*^-53*
    I)*CA*CF*L*irrational[Pi^2] + 
  (2.372468910430479770467557074989850800862489284704461174751593002`50.*^-52*
    I)*CF^2*L*irrational[Pi^2] + 
  (7.117406731291439311402671224969552402587467854113383524254779007`50.*^-52*
    I)*CA*CF*irrational[Zeta[3]] - 
  (
    2.8469626925165757245610684899878209610349871416453534097019116027`50.*^-51\
*I)*CF^2*irrational[Zeta[3]], 
 -2.3235758438541603970808516082351259897016386776015950906436706713`50.*^-51*
   CA*CF - 
  4.5589729543739285956584281249907978878210364748418769189292848954`50.*^-51*
   CF^2 + 
  3.487687619571456219039046201189062088583651860178621131005201417`50.*^-52*
   CA*CF*L + 
  2.3651954246195465218287625293796903593057290951772760107676448602`50.*^-51*
   CF^2*L - 
  6.6342516512741938094102295912922974019955058671242683424375664`50.*^-53*CA*
   CF*L^2 - 
  3.1645187631615765065570663523994765351671086709845521924686718`50.*^-52*
   CF^2*L^2 + 
  2.538613263785934535865200867734445373936409205227972957576050634`50.*^-52*
   CF*nf - 
  5.52120818203880165163547088539058497796824451582480121156214785`50.*^-53*
   CF*L*nf + 
  1.20622757295894432898367810750769043672645561220441242589773934`50.*^-53*
   CF*L^2*nf + 
  9.50302606994412259015963555897830488903542830941203733931855149`50.*^-53*
   CA*CF*irrational[Pi^2] + 
  3.98531331607763099507416931707560637933718578154772487325032985`50.*^-53*
   CF^2*irrational[Pi^2] + 
  1.3793423897851626572485796947615411632921449329677099853206936`50.*^-54*CA*
   CF*L*irrational[Pi^2] - 
  5.5173695591406506289943187790461646531685797318708399412827744`50.*^-54*
   CF^2*L*irrational[Pi^2] - 
  1.65521086774219518869829563371384939595057391956125198238483233`50.*^-53*
   CA*CF*irrational[Zeta[3]] + 
  6.62084347096878075479318253485539758380229567824500792953932931`50.*^-53*
   CF^2*irrational[Zeta[3]], 
 (-5.34639257652691546231635977865198451290485674918269426134026129`50.*^-53*
    I)*CA*CF - 
  (1.058061108808135852462249674148148538367873841772822181803672223`50.*^-52*
    I)*CF^2 + 
  (8.0312672380303419217953591980381103549100188272389163470990518`50.*^-54*
    I)*CA*CF*L + 
  (5.4609687469457101619901480645631305169498147741760896235694833`50.*^-53*
    I)*CF^2*L - 
  (1.5154512655490179012958261529449229955558148860538785448893964`50.*^-54*
    I)*CA*CF*L^2 - 
  (7.2654148720409418038336007131050782492744428821651730929139436`50.*^-54*
    I)*CF^2*L^2 + 
  (5.8422458429862471300672181806384059804573067882185025801974802`50.*^-54*
    I)*CF*nf - 
  (1.2723710810549683389142415923131325643730603779139055604464738`50.*^-54*
    I)*CF*L*nf + 
  (2.755365937361850729628774823536223628283299792825233717980721`50.*^-55*I)*
   CF*L^2*nf + 
  (2.1828566074760026161135440015308449775484347965987060754431992`50.*^-54*
    I)*CA*CF*irrational[Pi^2] + 
  (9.112128815988336738393270732664725543309355307681441503845458`50.*^-55*I)*
   CF^2*irrational[Pi^2] + 
  (3.13486906769355149374677203354895718930032939310843178481976`50.*^-56*I)*
   CA*CF*L*irrational[Pi^2] - 
  (1.253947627077420597498708813419582875720131757243372713927903`50.*^-55*I)*
   CF^2*L*irrational[Pi^2] - 
  (3.76184288123226179249612644025874862716039527173011814178371`50.*^-55*I)*
   CA*CF*irrational[Zeta[3]] + 
  (1.5047371524929047169984505761034994508641581086920472567134839`50.*^-54*
    I)*CF^2*irrational[Zeta[3]], 
 1.2024553306092188749556967151900015174262532675186665731724903`50.*^-54*CA*
   CF + 
  2.3996766239672707840132589572325082966276115920065466078195723`50.*^-54*
   CF^2 - 
  1.807623157381189255423033992443699900426438782142204446486175`50.*^-55*CA*
   CF*L - 
  1.2323332988823341337675196152339213629994488943738654808882478`50.*^-54*
   CF^2*L + 
  3.38433607997762251830736115573235603780237263013720177281036`50.*^-56*CA*
   CF*L^2 + 
  1.630556870634305326372486712399638562482573563836956552606805`50.*^-55*
   CF^2*L^2 - 
  1.314237832155465627682989658541965023475086707772805385501254`50.*^-55*CF*
   nf + 
  2.86589158808681105440145574838222823217377325638612024148822`50.*^-56*CF*L*
   nf - 6.1533383272320409423770202831497382505497684184312759505642933294710\
46001531839`50.*^-57*CF*L^2*nf - 
  4.90122583042889912051767623269431111813623697245546796489392`50.*^-56*CA*
   CF*irrational[Pi^2] - 2.03679214276543159352559389635350779994046513779615\
73252595284612680276357504184`50.*^-56*CF^2*irrational[Pi^2] - 
  6.9663757059856699861039378523310159762229542069076261884883515453371997484\
7885`50.*^-58*CA*CF*L*irrational[Pi^2] + 2.7865502823942679944415751409324063\
90489181682763050475395340618134879899391539`50.*^-57*CF^2*L*
   irrational[Pi^2] + 8.35965084718280398332472542279721917146754504828915142\
618602185440463969817462`50.*^-57*CA*CF*irrational[Zeta[3]] - 
  3.34386033887312159332989016911888766858701801931566057047441`50.*^-56*CF^2*
   irrational[Zeta[3]], 
 (2.64486459240989098328456880962670642907754878410394005557006`50.*^-56*I)*
   CA*CF + 
  (5.3212995750786841835444462606407878116155301068868754958466`50.*^-56*I)*
   CF^2 - (3.9786147744641581962983166684186679190597540580366933663689895661\
15506967625945`50.*^-57*I)*CA*CF*L - 
  (2.71935556585885668924836645592946559234655701676740978279518`50.*^-56*I)*
   CF^2*L + (7.39271249506787219818329669832387512214940871198867157151835479\
363483733750777`50.*^-58*I)*CA*CF*L^2 + 
  (3.578940249778812452855333810352494782024925960434529578477836435437173262\
148718`50.*^-57*I)*CF^2*L^2 - (2.89134017526606844128392353137661544087521774\
9458926883543609395444210542629567`50.*^-57*I)*CF*nf + 
  (6.312414395161833598479326858318244894146586335306735394493963235023127605\
81471`50.*^-58*I)*CF*L*nf - (1.3441295445577949451242357633316136585726197658\
1612210391242814429724315227415`50.*^-58*I)*CF*L^2*nf - 
  (1.076269438268896975462651441758116944331648140887121379621142777240472928\
190497`50.*^-57*I)*CA*CF*irrational[Pi^2] - 
  (4.453083091965940331910178640807959845456419280378383162603686086849845139\
93415`50.*^-58*I)*CF^2*irrational[Pi^2] - 
  (1.514429501301232605674769098332829560048468305849483954019206857681999945\
3214`50.*^-59*I)*CA*CF*L*irrational[Pi^2] + 
  (6.057718005204930422699076393331318240193873223397935816076827430727999781\
286`50.*^-59*I)*CF^2*L*irrational[Pi^2] + 
  (1.817315401561479126809722917999395472058161967019380744823048229218399934\
38579`50.*^-58*I)*CA*CF*irrational[Zeta[3]] - 
  (7.269261606245916507238891671997581888232647868077522979292192916873599737\
54315`50.*^-58*I)*CF^2*irrational[Zeta[3]], 
 -5.6921207445077015431813223319672667021834404372952252484945452524512288314\
3161`50.*^-58*CA*CF - 1.15431225771384901816648506925586146323488159045408647\
2869156271577592101655027`50.*^-57*CF^2 + 8.567795305628832208683313964391559\
4403411300427227669639102432323143233143949`50.*^-59*CA*CF*L + 
  5.8707930356419856030780184352040197144473191861012468441264981548996744264\
1735`50.*^-58*CF^2*L - 1.5803049448739400739087554720144730561506866520319253\
685737368660513705513986`50.*^-59*CA*CF*L^2 - 7.68646175428726288086165531199\
88110425166038736738614530940443252826146298393`50.*^-59*CF^2*L^2 + 
  6.2239507820276240634377326106601278008745139667570803608577431341317940170\
96`50.*^-59*CF*nf - 1.3602997392369265674282496765638113870964814610085270213\
442522863253056282411`50.*^-59*CF*L*nf + 
  2.8732817179526183161977372218444964657285211855125915792249761200934010025\
43`50.*^-60*CF*L^2*nf + 2.312517002024590467469629833831152830028921009920646\
0816756917196465964653578`50.*^-59*CA*CF*irrational[Pi^2] + 
  9.5273211693814506838894208451865845578443272566653696172029501402770245806\
26`50.*^-60*CF^2*irrational[Pi^2] + 
  3.2221904283004949056909980815592118298903580975520935191898018248553190326`\
50.*^-61*CA*CF*L*irrational[Pi^2] - 
  1.2888761713201979622763992326236847319561432390208374076759207299421276130\
4`50.*^-60*CF^2*L*irrational[Pi^2] - 
  3.8666285139605938868291976978710541958684297170625122230277621898263828391\
19`50.*^-60*CA*CF*irrational[Zeta[3]] + 1.54665140558423755473167907914842167\
83473718868250048892111048759305531356475`50.*^-59*CF^2*irrational[Zeta[3]], 
 (-1.199180001494118844101994494536056663253020349347351197309966242918172604\
1669`50.*^-59*I)*CA*CF - (2.4506148282869464619230360834070912968457697376844\
801035207599192759389855936`50.*^-59*I)*CF^2 + 
  (1.806023087025625132350768353765666947270923500842997085161408102206257140\
633`50.*^-60*I)*CA*CF*L + (1.240580449286536360702391388055596705322838230058\
9041672321277296282792360691`50.*^-59*I)*CF^2*L - 
  (3.307378015717010282050944108068003026497184891512523149865799922186857198\
74`50.*^-61*I)*CA*CF*L^2 - 
  (1.616045486047392564711269783139001222014311170140192621624228620854934112\
12`50.*^-60*I)*CF^2*L^2 + 
  (1.311524794118782071765654494000548948465859295392158812827642926714844070\
172`50.*^-60*I)*CF*nf - 
  (2.869336309204646150656067165103471431234148300848182434614457593186394462\
48`50.*^-61*I)*CF*L*nf + 
  (6.013414574030927785547171105578187320903972530022769363392363494885194906\
7`50.*^-62*I)*CF*L^2*nf + 
  (4.864054028637896662527711663260435693737083964399283572047265910803295336\
16`50.*^-61*I)*CA*CF*irrational[Pi^2] + 
  (1.995612374258069808890155263632147420404743107253406498703139400510764090\
12`50.*^-61*I)*CF^2*irrational[Pi^2] + 
  (
    6.712896725626031053522912669915024645604912703233528164978753801781914651`\
50.*^-63*I)*CA*CF*L*irrational[Pi^2] - 
  (2.685158690250412421409165067966009858241965081293411265991501520712765860\
5`50.*^-62*I)*CF^2*L*irrational[Pi^2] - 
  (8.055476070751237264227495203898029574725895243880233797974504562138297581\
5`50.*^-62*I)*CA*CF*irrational[Zeta[3]] + 
  (3.222190428300494905690998081559211829890358097552093519189801824855319032\
6`50.*^-61*I)*CF^2*irrational[Zeta[3]], 
 2.4741538349064798200699013205793321828663303871483873865299428911342959935`\
50.*^-61*CA*CF + 
  5.0941558276904322852606063411424272280250299211283437144085990177673269903\
6`50.*^-61*CF^2 - 
  3.7281189202519025540475457681681310812616036156168046189808218428834775398`\
50.*^-62*CA*CF*L - 
  2.5671206824102502384630576382393876665723611553001652353359399585327934534`\
50.*^-61*CF^2*L + 
  6.779902649441614903626499861778566282649624799926158019470659407807822451`\
50.*^-63*CA*CF*L^2 + 
  3.327583069204927114180571732301705440784932141212131265166014898768564585`\
50.*^-62*CF^2*L^2 - 
  2.7065964240222890520625737890960855017454261851879075390782641346569231601`\
50.*^-62*CF*nf + 
  5.926956332267048989292992969154516257555492211697865427209965071387291894`\
50.*^-63*CF*L*nf - 
  1.232709572625748164295727247596102960481749963622937821721938074146876809`\
50.*^-63*CF*L^2*nf - 
  1.0019700701675722907596185367729551663599603525349497083439435811284108178`\
50.*^-62*CA*CF*irrational[Pi^2] - 
  4.094194184310672303135667192545980224080640225824317234256134635877369789`\
50.*^-63*CF^2*irrational[Pi^2] - 
  1.36997892359714919459651278977857645828671687821092411530178649015957442`5\
0.*^-64*CA*CF*L*irrational[Pi^2] + 
  5.47991569438859677838605115911430583314686751284369646120714596063829767`5\
0.*^-64*CF^2*L*irrational[Pi^2] + 
  1.643974708316579033515815347734291749944060253853108938362143788191489302`\
50.*^-63*CA*CF*irrational[Zeta[3]] - 
  6.575898833266316134063261390937166999776241015412435753448575152765957209`\
50.*^-63*CF^2*irrational[Zeta[3]], 
 (
    5.001358409076118023114680909859997272925865408553270288773119979244738938`\
50.*^-63*I)*CA*CF + 
  (1.037297867033888343237610665940434072976907305869060364311608407779078562\
5`50.*^-62*I)*CF^2 - 
  (
    7.5397267539594242601941140839681683521897783910029979135546811595568635`\
50.*^-64*I)*CA*CF*L - 
  (
    5.204134831252758125145568500383176717786562080800984515510545473404607229`\
50.*^-63*I)*CF^2*L + 
  (
    1.36189251585861529378813569293314234416914686897504951488401112941525311`\
50.*^-64*I)*CA*CF*L^2 + 
  (
    6.71332482036779570472485754247602555386454372156145455986672292770208764`\
50.*^-64*I)*CF^2*L^2 - 
  (
    5.47258466887467603070493358935808580212988773175182828512075069986795175`\
50.*^-64*I)*CF*nf + 
  (
    1.19942482995294283725822426909283811932334790450048161681417571086432931`\
50.*^-64*I)*CF*L*nf - 
  (
    2.4761682106520278068875194416966224439439033981364536634254747807550057`\
50.*^-65*I)*CF*L^2*nf - 
  (
    2.02227174328758182758967460371888477038775161105988166239736555188500239`\
50.*^-64*I)*CA*CF*irrational[Pi^2] - 
  (
    8.2305892868715998958302841491707129978719876780973262731903028225053155`\
50.*^-65*I)*CF^2*irrational[Pi^2] - 
  (
    2.739957847194298389193025579557152916573433756421848230603572980319148`50.\
*^-66*I)*CA*CF*L*irrational[Pi^2] + 
  (
    1.0959831388777193556772102318228611666293735025687392922414291921276595`\
50.*^-65*I)*CF^2*L*irrational[Pi^2] + 
  (
    3.2879494166331580670316306954685834998881205077062178767242875763829786`\
50.*^-65*I)*CA*CF*irrational[Zeta[3]] - 
  (
    1.31517976665326322681265227818743339995524820308248715068971503055319144`\
50.*^-64*I)*CF^2*irrational[Zeta[3]], 
 -9.9093545884116013319257585029772609770850113005019235085517126362859408`50.\
*^-65*CA*CF - 
  2.06991257538686552532064901063756260933197087443986572293944533082842469`5\
0.*^-64*CF^2 + 
  1.4945154654732381461217910662112648822917864832810901107287507081242072`50.\
*^-65*CA*CF*L + 
  1.03397921132574063369134934420314945171671707793937178424052779438879763`5\
0.*^-64*CF^2*L - 
  2.681746519300841132144759188638151270536008667150001676140914249422831`50.\
*^-66*CA*CF*L^2 - 
  1.3275705862318012356627694596089652408141703350516391693867577010877701`50.\
*^-65*CF^2*L^2 + 
  1.0845794718949397190912910603372584603494561185036420115791030681284416`50.\
*^-65*CF*nf - 
  2.378950271876893511119685651062946326625650575095766447430395861342282`50.\
*^-66*CF*L*nf + 
  4.87590276236516569480865307025118412824728848572727577480166227167788`50.*^\
-67*CF*L^2*nf + 
  4.000651065418306911622657136064400378634521774724863868262782710582053`50.\
*^-66*CA*CF*irrational[Pi^2] + 
  1.62195948889302807024502785995651109588390838234994113945510075665617`50.*^\
-66*CF^2*irrational[Pi^2] + 
  5.3724663670476439003784815285434370913204583459251926090266136869004`50.*^\
-68*CA*CF*L*irrational[Pi^2] - 
  2.14898654681905756015139261141737483652818333837007704361064547476011`50.*^\
-67*CF^2*L*irrational[Pi^2] - 
  6.44695964045717268045417783425212450958455001511023113083193642428034`50.*^\
-67*CA*CF*irrational[Zeta[3]] + 
  2.57878385618286907218167113370084980383382000604409245233277456971214`50.*^\
-66*CF^2*irrational[Zeta[3]], 
 (
    -1.925179305338479999911776521245046560767802955196588535774156467718609`50.\
*^-66*I)*CA*CF - 
  (
    4.049408402387686557522323501372223103548594357959782078701443924908691`50.\
*^-66*I)*CF^2 + 
  (
    2.9046687719672864172461324824356679103554267126958249351578606963218`50.*^\
-67*I)*CA*CF*L + 
  (
    2.014229966877330427365570866826464914410388200917100266088792680082102`50.\
*^-66*I)*CF^2*L - 
  (
    5.1786555617991519169143726365654017408417643337127085932461595785215`50.*^\
-68*I)*CA*CF*L^2 - 
  (
    2.5743024327903811048946206321496271732018970704549387781424060007772`50.*^\
-67*I)*CF^2*L^2 + 
  (
    2.10766267217846229966264559728437121199402752801945388112901508402433`50.\
*^-67*I)*CF*nf - 
  (
    4.6263825760601839879846172113476171489702681943358916905232866016465`50.*^\
-68*I)*CF*L*nf + 
  (
    9.415737385089367121662495702846184983348662424932197442265744688221`50.*^\
-69*I)*CF*L^2*nf + 
  (
    7.7606707739882637546468506713068593923789664494267092145197495295559`50.*^\
-68*I)*CA*CF*irrational[Pi^2] + 
  (
    3.1344750906668739606068673682209317345011611224383332298903384991038`50.*^\
-68*I)*CF^2*irrational[Pi^2] + 
  (
    1.033166609047623826995861832412199440638549681908690886351271862865`50.*^\
-69*I)*CA*CF*L*irrational[Pi^2] - 
  (
    4.132666436190495307983447329648797762554198727634763545405087451462`50.*^\
-69*I)*CF^2*L*irrational[Pi^2] - 
  (
    1.2397999308571485923950341988946393287662596182904290636215262354386`50.*^\
-68*I)*CA*CF*irrational[Zeta[3]] + 
  (
    4.9591997234285943695801367955785573150650384731617162544861049417541`50.*^\
-68*I)*CF^2*irrational[Zeta[3]], 
 3.6688423369196381564323740716343187150840661688605746500406375665538`50.*^-\
68*CA*CF + 
  7.7694658425369944205190826149287719612554996823919829180522731936275`50.*^\
-68*CF^2 - 
  5.537451582525448656339266350232467202678044841766443785234171374453`50.*^-\
69*CA*CF*L - 
  3.8486331361216937430349136404155279661377041508494847025876267876247`50.*^\
-68*CF^2*L + 
  9.81077126070226006869410041000254423853695775518814316836261414289`50.*^-70\
*CA*CF*L^2 + 
  4.896747203705075103487391007135174172794864745261328082224069927284`50.*^-\
69*CF^2*L^2 - 
  4.017686109104965544145736198616722424939431663972509532082618585166`50.*^-\
69*CF*nf + 
  8.82485680900769350992165018320895262589298905331137709091992956239`50.*^-70\
*CF*L*nf - 
  1.78377659285495637612620007454591713427944686457966239424774802598`50.*^-70\
*CF*L^2*nf - 
  1.476759062545557561262762559077550356697310855111424156682873036753`50.*^-\
69*CA*CF*irrational[Pi^2] - 
  5.94248782566813420337850797388568609893200810234022801979982990665`50.*^-70\
*CF^2*irrational[Pi^2] - 
  1.9493709604672147679167204385135838502614144941673412950023997413`50.*^-71*
   CA*CF*L*irrational[Pi^2] + 
  7.797483841868859071666881754054335401045657976669365180009598965`50.*^-71*
   CF^2*L*irrational[Pi^2] + 
  2.3392451525606577215000645262163006203136973930008095540028796895`50.*^-70*
   CA*CF*irrational[Zeta[3]] - 
  9.35698061024263088600025810486520248125478957200323821601151875802`50.*^-70\
*CF^2*irrational[Zeta[3]], 
 (
    6.86085632772226723048679950417896563334281410598778249339541756653`50.*^-70\
*I)*CA*CF + 
  (
    1.462552184801070767384201777091764911934170537059411836396655912736`50.*^\
-69*I)*CF^2 - 
  (
    1.03585697873352916383626609182620386112273852532637285548958216749`50.*^\
-70*I)*CA*CF*L - 
  (
    7.2154610619974297687053694112542900671776554985512410898676706821`50.*^-70\
*I)*CF^2*L + 
  (1.824031772699386447995659491131305457590913177823465920137430822`50.*^-71*
    I)*CA*CF*L^2 + 
  (
    9.1402892912280893556933999458342128777121535880626991937758523808`50.*^-71\
*I)*CF^2*L^2 - 
  (
    7.5152634373227171008023736995484484692063328878276829331295347917`50.*^-71\
*I)*CF*nf + 
  (
    1.6517468166586194089459239826356790092359955128295414562127269973`50.*^-71\
*I)*CF*L*nf - 
  (3.316421404907975359992108165693282650165296686951756218431692404`50.*^-72*
    I)*CF*L^2*nf - 
  (
    2.7575285393056294256086051354396311230133466183039031489992355824`50.*^-71\
*I)*CA*CF*irrational[Pi^2] - 
  (1.105622800870193044476662114583844967974244496518005497003803873`50.*^-71*
    I)*CF^2*irrational[Pi^2] - 
  (3.60994622308743475540133414539552564863224906327285425000444396`50.*^-73*
    I)*CA*CF*L*irrational[Pi^2] + 
  (1.443978489234973902160533658158210259452899625309141700001777586`50.*^-72*
    I)*CF^2*L*irrational[Pi^2] + 
  (4.331935467704921706481600974474630778358698875927425100005332758`50.*^-72*
    I)*CA*CF*irrational[Zeta[3]] - 
  (
    1.7327741870819686825926403897898523113434795503709700400021331033`50.*^-71\
*I)*CF^2*irrational[Zeta[3]], 
 -1.2594200421836699664619581831613288202867001115958010629650944917`50.*^-71*
   CA*CF - 
  2.7021442482722262159611054160770180054775209088259987640054453961`50.*^-71*
   CF^2 + 
  1.902039861126562907523923828858197040578481820999580225201634748`50.*^-72*
   CA*CF*L + 
  1.3278092194490386446335509527835648454964658414195102574119012226`50.*^-71*
   CF^2*L - 
  3.32931818248327975210071899262420127449214874102150293855929999`50.*^-73*
   CA*CF*L^2 - 
  1.674821155756787374328846038724646938175791890094618731631851214`50.*^-72*
   CF^2*L^2 + 
  1.379932945205804418832409527064964917994909917268088048120293134`50.*^-72*
   CF*nf - 
  3.0346089189023526269250573940697392757176203466433583327810099`50.*^-73*CF*
   L*nf + 
  6.0533057863332359129103981684076386808948158927663689791987273`50.*^-74*CF*
   L^2*nf + 
  5.05455162637736943240612022517584874208010049975903858921908899`50.*^-73*
   CA*CF*irrational[Pi^2] + 
  2.01944413530376020245645002147396839754722611744803260778151282`50.*^-73*
   CF^2*irrational[Pi^2] + 
  6.563538587431699555275152991628228452058634660496098636371716`50.*^-75*CA*
   CF*L*irrational[Pi^2] - 
  2.6254154349726798221100611966512913808234538641984394545486865`50.*^-74*
   CF^2*L*irrational[Pi^2] - 
  7.8762463049180394663301835899538741424703615925953183636460595`50.*^-74*CA*
   CF*irrational[Zeta[3]] + 
  3.15049852196721578653207343598154965698814463703812734545842382`50.*^-73*
   CF^2*irrational[Zeta[3]], 
 (-2.27014550839212122250037178831806168582101413192790105458145453`50.*^-73*
    I)*CA*CF - 
  (4.90152843730267407069204996811227077245157585785562242483604594`50.*^-73*
    I)*CF^2 + 
  (3.4293924921880752961702316815286215148769855575680876371463374`50.*^-74*
    I)*CA*CF*L + 
  (2.39921708555862515618722638667545478154340407669735104304595794`50.*^-73*
    I)*CF^2*L - 
  (5.967836714708441123677598575662448722260350737904178441068492`50.*^-75*I)*
   CA*CF*L^2 - 
  (3.0135591749808347481500127544268928536530680267702747392874598`50.*^-74*
    I)*CF^2*L^2 + 
  (2.4880783040951966605474208338854529587512790176097742771536895`50.*^-74*
    I)*CF*nf - 
  (5.47436203703647414710396354707031215712075839817186330321571`50.*^-75*I)*
   CF*L*nf + (1.0850612208560802043050179228477179495018819523462142620124530\
442946627173961347`50.*^-75*I)*CF*L^2*nf + 
  (9.097964718845027327621298414851580524549630787821350436719355`50.*^-75*I)*
   CA*CF*irrational[Pi^2] + 
  (3.622331271704743481101780877919329347749543281287108257247759`50.*^-75*I)*
   CF^2*irrational[Pi^2] + (1.17206046204137492058484874850504079501047047508\
8589042209235053664952238042635`50.*^-76*I)*CA*CF*L*irrational[Pi^2] - 
  (4.688241848165499682339394994020163180041881900354356168836940214659808952\
170542`50.*^-76*I)*CF^2*L*irrational[Pi^2] - 
  (1.406472554449649904701818498206048954012564570106306850651082`50.*^-75*I)*
   CA*CF*irrational[Zeta[3]] + 
  (5.625890217798599618807273992824195816050258280425227402604328`50.*^-75*I)*
   CF^2*irrational[Zeta[3]], 
 4.019466761756792816864886368016556349834375649341552841412007`50.*^-75*CA*
   CF + 
  8.732235223783697508511104837841599278613886585291170628415182`50.*^-75*
   CF^2 - 6.07344351040415198822512861615828042566168728935173042016688528138\
1411438250399`50.*^-76*CA*CF*L - 
  4.258028747804393244751293147111375773561191317491005405146632`50.*^-75*
   CF^2*L + 1.050889834631919454688069724718815002044082797203958666719161808\
797600122403195`50.*^-76*CA*CF*L^2 + 5.32641618829759174099724100038701499495\
9605655739405356073538492458671419745441`50.*^-76*CF^2*L^2 - 
  4.4066023306312320950649021672981304076807834233749069578682892779764169521\
70466`50.*^-76*CF*nf + 9.7001528368838872385081308774835491435843553380669702\
4029633778078083406567059`50.*^-77*CF*L*nf - 1.910708790239853553978308590397\
84545826196872218901575767120328872290931346035`50.*^-77*CF*L^2*nf - 
  1.6085934479264171948656119697647909431551953936008474193719666608108270465\
34852`50.*^-76*CA*CF*irrational[Pi^2] - 6.38287348987846001371593843889562921\
800525999939648691284712107159644239855977`50.*^-77*CF^2*irrational[Pi^2] - 
  2.0562464246339910887453486815877908684394218861203316529986579888858811193\
73`50.*^-78*CA*CF*L*irrational[Pi^2] + 8.224985698535964354981394726351163473\
7576875444813266119946319555435244774922`50.*^-78*CF^2*L*irrational[Pi^2] + 
  2.4674957095607893064944184179053490421273062633443979835983895866630573432\
4765`50.*^-77*CA*CF*irrational[Zeta[3]] - 9.869982838243157225977673671621396\
16850922505337759193439355834665222937299062`50.*^-77*CF^2*
   irrational[Zeta[3]], (6.99281965793028216776292985228893256346327350542956\
251663260926116451617764319`50.*^-77*I)*CA*CF + 
  (1.528370432716029800705902298419443780226111841531581961268954316643990324\
187915`50.*^-76*I)*CF^2 - (1.056842918563967718735265306983556568138011735449\
89700202010986552735145895517`50.*^-77*I)*CA*CF*L - 
  (7.424900728480186433889923215710589028476694164900847474154850150188353633\
12561`50.*^-77*I)*CF^2*L + (1.81849071730824133198594924443370044086879705821\
97270672862883397560036635096`50.*^-78*I)*CA*CF*L^2 + 
  (9.250620956252777494318643437540541102652833835356186200115422724380429511\
1745`50.*^-78*I)*CF^2*L^2 - (7.6685618783322264793156881347347261361846556673\
919853736389467423230085814239`50.*^-78*I)*CF*nf + 
  (1.688789780667490660629830887331039468701622522375822955268984350146095209\
9563`50.*^-78*I)*CF*L*nf - 
  (3.306346758742256967247180444424909892488721924035867395065978799556370297\
29`50.*^-79*I)*CF*L^2*nf - (2.79463615075162767845791492207742150938982659344\
82181401671654323910110668384`50.*^-78*I)*CA*CF*irrational[Pi^2] - 
  (1.105226440763908648359532656570994444853472468852855302825319730146105596\
0583`50.*^-78*I)*CF^2*irrational[Pi^2] - 
  (3.545252456265501877147152899289294600757623941586778712066651704975657102\
36`50.*^-80*I)*CA*CF*L*irrational[Pi^2] + 
  (1.418100982506200750858861159715717840303049576634711484826660681990262840\
947`50.*^-79*I)*CF^2*L*irrational[Pi^2] + 
  (4.254302947518602252576583479147153520909148729904134454479982045970788522\
841`50.*^-79*I)*CA*CF*irrational[Zeta[3]] - 
  (1.701721179007440901030633391658861408363659491961653781791992818388315409\
1363`50.*^-78*I)*CF^2*irrational[Zeta[3]], 
 -1.1957393964921134888154739037095271321423076294914055970562435131035486866\
215`50.*^-78*CA*CF - 2.628912371141413773269187450843469987038955480115875858\
5511826140457525781976`50.*^-78*CF^2 + 
  1.8074910735442531158505141937456399032122682169539804393435283250407186627\
05`50.*^-79*CA*CF*L + 1.27247357879181602446236960363754499979264311329544235\
61072692942681420466684`50.*^-78*CF^2*L - 
  3.0932070385859126905339065653134332187621801397503404687097600727295701357`\
50.*^-80*CA*CF*L^2 - 
  1.5791329670994230022487391079517032956923865031555170204183729512221836486\
39`50.*^-79*CF^2*L^2 + 
  1.3116743479337513617942901020691176002527335049592533877231266563848864599\
09`50.*^-79*CF*nf - 
  2.8897311392238789139694007563481950900495911347915805962791387349020294966\
8`50.*^-80*CF*L*nf + 
  5.6240127974289321646071028460244240341130547995460735794722910413264911558`\
50.*^-81*CF*L^2*nf + 
  4.7721371931957522151627240816280980696821143767276962018426502446198558583\
4`50.*^-80*CA*CF*irrational[Pi^2] + 
  1.8811522930954873076563694449073963132758177677271369617852008107160117252\
1`50.*^-80*CF^2*irrational[Pi^2] + 
  6.00890246824661335109686932082931288264004057896064188485873170334857136`5\
0.*^-82*CA*CF*L*irrational[Pi^2] - 
  2.403560987298645340438747728331725153056016231584256753943492681339428544`\
50.*^-81*CF^2*L*irrational[Pi^2] - 
  7.2106829618959360213162431849951754591680486947527702618304780440182856319`\
50.*^-81*CA*CF*irrational[Zeta[3]] + 
  2.8842731847583744085264972739980701836672194779011081047321912176073142527\
7`50.*^-80*CF^2*irrational[Zeta[3]], 
 (
    -2.0102463125104720636784289267566461922948131458656485059651972510242305\
3108`50.*^-80*I)*CA*CF - 
  (4.445256818153331054401153946328561426821972260944470352352739975294253463\
26`50.*^-80*I)*CF^2 + 
  (3.039206781277184427326729155965242510796928074630997516354205175154184269\
9`50.*^-81*I)*CA*CF*L + 
  (2.143934160581199879799011442789274414389070212920384043960399995748265279\
61`50.*^-80*I)*CF^2*L - 
  (
    5.173409461963051068267021691804989365249921501862048588999869874678973933`\
50.*^-82*I)*CA*CF*L^2 - 
  (2.650364936156007464315891733898204517117449651666473711789599620651330236\
7`50.*^-81*I)*CF^2*L^2 + 
  (2.205806761963396967691243267176085999563838943932539891109676334444315489\
7`50.*^-81*I)*CF*nf - 
  (
    4.861300173308314828409499592192755261507696522866110342270916083159241535`\
50.*^-82*I)*CF*L*nf + 
  (
    9.40619902175100194230367580328179884590894818520372470727249068123449806`\
50.*^-83*I)*CF*L^2*nf + 
  (
    8.01191854686144143000024938903102360981764381731911143095663236442106683`\
50.*^-82*I)*CA*CF*irrational[Pi^2] + 
  (
    3.14818644857518746434916865534329794070463413783174366376524228083650452`\
50.*^-82*I)*CF^2*irrational[Pi^2] + 
  (
    1.00148374470776889184947822013821881377334009649344031414312195055809522`\
50.*^-83*I)*CA*CF*L*irrational[Pi^2] - 
  (
    4.00593497883107556739791288055287525509336038597376125657248780223238091`\
50.*^-83*I)*CF^2*L*irrational[Pi^2] - 
  (
    1.201780493649322670219373864165862576528008115792128376971746340669714272`\
50.*^-82*I)*CA*CF*irrational[Zeta[3]] + 
  (
    4.807121974597290680877495456663450306112032463168513507886985362678857088`\
50.*^-82*I)*CF^2*irrational[Zeta[3]], 
 3.32363275333299673077387556167610250938088228789757138316873617076888736`50.\
*^-82*CA*CF + 
  7.391231078712292525664530042301018478462344930653191306199742636620502358`\
50.*^-82*CF^2 - 
  5.02558350435111790001414053590069088353795274205591544817130488527523781`5\
0.*^-83*CA*CF*L - 
  3.552244329323697326642980934853925863873220342629883292520682360353481374`\
50.*^-82*CF^2*L + 
  8.5101349926044266534317446565482058730392453497466994949092285507050754`50.\
*^-84*CA*CF*L^2 + 
  4.37476475417969435351495932102698092904406123645129002790915627310130513`5\
0.*^-83*CF^2*L^2 - 
  3.64805433570215709304315392572348539184197204047198280418664764408700066`5\
0.*^-83*CF*nf + 
  8.0423801410528643639878741245712515781072994137970626253727931684106101`50.\
*^-84*CF*L*nf - 
  1.5472972713826230278966808466451283405525900635903089990744051910372865`50.\
*^-84*CF*L^2*nf - 
  1.32287585416251263386450531455984450120655019783452938337826232727713756`5\
0.*^-83*CA*CF*irrational[Pi^2] - 
  5.1818257245129102870707868165633054619907199548033548639617297820159722`50.\
*^-84*CF^2*irrational[Pi^2] - 
  1.641776630668473593195865934652817727497278846710557892037904836980484`50.\
*^-85*CA*CF*L*irrational[Pi^2] + 
  6.567106522673894372783463738611270909989115386842231568151619347921936`50.\
*^-85*CF^2*L*irrational[Pi^2] + 
  1.9701319568021683118350391215833812729967346160526694704454858043765808`50.\
*^-84*CA*CF*irrational[Zeta[3]] - 
  7.8805278272086732473401564863335250919869384642106778817819432175063231`50.\
*^-84*CF^2*irrational[Zeta[3]], 
 (
    5.4056463858915364274122163950409118735161285641595194874415823394100223`50.\
*^-84*I)*CA*CF + 
  (
    1.20880535824572828731872443857981224655379806691654756289289724496696351`\
50.*^-83*I)*CF^2 - 
  (
    8.174751992201386863615834658909352421412346853166385350332778111196943`50.\
*^-85*I)*CA*CF*L - 
  (
    5.7895257299213587150661300412568810812108887629636290635345442431155641`\
50.*^-84*I)*CF^2*L + 
  (
    1.377227122266831839426120102206958944651375803682359897637472590985972`50.\
*^-85*I)*CA*CF*L^2 + 
  (
    7.103700280123136973241806717468751247200993012419323552910624691062444`50.\
*^-85*I)*CF^2*L^2 - 
  (
    5.93507954854708323008487207864814146259701308583214381599617835486415`50.\
*^-85*I)*CF*nf + 
  (
    1.308801578494179161701700302974892552945984438015489751673575590819826`50.\
*^-85*I)*CF*L*nf - 
  (
    2.50404931321242152622930927673992535391159237033156345024995016542904`50.\
*^-86*I)*CF*L^2*nf - 
  (
    2.148718845761589161316693776218084518817812541248700991964408450726167`50.\
*^-85*I)*CA*CF*irrational[Pi^2] - 
  (
    8.39090840237757259341721662618298494577365644269483554850641635280503`50.\
*^-86*I)*CF^2*irrational[Pi^2] - 
  (
    2.6480268236588283761223644107303511733827078172750933742546852209362`50.*^\
-87*I)*CA*CF*L*irrational[Pi^2] + 
  (
    1.05921072946353135044894576429214046935308312691003734970187408837451`50.\
*^-86*I)*CF^2*L*irrational[Pi^2] + 
  (
    3.17763218839059405134683729287642140805924938073011204910562226512352`50.\
*^-86*I)*CA*CF*irrational[Zeta[3]] - 
  (
    1.271052875356237620538734917150568563223699752292044819642248906049407`50.\
*^-85*I)*CF^2*irrational[Zeta[3]], 
 -8.65102810127910146175658664147238571917875044301405458856681381171755`50.*^\
-86*CA*CF - 
  1.945061675510005422079405618142131273643854845813453357923012811059216`50.\
*^-85*CF^2 + 
  1.30839936666817279373424484643769306795574296234426119615013064602829`50.*^\
-86*CA*CF*L + 
  9.2842766295143027597408970804171468453147537754660370760053929362872`50.*^\
-86*CF^2*L - 
  2.1933008409485956680496398100622278623206768529615599504545625691582`50.*^\
-87*CA*CF*L^2 - 
  1.13503814079018759138704534108774947355489738885521322771997879972671`50.*^\
-86*CF^2*L^2 + 
  9.5011980636733202993918635183809680406491466370060988094560086633625`50.*^\
-87*CF*nf - 
  2.0957335620247321920823522518747636066202007824809017265848214891827`50.*^\
-87*CF*L*nf + 
  3.987819710815628487362981472840414295128503369021018091735568307561`50.*^-\
88*CF*L^2*nf + 
  3.4342597677385156779304940765656888639875325247946826997387312631004`50.*^\
-87*CA*CF*irrational[Pi^2] + 
  1.3370672256452589011366356270409534625389077730427650169966321808062`50.*^\
-87*CF^2*irrational[Pi^2] + 
  4.20321718041083869225772128687357329108366320202395773691219876339`50.*^-89\
*CA*CF*L*irrational[Pi^2] - 
  1.681286872164335476903088514749429316433465280809583094764879505356`50.*^-\
88*CF^2*L*irrational[Pi^2] - 
  5.043860616493006430709265544248287949300395842428749284294638516069`50.*^-\
88*CA*CF*irrational[Zeta[3]] + 
  2.0175442465972025722837062176993151797201583369714997137178554064276`50.*^\
-87*CF^2*irrational[Zeta[3]], 
 (
    -1.362653845701066614509160648622238636285137925796835301773999202216`50.*^\
-87*I)*CA*CF - 
  (
    3.0800701121631743444390689755322232442486122571084791926962066820052`50.*^\
-87*I)*CF^2 + 
  (
    2.06108453437518777325101902364287308105225819439812765106761061585`50.*^\
-88*I)*CA*CF*L + 
  (
    1.4653133725868341925310119869465131172733878086224237077621945476343`50.*^\
-87*I)*CF^2*L - 
  (
    3.43814947140107333040783368286280648506813270108461341757627342022`50.*^\
-89*I)*CA*CF*L^2 - 
  (
    1.785021806562661694032258364369947587522408687866472329072035554409`50.*^\
-88*I)*CF^2*L^2 + 
  (
    1.497022363811260825423568508171249950981916431923578163967422876533`50.*^\
-88*I)*CF*nf - 
  (
    3.30281041973459308086356428484806478066501958428010770773738436886`50.*^\
-89*I)*CF*L*nf + 
  (
    6.2511808570928606007415157870232845183056958201538425774114062186`50.*^-90\
*I)*CF*L^2*nf + 
  (
    5.40245550511475399234889309438414661753831742655827500905623558457`50.*^\
-89*I)*CA*CF*irrational[Pi^2] + 
  (
    2.09713374814661193212269621188360906408550294369592481783923786948`50.*^\
-89*I)*CF^2*irrational[Pi^2] + 
  (6.567526844391935456652689510739958267318223753162433963925310568`50.*^-91*
    I)*CA*CF*L*irrational[Pi^2] - 
  (
    2.6270107377567741826610758042959833069272895012649735855701242271`50.*^-90\
*I)*CF^2*L*irrational[Pi^2] - 
  (
    7.8810322132703225479832274128879499207818685037949207567103726814`50.*^-90\
*I)*CA*CF*irrational[Zeta[3]] + 
  (
    3.15241288530812901919329096515517996831274740151796830268414907254`50.*^\
-89*I)*CF^2*irrational[Zeta[3]], 
 2.11304440135823045148306083007330775709236001717599637714374095355`50.*^-89*
   CA*CF + 
  4.80118429473889387943543556365754472055629698351039303615927205516`50.*^-89\
*CF^2 - 
  3.196315092497063755539913919736982893027266371808828329378221455`50.*^-90*
   CA*CF*L - 
  2.27666536703099540748918980119852036114520531254564505353066007854`50.*^-89\
*CF^2*L + 
  5.306304404430613726164943642043802645762588790133869364699379493`50.*^-91*
   CA*CF*L^2 + 
  2.7637050775897605502880415139424177149994698601586585598664866569`50.*^-90*
   CF^2*L^2 - 
  2.3221181455309838627645371595897193676364611972593960769962205628`50.*^-90*
   CF*nf + 
  5.124190606884250800559666724798916381746847155349611496859330022`50.*^-91*
   CF*L*nf - 
  9.64782618987384313848171571280691390138652507297067157218068998`50.*^-92*
   CF*L^2*nf - 
  8.366844749279551409907497917267450065897989656429913584806569725`50.*^-91*
   CA*CF*irrational[Pi^2] - 
  3.238432314704432302960564299007861348757302785342133984562193599`50.*^-91*
   CF^2*irrational[Pi^2] - 
  1.01038874529106699333118300165230127189511134664037445598850932`50.*^-92*
   CA*CF*L*irrational[Pi^2] + 
  4.04155498116426797332473200660920508758044538656149782395403727`50.*^-92*
   CF^2*L*irrational[Pi^2] + 
  1.212466494349280391997419601982761526274133615968449347186211182`50.*^-91*
   CA*CF*irrational[Zeta[3]] - 
  4.849865977397121567989678407931046105096534463873797388744844727`50.*^-91*
   CF^2*irrational[Zeta[3]], 
 (3.226579093646647317433052099950796069172685075378831982997716594`50.*^-91*
    I)*CA*CF + 
  (7.368898210149837670090786537901537883274555151121348485154681802`50.*^-91*
    I)*CF^2 - 
  (4.8809781517821544582347457004894340150225328355071109557347114`50.*^-92*
    I)*CA*CF*L - 
  (3.483049508294443156236904986192276255587248874134802730820449088`50.*^-91*
    I)*CF^2*L + 
  (8.0649948068966895021190431226416440062122455154378684256256308`50.*^-93*
    I)*CA*CF*L^2 + 
  (4.21366005795069945081417418697762308563143548977471033654937629`50.*^-92*
    I)*CF^2*L^2 - 
  (3.54691786930382438391583091029731955804996061987594802258012301`50.*^-92*
    I)*CF*nf + 
  (7.8282793682025376977249619044770744446731191520164326393581533`50.*^-93*
    I)*CF*L*nf - 
  (1.4663626921630344549307351132075716374931355482614306228410238`50.*^-93*
    I)*CF*L^2*nf - 
  (1.27599599731800822923189007431098860688244516262161358727331102`50.*^-92*
    I)*CA*CF*irrational[Pi^2] - 
  (4.9247379875294450059050359263466353310149090595356292150369821`50.*^-93*
    I)*CF^2*irrational[Pi^2] - 
  (1.53089203831979847474421666917015344226532022218238553937653`50.*^-94*I)*
   CA*CF*L*irrational[Pi^2] + 
  (6.123568153279193898976866676680613769061280888729542157506117`50.*^-94*I)*
   CF^2*L*irrational[Pi^2] + 
  (1.8370704459837581696930600030041841307183842666188626472518351`50.*^-93*
    I)*CA*CF*irrational[Zeta[3]] - 
  (7.3482817839350326787722400120167365228735370664754505890073405`50.*^-93*
    I)*CF^2*irrational[Zeta[3]], 
 -4.8527471847738962420661789115636411809012908838910755659633874`50.*^-93*CA*
   CF - 
  1.11385007440536646070038333593268483526801145091314064408784583`50.*^-92*
   CF^2 + 
  7.341243392830856025365519333646959022239064446608605683567091`50.*^-94*CA*
   CF*L + 5.24824549067433540686456246416774455722105763223785171891`50.*^-93*
   CF^2*L - 
  1.207427551300916459048275939020867360736894920933570569282486`50.*^-94*CA*
   CF*L^2 - 
  6.327734910899368008113435162414642424946366726533278874629114`50.*^-94*
   CF^2*L^2 + 
  5.336177414792569910531348450167893429759489430072841162584182`50.*^-94*CF*
   nf - 
  1.177901305139390757078939934037208498922496256540041511262842`50.*^-94*CF*
   L*nf + 2.19532282054712083463322898003794065588526349260649194414997487923\
1714435385464`50.*^-95*CF*L^2*nf + 
  1.916705727434461318028931076295558409804705574833763963829707`50.*^-94*CA*
   CF*irrational[Pi^2] + 
  7.37686424367443054986326167550204995559340371104087006186869`50.*^-95*CF^2*
   irrational[Pi^2] + 2.28491349002954996230480099876142304815719436146624707\
369631234310902654632707`50.*^-96*CA*CF*L*irrational[Pi^2] - 
  9.1396539601181998492192039950456921926287774458649882947852493724361061853\
0829`50.*^-96*CF^2*L*irrational[Pi^2] - 2.74189618803545995476576119851370765\
7788633233759496488435574811730831855592486`50.*^-95*CA*CF*
   irrational[Zeta[3]] + 
  1.09675847521418398190630447940548306311545329350379859537423`50.*^-94*CF^2*
   irrational[Zeta[3]], 
 (-7.19024633126066929933750413476946732657488030066737651902336`50.*^-95*I)*
   CA*CF - 
  (1.658518956255006831205827169196297350731438172698472854920725`50.*^-94*I)*
   CF^2 + (1.0877692576219944242496007891523987252265711535604006340259143291\
15235124087417`50.*^-95*I)*CA*CF*L + 
  (7.79043831975532539655072177676634499964437316278377866960607`50.*^-95*I)*
   CF^2*L - (1.78098666509567678858245393886552392425949484949558969509206291\
538334957468048`50.*^-96*I)*CA*CF*L^2 - 
  (9.361735403065978115084339820678077116995376375541372936482467091917731367\
04524`50.*^-96*I)*CF^2*L^2 + (7.908974464125950200083231940428023870225399405\
62868165631432268697164020267626`50.*^-96*I)*CF*nf - 
  (1.746031601161547734400178573855088487195789121750101724961965280906507781\
08341`50.*^-96*I)*CF*L*nf + (3.2381575729012305246953707979373162259263542718\
101630819855689370606355903282`50.*^-97*I)*CF*L^2*nf + 
  (2.836472077164283660683652559279268858114979403765382572450491884974352716\
63753`50.*^-96*I)*CA*CF*irrational[Pi^2] + 
  (1.088675553950205016137527374781859822772650019037915728714660573320636838\
59857`50.*^-96*I)*CF^2*irrational[Pi^2] + 
  (3.360166897102279356330589704060916247289991708038598637788694622219156685\
775`50.*^-98*I)*CA*CF*L*irrational[Pi^2] - 
  (1.344066758840911742532235881624366498915996683215439455115477848887662674\
3101`50.*^-97*I)*CF^2*L*irrational[Pi^2] - 
  (4.032200276522735227596707644873099496747990049646318365346433546662988022\
9301`50.*^-97*I)*CA*CF*irrational[Zeta[3]] + 
  (1.612880110609094091038683057949239798699196019858527346138573418665195209\
17205`50.*^-96*I)*CF^2*irrational[Zeta[3]], 
 1.04979804008781592443305539205300251367728623185181944833045578448693003901\
179`50.*^-96*CA*CF + 2.433218581082670630606670741650689951076223635468101109\
85114872633600274675262`50.*^-96*CF^2 - 1.58819682695922030875114192867262050\
79860135533654157244758599596323602173695`50.*^-97*CA*CF*L - 
  1.1394602379638521442702061086739005214744145822963083101215830758163071264\
4597`50.*^-96*CF^2*L + 
  2.5887942104160293400040787345608748191885945974868550889613642450112909978\
2`50.*^-98*CA*CF*L^2 + 1.3648319319257163174427940146955844579594596692552639\
005608765002502061632964`50.*^-97*CF^2*L^2 - 1.155091657578373113917071487033\
9079293742755087413095033237724115861799384362`50.*^-97*CF*nf + 
  2.5503044632868124366970389844535322412399491979456965175516902446919176639\
81`50.*^-98*CF*L*nf - 
  4.7068985643927806181892340628379542167065356317942819799297531727478018142\
2`50.*^-99*CF*L^2*nf - 
  4.1363190200023382926924189360204026891328335637785373387133942534968227514\
2`50.*^-98*CA*CF*irrational[Pi^2] - 
  1.5832811428876778071783266198929287325324030720959223195836092727061243364\
27`50.*^-98*CF^2*irrational[Pi^2] - 
  4.8698070972496802265660720348708931120144807362878241127372385829263140374`\
50.*^-100*CA*CF*L*irrational[Pi^2] + 
  1.9479228388998720906264288139483572448057922945151296450948954331705256149\
4`50.*^-99*CF^2*L*irrational[Pi^2] + 
  5.8437685166996162718792864418450717344173768835453889352846862995115768448\
3`50.*^-99*CA*CF*irrational[Zeta[3]] - 
  2.3375074066798465087517145767380286937669507534181555741138745198046307379\
3`50.*^-98*CF^2*irrational[Zeta[3]], 
 (1.5106609397367417767588240658622501961655874383528428480415137605473185183\
05`50.*^-98*I)*CA*CF + 
  (3.518054220839676043404142907664851210808868819371022639102240243967400797\
415`50.*^-98*I)*CF^2 - 
  (2.285416921905038723595369705036299863629518847669503336037068989538172121\
64`50.*^-99*I)*CA*CF*L - 
  (1.642553201564889638552253150707043095589147089951451394827376834340189941\
286`50.*^-98*I)*CF^2*L + 
  (3.709057827076617878738672858497491713127933635454693184434737422956224813\
4`50.*^-100*I)*CA*CF*L^2 + 
  (1.961143469941661714829025513610301465925537576923217599520567644492153703\
72`50.*^-99*I)*CF^2*L^2 - 
  (1.662692293309801921401490702611744260044696218469264616296594696051598394\
51`50.*^-99*I)*CF*nf + 
  (3.671318081838573996953988286677599545469492546188507131689960496277546507\
8`50.*^-100*I)*CF*L*nf - 
  (
    6.743741503775668870433950651813621296596242973553987608063158950829499661`\
50.*^-101*I)*CF*L^2*nf - 
  (5.945039176371433784539201822391529918501356213878708790225893973288947292\
2`50.*^-100*I)*CA*CF*irrational[Pi^2] - 
  (2.269564594734466452400073448017231732798512648269433228482416844049938827\
3`50.*^-100*I)*CF^2*irrational[Pi^2] - 
  (
    6.95686728178525746652296004981556158859211533755403444676748368989473434`\
50.*^-102*I)*CA*CF*L*irrational[Pi^2] + 
  (
    2.782746912714102986609184019926224635436846135021613778706993475957893736`\
50.*^-101*I)*CF^2*L*irrational[Pi^2] + 
  (
    8.348240738142308959827552059778673906310538405064841336120980427873681207`\
50.*^-101*I)*CA*CF*irrational[Zeta[3]] - 
  (3.339296295256923583931020823911469562524215362025936534448392171149472482\
7`50.*^-100*I)*CF^2*irrational[Zeta[3]], 
 -2.1429755939871601244559261292653979545741734314888520472797723997508761559`\
50.*^-100*CA*CF - 
  5.0139097546533252432269669250492668792520137824458059183941748880799015162`\
50.*^-100*CF^2 + 
  3.241982230079786924417649077499860031570252310138892497002990762814509058`\
50.*^-101*CA*CF*L + 
  2.3340678339932268970905572297729711136631121395031564406340216650611851836`\
50.*^-100*CF^2*L - 
  5.23899778164526219374754499927635547331708200591726003694190990970102135`5\
0.*^-102*CA*CF*L^2 - 
  2.778030024977269234031465083275396036707765696575692741495019765698983809`\
50.*^-101*CF^2*L^2 + 
  2.359373130501837621330266487714527577314908310626947181986214780569888633`\
50.*^-101*CF*nf - 
  5.20993945135476653086254342078933536402531957880915277579634343359015078`5\
0.*^-102*CF*L*nf + 
  9.5254505120822948977228090895933735878492400107586546126216543812745843`50.\
*^-103*CF*L^2*nf + 
  8.42346278603972576117713682006302646211325963947187693843568901162844479`5\
0.*^-102*CA*CF*irrational[Pi^2] + 
  3.20731407744201449572000347372045599369093807549588483625757169214937821`5\
0.*^-102*CF^2*irrational[Pi^2] + 
  9.798404622232756995102760633543044490974810334583147108123216464640471`50.\
*^-104*CA*CF*L*irrational[Pi^2] - 
  3.9193618488931027980411042534172177963899241338332588432492865858561884`50.\
*^-103*CF^2*L*irrational[Pi^2] - 
  1.17580855466793083941233127602516533891697724014997765297478597575685651`5\
0.*^-102*CA*CF*irrational[Zeta[3]] + 
  4.70323421867172335764932510410066135566790896059991061189914390302742603`5\
0.*^-102*CF^2*irrational[Zeta[3]], 
 (
    -2.99739899680076179062535943909760847129608553673137277206587633978403937`\
50.*^-102*I)*CA*CF - 
  (
    7.04517070090087667913252829515403823671945952951785729207750543365741336`\
50.*^-102*I)*CF^2 + 
  (
    4.5344836181629919683681650957852058544950225830791008476272845904576506`\
50.*^-103*I)*CA*CF*L + 
  (
    3.27016340883933064928603996399210924335950074725274734075122433908193163`\
50.*^-102*I)*CF^2*L - 
  (
    7.296896211243140538183390401868475926211612824937923378614219799773238`50.\
*^-104*I)*CA*CF*L^2 - 
  (
    3.880157376774867850717969232062736699115055566284111689248722818637462`50.\
*^-103*I)*CF^2*L^2 + 
  (
    3.3010970049627500915678691873696913107599517484686241697552444407987365`\
50.*^-103*I)*CF*nf - 
  (
    7.289740631973868208238168799339019345134760325571172046010920550618334`50.\
*^-104*I)*CF*L*nf + 
  (
    1.326708402044207370578798254885177441129384149988713341566221781776953`50.\
*^-104*I)*CF*L^2*nf + 
  (
    1.1768182235149106814148553938943169702297994052283305756314575065579946`\
50.*^-103*I)*CA*CF*irrational[Pi^2] + 
  (
    4.469323378099428871139461007378687231084132073000694444703525842744021`50.\
*^-104*I)*CF^2*irrational[Pi^2] + 
  (
    1.36088953086566069376427231021431173485761254646988154279489117564451`50.\
*^-105*I)*CA*CF*L*irrational[Pi^2] - 
  (
    5.44355812346264277505708924085724693943045018587952617117956470257804`50.\
*^-105*I)*CF^2*L*irrational[Pi^2] - 
  (
    1.633067437038792832517126772257174081829135055763857851353869410773412`50.\
*^-104*I)*CA*CF*irrational[Zeta[3]] + 
  (
    6.532269748155171330068507089028696327316540223055431405415477643093647`50.\
*^-104*I)*CF^2*irrational[Zeta[3]], 
 4.134602563824053688635281448974449364827715891636957297890178251710922`50.*^\
-104*CA*CF + 
  9.761898303845354557281492810433584027422119218911029841266655218646992`50.\
*^-104*CF^2 - 
  6.25464321233841162112445137795249036867414635704212092581303139351346`50.*^\
-105*CA*CF*L - 
  4.518279737247660263080163391862741489455001786078292748391446119184285`50.\
*^-104*CF^2*L + 
  1.00234648562878987244702506327094140667357202421511925578273240871848`50.*^\
-105*CA*CF*L^2 + 
  5.34480182160889390666724535493449776634228694967598271294048853164307`50.*^\
-105*CF^2*L^2 - 
  4.55493330326530451773327983731738095570154782975120284081122403297401`50.*^\
-105*CF*nf + 
  1.00587915296334668412222659058590510845813132593971988544299969507699`50.*^\
-105*CF*L*nf - 
  1.8224481556887088589945910241289843757701309531183986468776952885791`50.*^\
-106*CF*L^2*nf - 
  1.62142168852640812052561761837416806074278747418873625193062253747168`50.*^\
-105*CA*CF*irrational[Pi^2] - 
  6.1422568873613686860428822955300918571350662384846007120303242652153`50.*^\
-106*CF^2*irrational[Pi^2] - 
  1.864232234062548895567496315362070869667962392424495264102590651568`50.*^-\
107*CA*CF*L*irrational[Pi^2] + 
  7.456928936250195582269985261448283478671849569697981056410362606271`50.*^-\
107*CF^2*L*irrational[Pi^2] + 
  2.2370786808750586746809955784344850436015548709093943169231087818814`50.*^\
-106*CA*CF*irrational[Zeta[3]] - 
  8.9483147235002346987239823137379401744062194836375772676924351275255`50.*^\
-106*CF^2*irrational[Zeta[3]], 
 (
    5.6255912396350157145061948238916685506698421742442968116975474433072`50.*^\
-106*I)*CA*CF + 
  (
    1.33409997321625349634486579851021886893113969743566464135725362803264`50.\
*^-105*I)*CF^2 - 
  (
    8.509770847951671114473504782585063872552916584682752863643593932289`50.*^\
-107*I)*CA*CF*L - 
  (
    6.1575481764695864121688220764417354368475164049594077569690753486006`50.*^\
-106*I)*CF^2*L + 
  (
    1.358217809558295113372828034398310223512871898889732416201542962474`50.*^\
-107*I)*CA*CF*L^2 + 
  (
    7.262170217981298735342108161090956529140316233368250750398106686123`50.*^\
-107*I)*CF^2*L^2 - 
  (
    6.199414365027917363349419117160584305049452983772415708751518546394`50.*^\
-107*I)*CF*nf + 
  (
    1.369043034500525633018384407988374731169049584681623863542546630414`50.*^\
-107*I)*CF*L*nf - 
  (
    2.46948692646962747885968733526965495184158527070860439309371447723`50.*^\
-108*I)*CF*L^2*nf - 
  (
    2.203602219222038246469047854481302856306660891135877566489147389903`50.*^\
-107*I)*CA*CF*irrational[Pi^2] - 
  (
    8.32687934641031759963567589508153440880346766166689532183382878799`50.*^\
-108*I)*CF^2*irrational[Pi^2] - 
  (
    2.5192327487331741831993193450838795536053545843574260325710684481`50.*^-\
109*I)*CA*CF*L*irrational[Pi^2] + 
  (
    1.00769309949326967327972773803355182144214183374297041302842737923`50.*^\
-108*I)*CF^2*L*irrational[Pi^2] + 
  (
    3.02307929847980901983918321410065546432642550122891123908528213768`50.*^\
-108*I)*CA*CF*irrational[Zeta[3]] - 
  (
    1.209231719391923607935673285640262185730570200491564495634112855071`50.*^\
-107*I)*CF^2*irrational[Zeta[3]], 
 -7.55140879881205648764034355475914602590580784239382288900741879811`50.*^-1\
08*CA*CF - 
  1.7986051155268143334322828799797389525848587810625168597188875272`50.*^-107\
*CF^2 + 
  1.14223292540061369158048653831213763985945422883440738617294464206`50.*^-1\
08*CA*CF*L + 
  8.27855726308658337625109907268358777907363125898401623303946208642`50.*^-1\
08*CF^2*L - 
  1.8158195984943292619681681289177818814095182638761172375633373138`50.*^-109\
*CA*CF*L^2 - 
  9.7349616338963513266942603615553778878523717883037508397871464177`50.*^-109\
*CF^2*L^2 + 
  8.3242440398951876390662226398378145851591784782613203945038056071`50.*^-109\
*CF*nf - 
  1.8382599265579467982663607303928514953483130011273507801595588402`50.*^-109\
*CF*L*nf + 
  3.301490179080598658123942052577785238926396843411122250115158753`50.*^-110*
   CF*L^2*nf + 
  2.9546195198079071376736624474245498790163559629799621404267676304`50.*^-109\
*CA*CF*irrational[Pi^2] + 
  1.1137422476475815196076803987742278739378373656258161035247030043`50.*^-109\
*CF^2*irrational[Pi^2] + 
  3.35897699831089891093242579344517273814047277914323471009475793`50.*^-111*
   CA*CF*L*irrational[Pi^2] - 
  1.343590799324359564372970317378069095256189111657293884037903172`50.*^-110*
   CF^2*L*irrational[Pi^2] - 
  4.030772397973078693118910952134207285768567334971881652113709517`50.*^-110*
   CA*CF*irrational[Zeta[3]] + 
  1.6123089591892314772475643808536829143074269339887526608454838068`50.*^-109\
*CF^2*irrational[Zeta[3]], 
 (
    -1.000212041180945603589934264879492805593787781771461423028532244`50.*^-109\
*I)*CA*CF - 
  (
    2.3925209260567246401312709263405761423384240730788550042466933854`50.*^-\
109*I)*CF^2 + 
  (
    1.512835348314622578119917706858709396013952720550954513551689028`50.*^-110\
*I)*CA*CF*L + 
  (
    1.0982280929498775935094467484841569640595657091172738997085093052`50.*^-\
109*I)*CF^2*L - 
  (2.39555124543870240667015109265019967817486905868158387098470377`50.*^-111*
    I)*CA*CF*L^2 - 
  (
    1.287696067803108820856655390827743504170261185452102003439013508`50.*^-110\
*I)*CF^2*L^2 + 
  (1.10291710788506923494178446608099791441454914442013176324134426`50.*^-110*
    I)*CF*nf - 
  (2.43553322673154568030570956857606957219596163601768770623771956`50.*^-111*
    I)*CF*L*nf + 
  (4.3555477189794589212184565320912721421361255612392434017903705`50.*^-112*
    I)*CF*L^2*nf + 
  (3.90912383864209835085816917666070653652721498102219202447762799`50.*^-111*
    I)*CA*CF*irrational[Pi^2] + 
  (1.4699856232446544920096839102599341563300390775518251663368816`50.*^-111*
    I)*CF^2*irrational[Pi^2] + 
  (4.419706576724866988068981307164700971237464183083203565914155`50.*^-113*
    I)*CA*CF*L*irrational[Pi^2] - 
  (1.7678826306899467952275925228658803884949856732332814263656621`50.*^-112*
    I)*CF^2*L*irrational[Pi^2] - 
  (5.3036478920698403856827775685976411654849570196998442790969862`50.*^-112*
    I)*CA*CF*irrational[Zeta[3]] + 
  (2.12145915682793615427311102743905646619398280787993771163879448`50.*^-111*
    I)*CF^2*irrational[Zeta[3]], 
 1.3074842891344022143339372847489793313979713137868700318355977`50.*^-111*CA*
   CF + 
  3.14069536329071238208508249671504825737731472284120971960915732`50.*^-111*
   CF^2 - 
  1.9774496928917122598081512366917224254575453120822031555586097`50.*^-112*
   CA*CF*L - 
  1.43779947395047180509827171245050628440337683411558841293574646`50.*^-111*
   CF^2*L + 
  3.119201544955374056831186115063405952862233887211950821812438`50.*^-113*CA*
   CF*L^2 + 
  1.6810477042243942423835417525958539607498968202123330396665207`50.*^-112*
   CF^2*L^2 - 
  1.4421858906631874301514303729696748393036959473034044404576371`50.*^-112*
   CF*nf + 
  3.184602423869066372414378175890406334826007031121151586522349`50.*^-113*CF*
   L*nf - 
  5.67127553628249828514761111829710173247678888583991058511352`50.*^-114*CF*
   L^2*nf - 
  5.104381071257878067176317224084515853054419773147607169095229`50.*^-113*CA*
   CF*irrational[Pi^2] - 
  1.914887653761708306638615119997572614648033212999507274116394`50.*^-113*
   CF^2*irrational[Pi^2] - 5.739878671071255828661014684629481780827875562445\
71891677163009356259724416919`50.*^-115*CA*CF*L*irrational[Pi^2] + 
  2.2959514684285023314644058738517927123311502249782875667086522907697499758\
00855`50.*^-114*CF^2*L*irrational[Pi^2] + 
  6.88785440528550699439321762155537813699345067493486270012596`50.*^-114*CA*
   CF*irrational[Zeta[3]] - 
  2.755141762114202797757287048622151254797380269973945080050382`50.*^-113*
   CF^2*irrational[Zeta[3]], 
 (1.687081177543412764328834668057407418712399864839761525020922`50.*^-113*I)*
   CA*CF + 
  (4.0693123923068452421784956968611148340736014304799217808209`50.*^-113*I)*
   CF^2 - (2.5513534415899657491382734224258168244348208865876526340636136689\
87531888364701`50.*^-114*I)*CA*CF*L - 
  (1.858004622944774601656952630934190884765477222711574202578922`50.*^-113*
    I)*CF^2*L + (4.0092244383163098553126367471246473008168420641930116751923\
8136759618419532528`50.*^-115*I)*CA*CF*L^2 + 
  (2.166249641688539452844553896089534615201868128053406118057952388509495669\
225351`50.*^-114*I)*CF^2*L^2 - (1.8614625076789658218294032434686273522339651\
40663410246753896404627456317495553`50.*^-114*I)*CF*nf + 
  (4.110220362294169878287661076173318257201572934021764827337844765676901899\
38857`50.*^-115*I)*CF*L*nf - (7.289498978756927009659339540226631456030621934\
8963848639861479410839712642278`50.*^-116*I)*CF*L^2*nf - 
  (6.579105600687152845817005860715017967126398573934644242306760501210329496\
85815`50.*^-115*I)*CA*CF*irrational[Pi^2] - 
  (2.462346484514394057157761828630897219519907882476827774762438935460286331\
2583`50.*^-115*I)*CF^2*irrational[Pi^2] - 
  (7.358818809065712600847454723883951001061378926212460149707218068669996466\
883`50.*^-117*I)*CA*CF*L*irrational[Pi^2] + 
  (2.943527523626285040338981889553580400424551570484984059882887227467998586\
7534`50.*^-116*I)*CF^2*L*irrational[Pi^2] + 
  (8.830582570878855121016945668660741201273654711454952179648661682403995760\
2603`50.*^-116*I)*CA*CF*irrational[Zeta[3]] - 
  (3.532233028351542048406778267464296480509461884581980871859464672961598304\
10412`50.*^-115*I)*CF^2*irrational[Zeta[3]], 
 -2.1491301637305971236808011925673361480228599307037608926527875052615481293\
2773`50.*^-115*CA*CF - 5.2049321253408895129063048217826768397744753415045356\
6881230120232607862809508`50.*^-115*CF^2 + 
  3.2498244193837461099152422602666116376485795505496620308547981296922242685\
22`50.*^-116*CA*CF*L + 2.3703410980934947144036240193238836766423710322227188\
929231143472518127032454`50.*^-115*CF^2*L - 
  5.0877777157241430197821693157001977854008661367820033903385758238040118283\
5`50.*^-117*CA*CF*L^2 - 2.755948608858322553257936718040720206936237595228528\
0388841472633178291575612`50.*^-116*CF^2*L^2 + 
  2.3719989838947436043965342107469347359508777242911638451339766510432244194\
74`50.*^-116*CF*nf - 
  5.2371677593424880728096156754102432708916919858851722343780002608999506649\
63`50.*^-117*CF*L*nf + 
  9.250504937680260035967580574000359609819756612330915255161046952370930597`\
50.*^-118*CF*L^2*nf + 
  8.3718825526866627509850266141826830297919245962790595273598882879258621700\
88`50.*^-117*CA*CF*irrational[Pi^2] + 
  3.1260985785527433125805360087121231299054376218763932040912663856692032359\
13`50.*^-117*CF^2*irrational[Pi^2] + 
  9.3149605178046994947436135745366468367865556028005824679838203400886031226`\
50.*^-119*CA*CF*L*irrational[Pi^2] - 
  3.7259842071218797978974454298146587347146222411202329871935281360354412490\
5`50.*^-118*CF^2*L*irrational[Pi^2] - 
  1.1177952621365639393692336289443976204143866723360698961580584408106323747\
16`50.*^-117*CA*CF*irrational[Zeta[3]] + 
  4.4711810485462557574769345157775904816575466893442795846322337632425294988\
66`50.*^-117*CF^2*irrational[Zeta[3]], 
 (-2.703259381109580345907218710349785999609472074820230868071861183378570646\
708`50.*^-117*I)*CA*CF - 
  (6.573234549476204170917099328366444754550835038941708777208484544269140808\
479`50.*^-117*I)*CF^2 + 
  (4.087371342165411098806099506259257744352080878245372749492436697027231172\
36`50.*^-118*I)*CA*CF*L + 
  (2.985805549892746661884021678094130670833956059941409283879318376293952805\
519`50.*^-117*I)*CF^2*L - 
  (6.375536988064790030920197467214637765919483625707106598782544444242474666\
1`50.*^-119*I)*CA*CF*L^2 - 
  (3.462090239838152373500206052285806533916604907617114374732232309227283065\
23`50.*^-118*I)*CF^2*L^2 + 
  (2.984506254999221536163838095288814519075525862402736919176315574698724204\
61`50.*^-118*I)*CF*nf - 
  (6.589011667562234859312879372743278695712148975442969717606642455330380528\
8`50.*^-119*I)*CF*L*nf + 
  (
    1.159188543284507278349126812220843230167178841037655745233189898953177212`\
50.*^-119*I)*CF*L^2*nf + 
  (1.051919400474685076389327475814426140505198923011250213060334769974448214\
74`50.*^-118*I)*CA*CF*irrational[Pi^2] + 
  (3.918988063537640979313603787149272143526517327240695051494999915402550289\
1`50.*^-119*I)*CF^2*irrational[Pi^2] + 
  (
    1.16437006472558743684295169681708085459831945035007280849797754251107539`\
50.*^-120*I)*CA*CF*L*irrational[Pi^2] - 
  (
    4.657480258902349747371806787268323418393277801400291233991910170044301561`\
50.*^-120*I)*CF^2*L*irrational[Pi^2] - 
  (1.397244077670704924211542036180497025517983340420087370197573051013290468\
4`50.*^-119*I)*CA*CF*irrational[Zeta[3]] + 
  (5.588976310682819696846168144721988102071933361680349480790292204053161873\
6`50.*^-119*I)*CF^2*irrational[Zeta[3]], 
 3.3579909958907174468428260914749614489401230781605705702343726342303184804`\
50.*^-119*CA*CF + 
  8.1975330973125245312537846310928280574977544535837751756784609225121440755`\
50.*^-119*CF^2 - 
  5.076825974423295119096684558818460235304361719649848345285026450541291396`\
50.*^-120*CA*CF*L - 
  3.7142237130865869494199097345435022194828071110944819281056565727037295989`\
50.*^-119*CF^2*L + 
  7.89031964173067787651377743532647469500525317181858742348296962389597828`5\
0.*^-121*CA*CF*L^2 + 
  4.29515714073154170100984959469872560530172998800847764564337517920544011`5\
0.*^-120*CF^2*L^2 - 
  3.708490276634258820183146962016903215084303641960373808289022645594770278`\
50.*^-120*CF*nf + 
  8.18663849283557006949930067031188539960419333305513983761647140296059383`5\
0.*^-121*CF*L*nf - 
  1.43460357122375961391159589733208630818277330396701589517872174979926878`5\
0.*^-121*CF*L^2*nf - 
  1.305309988726962785149652477376441488160378874869063041074676439912964024`\
50.*^-120*CA*CF*irrational[Pi^2] - 
  4.85211844236358911173195217055279302936073130174911759622305069108465923`5\
0.*^-121*CF^2*irrational[Pi^2] - 
  1.4374939070686264652382119713791121661707647535186084055530586944581178`50.\
*^-122*CA*CF*L*irrational[Pi^2] + 
  5.7499756282745058609528478855164486646830590140744336222122347778324711`50.\
*^-122*CF^2*L*irrational[Pi^2] + 
  1.72499268848235175828585436565493459940491770422233008666367043334974132`5\
0.*^-121*CA*CF*irrational[Zeta[3]] - 
  6.89997075392940703314341746261973839761967081688932034665468173339896528`5\
0.*^-121*CF^2*irrational[Zeta[3]], 
 (
    4.12008019288139609642623231915982283267265083243771977099501586910563291`\
50.*^-121*I)*CA*CF + 
  (
    1.0097059019182299416038583831323150198897091257566524267596828858385543`\
50.*^-120*I)*CF^2 - 
  (
    6.2283324219026831299708857476069277482991633467704392584973989473772056`\
50.*^-122*I)*CA*CF*L - 
  (
    4.56349925571350478703841929711909391107253002825970995843638914474123312`\
50.*^-121*I)*CF^2*L + 
  (
    9.64557747761328907284906017667978078524113599286894831597859993842234`50.\
*^-123*I)*CA*CF*L^2 + 
  (
    5.2633249457106459072716969253774897826487051455880250995553299830346786`\
50.*^-122*I)*CF^2*L^2 - 
  (
    4.5515112089759007210561671231042311188551770726491028938457684811490707`\
50.*^-122*I)*CF*nf + 
  (
    1.0046618522228816959770320584673543985330629572776501097568316928215588`\
50.*^-122*I)*CF*L*nf - 
  (
    1.75374135956605255869982912303268741549838836233980878472338180698588`50.\
*^-123*I)*CF*L^2*nf - 
  (
    1.5998667500282149334632669430316945951658290388392113294729891513914354`\
50.*^-122*I)*CA*CF*irrational[Pi^2] - 
  (
    5.933920430612334301083180859891468043185512068165669309830851528196609`50.\
*^-123*I)*CF^2*irrational[Pi^2] - 
  (
    1.75304135008369081126611216021842947093995701648610781165007157860746`50.\
*^-124*I)*CA*CF*L*irrational[Pi^2] + 
  (
    7.01216540033476324506444864087371788375982806594443124660028631442984`50.\
*^-124*I)*CF^2*L*irrational[Pi^2] + 
  (
    2.103649620100428973519334592262115365127948419783329373980085894328953`50.\
*^-123*I)*CA*CF*irrational[Zeta[3]] - 
  (
    8.414598480401715894077338369048461460511793679133317495920343577315811`50.\
*^-123*I)*CF^2*irrational[Zeta[3]], 
 -4.993802558224144898417881573498719041244754945010358068919325711259057`50.\
*^-123*CA*CF - 
  1.2285160080797452435510524266297270332929855276924513366978889581134942`50.\
*^-122*CF^2 + 
  7.54828534682018625641978941551603654060658543227693832349813106509179`50.*^\
-124*CA*CF*L + 
  5.538818913995832688586364407455713608267835300109708791431829741230624`50.\
*^-123*CF^2*L - 
  1.16488400306216197074468433581378730496172186619783878358551978310577`50.*^\
-124*CA*CF*L^2 - 
  6.37158044210510008381286850171038637114935993152806788286279864091692`50.*^\
-124*CF^2*L^2 + 
  5.51840325511265020838181063471785747415741755377351045054072234907669`50.*^\
-124*CF*nf - 
  1.21794853168995988446334507902983957792057856966400410298978581832191`50.*^\
-124*CF*L*nf + 
  2.1179709146584763104448806105705223726576761203597068792463996056468`50.*^\
-125*CF*L^2*nf + 
  1.93712821963473487705572940904694853054346782645832772442519067413015`50.*^\
-124*CA*CF*irrational[Pi^2] + 
  7.169188783626505168583831640354219805945347042829657701614383506996`50.*^-\
125*CF^2*irrational[Pi^2] + 
  2.112098012149025073814592964118589724024044598176033508012134432057`50.*^-\
126*CA*CF*L*irrational[Pi^2] - 
  8.448392048596100295258371856474358896096178392704134032048537728229`50.*^-\
126*CF^2*L*irrational[Pi^2] - 
  2.5345176145788300885775115569423076688288535178112402096145613184686`50.*^\
-125*CA*CF*irrational[Zeta[3]] + 
  1.01380704583153203543100462277692306753154140712449608384582452738745`50.*^\
-124*CF^2*irrational[Zeta[3]], 
 (
    -5.9802715035657853136470718974677844018064155320326684989186177541578`50.*^\
-125*I)*CA*CF - 
  (
    1.47674450461789551426670101192988675917915886478420380236312962428562`50.\
*^-124*I)*CF^2 + 
  (
    9.038283397730521121345410620146472979580970607891976083724200299804`50.*^\
-126*I)*CA*CF*L + 
  (
    6.6418624661716955780049252593290332524541322774436614291782421508031`50.*^\
-125*I)*CF^2*L - 
  (
    1.390021053257437421079827507207013049254321504114283948663467734881`50.*^\
-126*I)*CA*CF*L^2 - 
  (
    7.620857662604240834014183074974639226098712513231407877575612564537`50.*^\
-126*I)*CF^2*L^2 + 
  (
    6.610503468686949149092163807802720688409688216086428744020497146866`50.*^\
-126*I)*CF*nf - 
  (
    1.458803694802502407520492005273730269219145902112892629939569638372`50.*^\
-126*I)*CF*L*nf + 
  (
    2.52731100592261349287241364946729645318967546202597081575175951797`50.*^\
-127*I)*CF*L^2*nf + 
  (
    2.317401068860809508759336142806186910879342359518486462675983435191`50.*^\
-126*I)*CA*CF*irrational[Pi^2] + 
  (
    8.55814794338103094866197765663950189634421762702848494427798680819`50.*^\
-127*I)*CF^2*irrational[Pi^2] + 
  (
    2.5144023954155060402554678144268925286000530930667065571573028953`50.*^-\
128*I)*CA*CF*L*irrational[Pi^2] - 
  (
    1.00576095816620241610218712577075701144002123722668262286292115812`50.*^\
-127*I)*CF^2*L*irrational[Pi^2] - 
  (
    3.01728287449860724830656137731227103432006371168004786858876347437`50.*^\
-127*I)*CA*CF*irrational[Zeta[3]] + 
  (
    1.206913149799442899322624550924908413728025484672019147435505389747`50.*^\
-126*I)*CF^2*irrational[Zeta[3]], 
 7.07679155074914996256345253623277706608672749021418036113720834549`50.*^-127\
*CA*CF + 
  1.754009274109187744138194383058961662421272776443377945974642445802`50.*^-\
126*CF^2 - 
  1.06941750237136480908248555464140893785956176308015016878624355306`50.*^-1\
27*CA*CF*L - 
  7.87007467133281879934634439308162597080139620388170949997006397582`50.*^-1\
27*CF^2*L + 
  1.6391030402894452397925690874311482166099930835915429096602715642`50.*^-128\
*CA*CF*L^2 + 
  9.0072565214745553242837752900643847162151115996714258626368140488`50.*^-128\
*CF^2*L^2 - 
  7.8249459779849948782705347330580082673649242260797400064985833472`50.*^-128\
*CF*nf + 
  1.7265783868380295546689257360282512083738172162492814563695912093`50.*^-128\
*CF*L*nf - 
  2.980187345980809526895580158965724030199987424711896199382311935`50.*^-129*
   CF*L^2*nf - 
  2.7395211886576539638894455418500073241737218370997726079359470902`50.*^-128\
*CA*CF*irrational[Pi^2] - 
  1.0095621535512241398796349168901671801480652285645326965593259645`50.*^-128\
*CF^2*irrational[Pi^2] - 
  2.95812046519471298853584448756105003364712128596083124371447399`50.*^-130*
   CA*CF*L*irrational[Pi^2] + 
  1.183248186077885195414337795024420013458848514384332497485789598`50.*^-129*
   CF^2*L*irrational[Pi^2] + 
  3.549744558233655586243013385073260040376545543152997492457368793`50.*^-129*
   CA*CF*irrational[Zeta[3]] - 
  1.4198978232934622344972053540293040161506182172611989969829475173`50.*^-128\
*CF^2*irrational[Zeta[3]], 
 (8.276355493830816213852682942009511073619201224548767772924267024`50.*^-129*
    I)*CA*CF + 
  (
    2.0588360290829377564494088005167337730489798741305347162778648661`50.*^-\
128*I)*CF^2 - 
  (
    1.250527933504447116321056270775637257867669492834031260225688488`50.*^-129\
*I)*CA*CF*L - 
  (
    9.216060979863194567573939934330691229009970473679002635808923412`50.*^-129\
*I)*CF^2*L + 
  (1.91028335675341016305657402118849392671198660936615644440964445`50.*^-130*
    I)*CA*CF*L^2 + 
  (
    1.052141267005511472930305584398063470455293476267702416920308128`50.*^-129\
*I)*CF^2*L^2 - 
  (9.15408230101799340385799185153167828428370743252815649192501518`50.*^-130*
    I)*CF*nf + 
  (2.01956773563484664668068283929433279020259952166262754642996083`50.*^-130*
    I)*CF*L*nf - 
  (3.4732424668243821146483164021608980485672483806657389898357172`50.*^-131*
    I)*CF*L^2*nf - 
  (3.20066066419337405348720869871516397787173804156034540071055593`50.*^-130*
    I)*CA*CF*irrational[Pi^2] - 
  (1.17703768373418484229608931704605925581702728541431012183996854`50.*^-130*
    I)*CF^2*irrational[Pi^2] - 
  (3.439674959528736033181214520419825620519908472047478190365667`50.*^-132*
    I)*CA*CF*L*irrational[Pi^2] + 
  (1.375869983811494413272485808167930248207963388818991276146267`50.*^-131*
    I)*CF^2*L*irrational[Pi^2] + 
  (4.1276099514344832398174574245037907446238901664569738284388009`50.*^-131*
    I)*CA*CF*irrational[Zeta[3]] - 
  (1.65104398057379329592698296980151629784955606658278953137552037`50.*^-130*
    I)*CF^2*irrational[Zeta[3]], 
 -9.5672772122078643419985013110555889606160038689787550372393276`50.*^-131*
   CA*CF - 
  2.3885557757735819363721703768052082352218059797995026564673179`50.*^-130*
   CF^2 + 
  1.4453863367396296598177762138282933589864373374383970501497941`50.*^-131*
   CA*CF*L + 
  1.06671685099421441938299520302890500751901947784321765576893157`50.*^-130*
   CF^2*L - 
  2.200670696253626643471559302747334616886078049039706451648076`50.*^-132*CA*
   CF*L^2 - 
  1.2148085630630585671286298954330512442312752611637822734014769`50.*^-131*
   CF^2*L^2 + 
  1.0585087698729910354112679150074693340312891216089273787958946`50.*^-131*
   CF*nf - 
  2.334925063723923687134912007812344325471855230968373342150783`50.*^-132*CF*
   L*nf + 
  4.00121944773386662449374418681333566706559645279946627572377`50.*^-133*CF*
   L^2*nf + 
  3.696200888721227358172353937020631768340212508627798375636469`50.*^-132*CA*
   CF*irrational[Pi^2] + 
  1.356472102721235421945299360939369411909471253589232943512682`50.*^-132*
   CF^2*irrational[Pi^2] + 3.953649378768662107104844276344627150022883301203\
997919960537282114201168283491`50.*^-134*CA*CF*L*irrational[Pi^2] - 
  1.5814597515074648428419377105378508600091533204815991679842157365258001359\
48498`50.*^-133*CF^2*L*irrational[Pi^2] - 
  4.74437925452239452852581313161355258002745996144479750395265`50.*^-133*CA*
   CF*irrational[Zeta[3]] + 
  1.897751701808957811410325252645421032010983984577919001581058`50.*^-132*
   CF^2*irrational[Zeta[3]], 
 (-1.09330798715819699233933603454402816826275401546328756535616`50.*^-132*I)*
   CA*CF - 
  (2.739247765377505133839598261520685393220487011039258096556823`50.*^-132*
    I)*CF^2 + (1.651494817186028129120384830553220505518044446649539367797517\
1711006546181253032`50.*^-133*I)*CA*CF*L + 
  (1.220530779205483556017418553217774012423950015383255976086203`50.*^-132*
    I)*CF^2*L - (2.5063157342956365097456534239015587789165034113741480481934\
65442757977169794929`50.*^-134*I)*CA*CF*L^2 - 
  (1.386602429543179611135906254109441572684356772070403678285098844980924612\
0371286`50.*^-133*I)*CF^2*L^2 + (1.209980719725823843935263215080807896069577\
2836067720866527123696198193981704101`50.*^-133*I)*CF*nf - 
  (2.668629060002404665155192156765342175626952527675617674514989475184885082\
680533`50.*^-134*I)*CF*L*nf + (4.55693769871933910862846077073010687075727892\
977117826944266444137814030871805`50.*^-135*I)*CF*L^2*nf + 
  (4.219690148191906976808773873606737182452286965660130373949378982755619038\
342925`50.*^-134*I)*CA*CF*irrational[Pi^2] + 
  (1.545440652603573909480067766854430397883840886602203959606373446280870151\
443108`50.*^-134*I)*CF^2*irrational[Pi^2] + 
  (4.492783384964388758073686677664349034116912842277270363591519638766137691\
2312`50.*^-136*I)*CA*CF*L*irrational[Pi^2] - 
  (1.797113353985755503229474671065739613646765136910908145436607855506455076\
4925`50.*^-135*I)*CF^2*L*irrational[Pi^2] - 
  (5.391340061957266509688424013197218840940295410732724436309823566519365229\
47749`50.*^-135*I)*CA*CF*irrational[Zeta[3]] + 
  (2.156536024782906603875369605278887536376118164293089774523929426607746091\
790996`50.*^-134*I)*CF^2*irrational[Zeta[3]], 
 1.23525949939173829716702718907508476462191587135816782858871695498045870895\
9399`50.*^-134*CA*CF + 3.1057549816473734289944412342081249753811186895769043\
2316613021150184173235549`50.*^-134*CF^2 - 1.86564995069503649651760882698582\
592335364387500641173608503503430068520009957`50.*^-135*CA*CF*L - 
  1.3807058976848455694162446498162676385036513221249589911068027323009550415\
00575`50.*^-134*CF^2*L + 2.82225572134325191223982105965192007417790774084437\
80712167867395642743883366`50.*^-136*CA*CF*L^2 + 
  1.5648154542693989572268884308771792678288713347939595173687750375739248491\
2745`50.*^-135*CF^2*L^2 - 1.3674882920550331305919619934012411700354537024386\
6517821184089548427371385628`50.*^-135*CF*nf + 3.0155131325792208441515661597\
240461789532980687299774219490241291510041567209`50.*^-136*CF*L*nf - 
  5.1313740388059125677087655630034910439598322560806874022123395264804988878\
84`50.*^-137*CF*L^2*nf - 4.76289912404802717386408508252135112973970382501919\
74632269307398228689963404`50.*^-136*CA*CF*irrational[Pi^2] - 
  1.7408896868882919898927440270691841599012752818103088768312064916318269968\
188`50.*^-136*CF^2*irrational[Pi^2] - 
  5.0480712190611109641277378400723022855246211710980565883050782458046490912\
7`50.*^-138*CA*CF*L*irrational[Pi^2] + 
  2.0192284876244443856510951360289209142098484684392226353220312983218596365\
09`50.*^-137*CF^2*L*irrational[Pi^2] + 
  6.0576854628733331569532854080867627426295454053176679059660938949655789095\
26`50.*^-137*CA*CF*irrational[Zeta[3]] - 2.4230741851493332627813141632347050\
970518181621270671623864375579862315638101`50.*^-136*CF^2*
   irrational[Zeta[3]], (1.38003860679008421344150418691196484565842445686968\
86747842162727121536404234`50.*^-136*I)*CA*CF + 
  (3.481760744776626824048132948045237369483131620039330782417615058903404844\
7039`50.*^-136*I)*CF^2 - 
  (2.084003532747223998396509818284250320272503642371941990470127810327456617\
038`50.*^-137*I)*CA*CF*L - (1.54440890814746315314715002509046533194318658915\
87474791038238058358740874466`50.*^-136*I)*CF^2*L + 
  (3.142620580464966123738142381870239125076647551276723292555545898662465978\
64`50.*^-138*I)*CA*CF*L^2 + 
  (1.746211372789191882638981254297780760347025345479840863862261047493217698\
46`50.*^-137*I)*CF^2*L^2 - 
  (1.528218725137144171108122394050281091390143344516398451730519701745965293\
789`50.*^-137*I)*CF*nf + 
  (3.369362264843719363010994204679948048069881467471513979544652193708242142\
59`50.*^-138*I)*CF*L*nf - 
  (5.713855600845392952251167967036798409230268275048587804646447088477210870\
2`50.*^-139*I)*CF*L^2*nf - 
  (5.315982288076316978489737485194512914287788290055584693345228249678802712\
51`50.*^-138*I)*CA*CF*irrational[Pi^2] - 
  (
    1.939200985975961217693193332697217174076547005134594118833960314368000864`\
50.*^-138*I)*CF^2*irrational[Pi^2] - 
  (
    5.608968021179012182364153155635891428360690190108951764783420273116276768`\
50.*^-140*I)*CA*CF*L*irrational[Pi^2] + 
  (2.243587208471604872945661262254356571344276076043580705913368109246510707\
3`50.*^-139*I)*CF^2*L*irrational[Pi^2] + 
  (6.730761625414814618836983786763069714032828228130742117740104327739532121\
7`50.*^-139*I)*CA*CF*irrational[Zeta[3]] - 
  (2.692304650165925847534793514705227885613131291252296847096041731095812848\
68`50.*^-138*I)*CF^2*irrational[Zeta[3]], 
 -1.5247396569791439983072210012794386407098467556841973140951544598100126082\
1`50.*^-138*CA*CF - 
  3.8599492079899434401969400875926450107572334368079441053035250651169955841\
8`50.*^-138*CF^2 + 
  2.3021653367414046036280910282586344014951356214578483212159725196599380591`\
50.*^-139*CA*CF*L + 
  1.7083885558866857547674816506169723600427233744266529895241996580816972435\
8`50.*^-138*CF^2*L - 
  3.460799722755594151722030377571519326762868025546082535971993558715752513`\
50.*^-140*CA*CF*L^2 - 
  1.9271132556737188157633454207986757876418512026757861945088055076482216921`\
50.*^-139*CF^2*L^2 + 
  1.6889565245996975640376385479150532390157882727590972555529843177089637999`\
50.*^-139*CF*nf - 
  3.723078027677958270101402170484745311782860883423840285152257029039033218`\
50.*^-140*CF*L*nf + 
  6.29236313228289845767641886831185332138703277372015006540362465221045911`5\
0.*^-141*CF*L^2*nf + 
  5.867745124743756408051780452249046404333506633726814483742462008976995959`\
50.*^-140*CA*CF*irrational[Pi^2] + 
  2.136294090028929867692900588666328576546399683204783797257680396234931377`\
50.*^-140*CF^2*irrational[Pi^2] + 
  6.1637011221747386619386298413581224487480111979219250162455167836442602`50.\
*^-142*CA*CF*L*irrational[Pi^2] - 
  2.46548044886989546477545193654324897949920447916877000649820671345770408`5\
0.*^-141*CF^2*L*irrational[Pi^2] - 
  7.39644134660968639432635580962974693849761343750631001949462014037311222`5\
0.*^-141*CA*CF*irrational[Zeta[3]] + 
  2.958576538643874557730542323851898775399045375002524007797848056149244888`\
50.*^-140*CF^2*irrational[Zeta[3]], 
 (
    -1.666191705512501452546574874398892198122469536357604131095752481573760474`\
50.*^-140*I)*CA*CF - 
  (
    4.232223948521880804376304520531048886198646599324324098625586641021963993`\
50.*^-140*I)*CF^2 + 
  (
    2.51534502557486307802036792277552264755213387737973186700693069651685528`\
50.*^-141*I)*CA*CF*L + 
  (
    1.869078771931023200071609548780274001165979905046671564589257805506032176`\
50.*^-140*I)*CF^2*L - 
  (
    3.7696640923347727799093722208346228243896521487095864165630143099774902`\
50.*^-142*I)*CA*CF*L^2 - 
  (
    2.10352383317942830808428548496363417297570792082893166574201033730692741`\
50.*^-141*I)*CF^2*L^2 + 
  (
    1.84618663722815868026640697524079214544896625000811958448568412248054585`\
50.*^-141*I)*CF*nf - 
  (
    4.0689072411502666606259765912177928056388352239798101881985443377525422`\
50.*^-142*I)*CF*L*nf + 
  (
    6.853934713335950508926131310608405135253912997653793484660026018140892`50.\
*^-143*I)*CF*L^2*nf + 
  (
    6.4060097483524696747441251235995315262563291765863202402286433428548111`\
50.*^-142*I)*CA*CF*irrational[Pi^2] + 
  (
    2.3277626018437108000679060235365439853992145810171273945807004894584459`\
50.*^-142*I)*CF^2*irrational[Pi^2] + 
  (
    6.69967513279862898036807591451969831385653391078470110461469215613506`50.\
*^-144*I)*CA*CF*L*irrational[Pi^2] - 
  (
    2.679870053119451592147230365807879325542613564313880441845876862454026`50.\
*^-143*I)*CF^2*L*irrational[Pi^2] - 
  (
    8.039610159358354776441691097423637976627840692941641325537630587362078`50.\
*^-143*I)*CA*CF*irrational[Zeta[3]] + 
  (
    3.2158440637433419105766764389694551906511362771766565302150522349448314`\
50.*^-142*I)*CF^2*irrational[Zeta[3]], 
 1.8010708062505734625692713022042124826981156312425152239968805827290495`50.\
*^-142*CA*CF + 
  4.5900006199293408120097607740585946172845827002823534043372693215531184`50.\
*^-142*CF^2 - 
  2.718527164520865815205901148443893088640328838176631973189819018597597`50.\
*^-143*CA*CF*L - 
  2.0227273428602323032014162464770856507587834065778321870267488621075585`50.\
*^-142*CF^2*L + 
  4.06183336030947968845273374786620008812066540025761539816053542491016`50.*^\
-144*CA*CF*L^2 + 
  2.271272718465536111960090611175416893169379731166562278335733870315554`50.\
*^-143*CF^2*L^2 - 
  1.996222211240713654220007920711766697464756371160842446517175023510657`50.\
*^-143*CF*nf + 
  4.39872459185957968340095600716547123654445226295742785618266971595192`50.*^\
-144*CF*L*nf - 
  7.3851515641990539790049704506658183420375734550138461784737007725639`50.*^\
-145*CF*L^2*nf - 
  6.91806266396396365040990336530431710292368100936476411677796361758401`50.*^\
-144*CA*CF*irrational[Pi^2] - 
  2.50903909330856214288497172370478581315001977052637064428753096257907`50.*^\
-144*CF^2*irrational[Pi^2] - 
  7.203951755697450516524812811311503563286595602994302263026550705522`50.*^-\
146*CA*CF*L*irrational[Pi^2] + 
  2.8815807022789802066099251245246014253146382411977209052106202822086`50.*^\
-145*CF^2*L*irrational[Pi^2] + 
  8.6447421068369406198297753735738042759439147235931627156318608466259`50.*^\
-145*CA*CF*irrational[Zeta[3]] - 
  3.45789684273477624793191014942952171037756588943726508625274433865036`50.*^\
-144*CF^2*irrational[Zeta[3]], 
 (
    1.92603532132509440477195583323120231081458112277269860502111302085753`50.*^\
-144*I)*CA*CF + 
  (
    4.92453301672902760850746553678581562236202986331768040654533368549834`50.\
*^-144*I)*CF^2 - 
  (
    2.9066703849708755291090073403197200113910580880725482531152577112295`50.*^\
-145*I)*CA*CF*L - 
  (
    2.1655436351810962104121049274379358573542426235265116369441410830767`50.*^\
-144*I)*CF^2*L + 
  (
    4.329974151586287991655249551388118069007142831406557903704695178019`50.*^\
-146*I)*CA*CF*L^2 + 
  (
    2.4261829207533643780273431886010835496690307784009515662624746118316`50.*^\
-145*I)*CF^2*L^2 - 
  (
    2.1353504524607800122392939960191893694307555579361107781359268984159`50.*^\
-145*I)*CF*nf + 
  (
    4.704354795281534265596052614724890298574305893384742503681913151136`50.*^\
-146*I)*CF*L*nf - 
  (
    7.87268027561143271210045372979657830728571423892101437037217305094`50.*^\
-147*I)*CF*L^2*nf - 
  (
    7.391161987659167088572996043230436155353047685464762176568915178285`50.*^\
-146*I)*CA*CF*irrational[Pi^2] - 
  (
    2.675579108126537173445346729575146413411375651591490768832042335122`50.*^\
-146*I)*CF^2*irrational[Pi^2] - 
  (
    7.6637784635079260814093753311824505992410591521215981521559050059`50.*^-\
148*I)*CA*CF*L*irrational[Pi^2] + 
  (
    3.06551138540317043256375013247298023969642366084863926086236200235`50.*^\
-147*I)*CF^2*L*irrational[Pi^2] + 
  (
    9.19653415620951129769125039741894071908927098254591778258708600704`50.*^\
-147*I)*CA*CF*irrational[Zeta[3]] - 
  (
    3.678613662483804519076500158967576287635708393018367113034834402819`50.*^\
-146*I)*CF^2*irrational[Zeta[3]], 
 -2.03786257165614235176795118711258253539882881699044618106249584793`50.*^-1\
46*CA*CF - 
  5.227282692309959381158869362436256980444767473230510817693645452223`50.*^-\
146*CF^2 + 
  3.07491944070277503489785179826320626819592386937982788110857071175`50.*^-1\
47*CA*CF*L + 
  2.293857103653783203670102719341384455217256272345925928566460652711`50.*^-\
146*CF^2*L - 
  4.5671121235334023522886378181499037249597403291039021228689530711`50.*^-148\
*CA*CF*L^2 - 
  2.56424717900891791372829088815237347758268603757040213748677186028`50.*^-1\
47*CF^2*L^2 + 
  2.2599883657861867048901180213648780871404520996038285153225735849`50.*^-147\
*CF*nf - 
  4.9779161230128804127933462280094903434633382817245327576830808591`50.*^-148\
*CF*L*nf + 
  8.303840224606186095070250578454370409017709689279822041579914675`50.*^-149*
   CF*L^2*nf + 
  7.8130748818078635059267504335250929880927130921937492827857124706`50.*^-148\
*CA*CF*irrational[Pi^2] + 
  2.8230545429109346722316724281114699140387038375798055004539069758`50.*^-148\
*CF^2*irrational[Pi^2] + 
  8.06713522474518534885197403282363220972743068644378752858516316`50.*^-150*
   CA*CF*L*irrational[Pi^2] - 
  3.226854089898074139540789613129452883890972274577515011434065266`50.*^-149*
   CF^2*L*irrational[Pi^2] - 
  9.680562269694222418622368839388358651672916823732545034302195797`50.*^-149*
   CA*CF*irrational[Zeta[3]] + 
  3.8722249078776889674489475357553434606691667294930180137208783187`50.*^-148\
*CF^2*irrational[Zeta[3]], 
 (
    -2.133593468314073353640829437616862660326797236407105824272645395`50.*^-148\
*I)*CA*CF - 
  (
    5.4902806136556525966032683854257975424112235940154529090910622075`50.*^-\
148*I)*CF^2 + 
  (
    3.218817426565380239726296009141060971830164672549948448265564018`50.*^-149\
*I)*CA*CF*L + 
  (
    2.4042771232306282951509096718343042291202342022272357315532938237`50.*^-\
148*I)*CF^2*L - 
  (4.76693895167347386732078142229181308461980813111556946048588016`50.*^-150*
    I)*CA*CF*L^2 - 
  (
    2.681803493507600576813552238286867112642187200752309937757734458`50.*^-149\
*I)*CF^2*L^2 + 
  (
    2.366839058260318993479638887823066401840436158643902693259020725`50.*^-149\
*I)*CF*nf - 
  (5.21216469283128307421818999304442514118573427123238078507447046`50.*^-150*
    I)*CF*L*nf + 
  (8.6671617303154070314923298587123874265814693293010353827016003`50.*^-151*
    I)*CF*L^2*nf + 
  (8.17261329569143421639709425554993194927363525902237620733919972`50.*^-150*
    I)*CA*CF*irrational[Pi^2] + 
  (2.94754378974051010969795377905463288628043511237079810349444932`50.*^-150*
    I)*CF^2*irrational[Pi^2] + 
  (8.403265859109568071720806284191283551799406965045612008942878`50.*^-152*
    I)*CA*CF*L*irrational[Pi^2] - 
  (3.3613063436438272286883225136765134207197627860182448035771513`50.*^-151*
    I)*CF^2*L*irrational[Pi^2] - 
  (1.00839190309314816860649675410295402621592883580547344107314539`50.*^-150*
    I)*CA*CF*irrational[Zeta[3]] + 
  (4.03356761237259267442598701641181610486371534322189376429258158`50.*^-150*
    I)*CF^2*irrational[Zeta[3]], 
 2.21066062634862472780793574950449097751111498624160464289818884`50.*^-150*
   CA*CF + 
  5.70648958226348618134481651419849098710917622954244647174714008`50.*^-150*
   CF^2 - 
  3.3345049608181191336983726502720318113783447476963526689867554`50.*^-151*
   CA*CF*L - 
  2.49384423617227906909983071431721046389101399857020515628342506`50.*^-150*
   CF^2*L + 
  4.924095021731994264216682103210000213452670513207964996602469`50.*^-152*CA*
   CF*L^2 + 
  2.7756989192373418169662754058043943631801295210295849792215661`50.*^-151*
   CF^2*L^2 - 
  2.4530388998623065401572102200606094376262121338624722455882855`50.*^-151*
   CF*nf + 
  5.400818119759527893961594811416345576926208600048684209893454`50.*^-152*CF*
   L*nf - 8.95290003951271684403033109674545493355031002401448181200449077943\
0310363603287`50.*^-153*CF*L^2*nf - 
  8.460134187872628587780182133695047871872397256822066217562997`50.*^-152*CA*
   CF*irrational[Pi^2] - 
  3.045707666934433718781830955489167279205298156726316618018165`50.*^-152*
   CF^2*irrational[Pi^2] - 8.663160679494400073938975550712663455463306149531\
55877210606009888091960769437`50.*^-154*CA*CF*L*irrational[Pi^2] + 
  3.4652642717977600295755902202850653821853224598126235088424240395523678430\
77749`50.*^-153*CF^2*L*irrational[Pi^2] + 
  1.039579281539328008872677066085519614655596737943787052652727`50.*^-152*CA*
   CF*irrational[Zeta[3]] - 
  4.158317126157312035490708264342078458622386951775148210610908`50.*^-152*
   CF^2*irrational[Zeta[3]], 
 (2.267007923727240317527484840070292988405632061349909440842152`50.*^-152*I)*
   CA*CF + 
  (5.870112453740523463649759116581815817298582194336788880198829`50.*^-152*
    I)*CF^2 - (3.418893735798595828627015301009466752646600302823697141489587\
206282726720729746`50.*^-153*I)*CA*CF*L - 
  (2.560163260483709682637216806164269376259509902244350171888372`50.*^-152*
    I)*CF^2*L + (5.0344099367735566228788713093716433774329619360065030863944\
6465141844352159472`50.*^-154*I)*CA*CF*L^2 + 
  (2.843431260884159378136150470380687446374147086293551816639010141747156276\
889719`50.*^-153*I)*CF^2*L^2 - (2.5162862448486680500687313603611420213349089\
04733278185115166395373986770596639`50.*^-153*I)*CF*nf + 
  (5.538838064066663929645033171757579358313108759403213212568201502689190958\
0805`50.*^-154*I)*CF*L*nf - (9.1534726123155574961434023806757152316962944291\
027328843535720934880791301722`50.*^-155*I)*CF*L^2*nf - 
  (8.667973054942444993507727045304986119229993139675067144911041656973707721\
27357`50.*^-154*I)*CA*CF*irrational[Pi^2] - 
  (3.114939077614851505004950354325741192229318117309443203931724651201552429\
67203`50.*^-154*I)*CF^2*irrational[Pi^2] - 
  (8.839959877035102116264260766033330056595210356664855889904142958041754701\
729`50.*^-156*I)*CA*CF*L*irrational[Pi^2] + 
  (3.535983950814040846505704306413332022638084142665942355961657183216701880\
6916`50.*^-155*I)*CF^2*L*irrational[Pi^2] + 
  (1.060795185244212253951711291923999606791425242799782706788497154965010564\
20747`50.*^-154*I)*CA*CF*irrational[Zeta[3]] - 
  (4.243180740976849015806845167695998427165700971199130827153988619860042256\
8299`50.*^-154*I)*CF^2*irrational[Zeta[3]], 
 -2.3011774919317764681845804425968547188846476253174254953068331528945323882\
2732`50.*^-154*CA*CF - 5.9768595649439615257439056764078996027054213299343729\
4537085489212625803182384`50.*^-154*CF^2 + 3.46980347746010171630462175291017\
79564325568176954831223482783618567811970689`50.*^-155*CA*CF*L + 
  2.6015098435858146859373353817472788910960013403456181524445934561563835377\
8537`50.*^-154*CF^2*L - 
  5.0950857223546777703472105888198343835974237536937873358696675346394716314\
2`50.*^-156*CA*CF*L^2 - 2.883259733958853813349009531456155946809643253109526\
4996304656980106950473856`50.*^-155*CF^2*L^2 + 2.5549435849878730538247984177\
948646072073625811518828470970617436371690750846`50.*^-155*CF*nf - 
  5.6226538277388226887400506286746952028155656205295765524903574778587078857\
77`50.*^-156*CF*L*nf + 
  9.2637922224630504915403828887633352429044068248977951561266682447990393298\
5`50.*^-157*CF*L^2*nf + 
  8.7907829557702963502007644074363276487076672415606218771251419672197841345\
95`50.*^-156*CA*CF*irrational[Pi^2] + 
  3.1534779136610244859713087037056562243693746223822132626816676853448748374\
78`50.*^-156*CF^2*irrational[Pi^2] + 
  8.929252401045557693196222995993262683429505410772581706973881775799752224`\
50.*^-158*CA*CF*L*irrational[Pi^2] - 
  3.5717009604182230772784891983973050733718021643090326827895527103199008895\
9`50.*^-157*CF^2*L*irrational[Pi^2] - 
  1.0715102881254669231835467595191915220115406492927098048368658130959702668\
76`50.*^-156*CA*CF*irrational[Zeta[3]] + 
  4.2860411525018676927341870380767660880461625971708392193474632523838810675\
05`50.*^-156*CF^2*irrational[Zeta[3]], 
 (-2.312375496801829414853739923719375297770160804870438211966625631723364949\
248`50.*^-156*I)*CA*CF - 
  (6.024125276538036034391232463967735071078622065541640501699590246546400316\
865`50.*^-156*I)*CF^2 + 
  (3.486053879678064874258685991215041073841044114430438898210978546033513858\
96`50.*^-157*I)*CA*CF*L + 
  (2.616903867508473068524326822124627093071979273292186028044937750042819750\
494`50.*^-156*I)*CF^2*L - 
  (5.104811604136600921913035102298803515794767067920619040062263596063896655\
6`50.*^-158*I)*CA*CF*L^2 - 
  (2.894277804867683964663643593646562175984387758702928157854734415060973552\
17`50.*^-157*I)*CF^2*L^2 + 
  (2.568106834486079715179274783479692886892747313492527484665293330529127295\
65`50.*^-157*I)*CF*nf - 
  (5.650313215712968953755651674136424597354260717142556896021251432228280775\
7`50.*^-158*I)*CF*L*nf + 
  (
    9.281475643884728948932791095088733665081394668946580072840479265570721192`\
50.*^-159*I)*CF*L^2*nf + 
  (8.825758685127865159875557032979114592053872607271603304902252350420845633\
5`50.*^-158*I)*CA*CF*irrational[Pi^2] + 
  (3.160483288683904545435462572773062931807210083585121308318595300340958206\
8`50.*^-158*I)*CF^2*irrational[Pi^2] + 
  (
    8.92925240104555769319622299599326268342950541077258170697388177579975222`\
50.*^-160*I)*CA*CF*L*irrational[Pi^2] - 
  (
    3.57170096041822307727848919839730507337180216430903268278955271031990089`\
50.*^-159*I)*CF^2*L*irrational[Pi^2] - 
  (1.071510288125466923183546759519191522011540649292709804836865813095970266\
9`50.*^-158*I)*CA*CF*irrational[Zeta[3]] + 
  (4.286041152501867692734187038076766088046162597170839219347463252383881067\
5`50.*^-158*I)*CF^2*irrational[Zeta[3]]}


==> attachedfiles/B1 <==
{(1.`50.*I)*CF, -0.3333333333333333333333333333333333333333333333333333333333\
3333333333333333333`50.*CF, 
 (-0.083333333333333333333333333333333333333333333333333333333333333333333333\
33333`50.*I)*CF, 0.0166666666666666666666666666666666666666666666666666666666\
6666666666666666666`50.*CF, (0.0027777777777777777777777777777777777777777777\
7777777777777777777777777777778`50.*I)*CF, 
 -0.0003968253968253968253968253968253968253968253968253968253968253968253968\
254`50.*CF, (-0.0000496031746031746031746031746031746031746031746031746031746\
0317460317460317`50.*I)*CF, 
 5.51146384479717813051146384479717813051146384479717813051146384479717813`50.\
*^-6*CF, 
 (
   5.5114638447971781305114638447971781305114638447971781305114638447971781`50.\
*^-7*I)*CF, 
 -5.010421677088343755010421677088343755010421677088343755010421677088344`50.\
*^-8*CF, 
 (
   -4.17535139757361979584201806424028646250868473090695312917535139757362`50.\
*^-9*I)*CF, 
 3.2118087673643229198784754340309895865451421006976562532118087673643`50.*^-\
10*CF, 
 (
   2.294149119545944942770339595736421133246530071926897323722720548117`50.*^\
-11*I)*CF, 
 -1.52943274636396329518022639715761408883102004795126488248181369875`50.*^-12\
*CF, 
 (-9.558954664774770594876414982235088055193875299695405515511335618`50.*^-14*
   I)*CF, 
 5.62291450869104152639789116602064003246698547040906206794784448`50.*^-15*
  CF, 
 (3.1238413937172452924432728700114666847038808168939233710821358`50.*^-16*I)*
  CF, 
 -1.644127049324865943391196247374456149844147798365222826885335`50.*^-17*CF, 
 (-8.220635246624329716955981236872280749220738991826114134426673217368182813\
75026`50.*^-19*I)*CF, 
 3.91458821267825224616951487470108607105749475801243530210793962731818229226\
2`50.*^-20*CF, 
 (1.7793582784901146573497794885004936686624976172783796827763361942355374055\
74`50.*^-21*I)*CF, 
 -7.7363403412613680754338238630456246463586852925146942729405921488501626329`\
50.*^-23*CF, 
 (
   -3.223475142192236698097426609602343602649452205214455947058580062020901097`\
50.*^-24*I)*CF, 
 1.28939005687689467923897064384093744105978088208578237882343202480836044`50.\
*^-25*CF, 
 (
   4.959192526449594920149887091695913234845311084945316841628584710801386`50.\
*^-27*I)*CF, 
 -1.8367379727591092296851433672947826795723374388686358672698461891857`50.*^\
-28*CF, 
 (
   -6.559778474139675820304083454624223855615490853102270954535164961378`50.*^\
-30*I)*CF, 
 2.26199257728954338631175291538766339848810029417319688087419481427`50.*^-31*
  CF, 
 (7.539975257631811287705843051292211328293667647243989602913982714`50.*^-33*
   I)*CF, 
 -2.4322500831070358992599493713845842994495702087883837428754783`50.*^-34*
  CF, 
 (-7.60078150970948718518734178557682593577990690246369919648587`50.*^-36*I)*
  CF, 2.303267124154390056117376298659644222963608152261727029238143904664679\
168454126`50.*^-37*CF, (6.774315071042323694462871466646012420481200447828608\
9095239480139035689019846`50.*^-39*I)*CF, 
 -1.9355185917263781984179632761845749772803429850938882598639851468295911148\
53`50.*^-40*CF, 
 (-5.376440532573272773383231322734930492445397180816356277399958741193308652\
4`50.*^-42*I)*CF, 
 1.453092035830614263076549006144575808769026265085501696594583443565759095`5\
0.*^-43*CF, 
 (
   3.823926410080563850201444753012041602023753329172372885775219588330945`50.\
*^-45*I)*CF, 
 -9.80493951302708679538831987951805538980449571582659714301338355982293`50.*^\
-47*CF, 
 (
   -2.4512348782567716988470799698795138474511239289566492857533458899557`50.*^\
-48*I)*CF, 
 5.97862165428480902157824382897442401817347299745524216037401436575`50.*^-50*
  CF, 
 (1.4234813462582878622805342449939104805174935708226767048509558014`50.*^-51*
   I)*CF, 
 -3.31042173548439037739659126742769879190114783912250396476966465`50.*^-53*
  CF, 
 (-7.52368576246452358499225288051749725432079054346023628356742`50.*^-55*I)*
  CF, 1.671930169436560796664945084559443834293509009657830285237203815293208\
6298566058`50.*^-56*CF, (3.63463080312295825361944583599879094411632393403876\
148964609645843679986877157`50.*^-58*I)*CF, 
 -7.7332570279211877736583953957421083917368594341250244460555243796527656782\
37`50.*^-60*CF, 
 (
   -1.61109521415024745284549904077960591494517904877604675959490091242765951\
629`50.*^-61*I)*CF, 
 3.287949416633158067031630695468583499888120507706217876724287576382978604`5\
0.*^-63*CF, 
 (
   6.5758988332663161340632613909371669997762410154124357534485751527659573`50.\
*^-65*I)*CF, 
 -1.28939192809143453609083556685042490191691000302204622616638728485607`50.*^\
-66*CF, 
 (
   -2.479599861714297184790068397789278657532519236580858127243052470877`50.*^\
-68*I)*CF, 
 4.67849030512131544300012905243260124062739478600161910800575937902`50.*^-70*
  CF, 
 (8.663870935409843412963201948949261556717397751854850200010665517`50.*^-72*
   I)*CF, 
 -1.57524926098360789326603671799077482849407231851906367272921192`50.*^-73*
  CF, 
 (-2.812945108899299809403636996412097908025129140212613701302164`50.*^-75*I)*
  CF, 4.934991419121578612988836835810698084254612526688795967196779173326114\
68649531`50.*^-77*CF, 
 (8.5086058950372045051531669582943070418182974598082689089599640919415770456\
81`50.*^-79*I)*CF, 
 -1.4421365923791872042632486369990350918336097389505540523660956088036571263\
9`50.*^-80*CF, 
 (
   -2.403560987298645340438747728331725153056016231584256753943492681339428544`\
50.*^-82*I)*CF, 
 3.9402639136043366236700782431667625459934692321053389408909716087531615`50.\
*^-84*CF, 
 (
   6.35526437678118810269367458575284281611849876146022409821124453024704`50.*^\
-86*I)*CF, 
 -1.0087721232986012861418531088496575898600791684857498568589277032138`50.*^\
-87*CF, 
 (
   -1.57620644265406450959664548257758998415637370075898415134207453627`50.*^\
-89*I)*CF, 
 2.424932988698560783994839203965523052548267231936898694372422363`50.*^-91*
  CF, 
 (3.6741408919675163393861200060083682614367685332377252945036702`50.*^-93*I)*
  CF, -5.48379237607091990953152239702741531557726646751899297687114779141770\
6160029608`50.*^-95*CF, (-8.0644005530454704551934152897461989934959800992926\
367306928670933259760458603`50.*^-97*I)*CF, 
 1.16875370333992325437585728836901434688347537670907778705693725990231536896\
5`50.*^-98*CF, 
 (
   1.6696481476284617919655104119557347812621076810129682672241960855747362414`\
50.*^-100*I)*CF, 
 -2.35161710933586167882466255205033067783395448029995530594957195151371302`5\
0.*^-102*CF, 
 (
   -3.266134874077585665034253544514348163658270111527715702707738821546823`50.\
*^-104*I)*CF, 
 4.4741573617501173493619911568689700872031097418187886338462175637628`50.*^-\
106*CF, 
 (
   6.04615859695961803967836642820131092865285100245782247817056427536`50.*^-\
108*I)*CF, 
 -8.061544795946157386237821904268414571537134669943763304227419034`50.*^-110*
  CF, 
 (-1.06072957841396807713655551371952823309699140393996885581939724`50.*^-111*
   I)*CF, 
 1.377570881057101398878643524311075627398690134986972540025191`50.*^-113*CF, 
 (1.7661165141757710242033891337321482402547309422909904359297323364807991520\
5206`50.*^-115*I)*CF, 
 -2.2355905242731278787384672578887952408287733446721397923161168816212647494\
33`50.*^-117*CF, 
 (-2.794488155341409848423084072360994051035966680840174740395146102026580936\
8`50.*^-119*I)*CF, 
 3.44998537696470351657170873130986919880983540844466017332734086669948264`50.\
*^-121*CF, 
 (
   4.207299240200857947038669184524230730255896839566658747960171788657906`50.\
*^-123*I)*CF, 
 -5.0690352291576601771550231138846153376577070356224804192291226369372`50.*^\
-125*CF, 
 (
   -6.03456574899721449661312275462454206864012742336009573717752694873`50.*^\
-127*I)*CF, 
 7.099489116467311172486026770146520080753091086305994984914737587`50.*^-129*
  CF, 
 (8.2552199028689664796349148490075814892477803329139476568776018`50.*^-131*
   I)*CF, 
 -9.48875850904478905705162626322710516005491992288959500790529`50.*^-133*CF, 
 (-1.078268012391453301937684802639443768188059082146544887261964713303873045\
895497`50.*^-134*I)*CF, 
 1.21153709257466663139065708161735254852590908106353358119321877899311578190\
5`50.*^-136*CF, 
 (1.3461523250829629237673967573526139428065656456261484235480208655479064243\
4`50.*^-138*I)*CF, 
 -1.479288269321937278865271161925949387699522687501262003898924028074622444`\
50.*^-140*CF, 
 (
   -1.6079220318716709552883382194847275953255681385883282651075261174724157`\
50.*^-142*I)*CF, 
 1.72894842136738812396595507471476085518878294471863254312637216932517`50.*^\
-144*CF, 
 (
   1.83930683124190225953825007948378814381785419650918355651741720141`50.*^-\
146*I)*CF, 
 -1.9361124539388444837244737678776717303345833647465090068604391594`50.*^-148\
*CF, 
 (-2.01678380618629633721299350820590805243185767161094688214629079`50.*^-150*
   I)*CF, 
 2.079158563078656017745354132171039229311193475887574105305454`50.*^-152*CF, 
 (2.1215903704884245079034225838479992135828504855995654135769943099300211284\
1495`50.*^-154*I)*CF, 
 -2.1430205762509338463670935190383830440230812985854196096737316261919405337\
52`50.*^-156*CF, 
 (-2.143020576250933846367093519038383044023081298585419609673731626191940533\
8`50.*^-158*I)*CF, 
 2.12180255074349885778920150399839905348819930553011842541953626355637677`50.\
*^-160*CF, 
 (
   2.080198579160292997832550494116077503419803240715802377862290454467036`50.\
*^-162*I)*CF}


==> attachedfiles/B2 <==
{(1.2361111111111111111111111111111111111111111111111111111111111111111111111\
1111`50.*I)*CA*CF - (0.708333333333333333333333333333333333333333333333333333\
33333333333333333333333`50.*I)*CF^2 + 
  (0.916666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CA*CF*L + (0.75`50.*I)*CF^2*L - 
  (0.027777777777777777777777777777777777777777777777777777777777777777777777\
77777`50.*I)*CF*nf - (0.16666666666666666666666666666666666666666666666666666\
666666666666666666666667`50.*I)*CF*L*nf - 
  (0.166666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CA*CF*irrational[Pi^2] + 
  (0.222222222222222222222222222222222222222222222222222222222222222222222222\
22223`50.*I)*CF^2*irrational[Pi^2], 
 -0.9490740740740740740740740740740740740740740740740740740740740740740740740\
7407`50.*CA*CF + 1.6990740740740740740740740740740740740740740740740740740740\
7407407407407407407`50.*CF^2 - 0.30555555555555555555555555555555555555555555\
555555555555555555555555555555556`50.*CA*CF*L - 
  0.4722222222222222222222222222222222222222222222222222222222222222222222222\
2223`50.*CF^2*L + 0.046296296296296296296296296296296296296296296296296296296\
2962962962962962963`50.*CF*nf + 0.0555555555555555555555555555555555555555555\
5555555555555555555555555555555556`50.*CF*L*nf + 
  0.1111111111111111111111111111111111111111111111111111111111111111111111111\
1111`50.*CA*CF*irrational[Pi^2] - 0.16666666666666666666666666666666666666666\
666666666666666666666666666666666667`50.*CF^2*irrational[Pi^2], 
 (-0.376157407407407407407407407407407407407407407407407407407407407407407407\
40741`50.*I)*CA*CF + (0.77459490740740740740740740740740740740740740740740740\
740740740740740740740741`50.*I)*CF^2 - 
  (0.076388888888888888888888888888888888888888888888888888888888888888888888\
88889`50.*I)*CA*CF*L - (0.149305555555555555555555555555555555555555555555555\
55555555555555555555555556`50.*I)*CF^2*L + 
  (0.015046296296296296296296296296296296296296296296296296296296296296296296\
2963`50.*I)*CF*nf + (0.013888888888888888888888888888888888888888888888888888\
88888888888888888888889`50.*I)*CF*L*nf + 
  (0.041666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CA*CF*irrational[Pi^2] - 
  (0.066666666666666666666666666666666666666666666666666666666666666666666666\
66667`50.*I)*CF^2*irrational[Pi^2], 0.1025`50.*CA*CF - 
  0.2225439814814814814814814814814814814814814814814814814814814814814814814\
8148`50.*CF^2 + 0.01527777777777777777777777777777777777777777777777777777777\
777777777777777778`50.*CA*CF*L + 0.034305555555555555555555555555555555555555\
55555555555555555555555555555555555`50.*CF^2*L - 
  0.0033796296296296296296296296296296296296296296296296296296296296296296296\
2963`50.*CF*nf - 0.0027777777777777777777777777777777777777777777777777777777\
7777777777777777778`50.*CF*L*nf - 0.01111111111111111111111111111111111111111\
111111111111111111111111111111111111`50.*CA*CF*irrational[Pi^2] + 
  0.0185185185185185185185185185185185185185185185185185185185185185185185185\
1852`50.*CF^2*irrational[Pi^2], 
 (0.0215682870370370370370370370370370370370370370370370370370370370370370370\
3704`50.*I)*CA*CF - (0.048080246913580246913580246913580246913580246913580246\
91358024691358024691358`50.*I)*CF^2 + 
  (0.002546296296296296296296296296296296296296296296296296296296296296296296\
2963`50.*I)*CA*CF*L + (0.0062962962962962962962962962962962962962962962962962\
9629629629629629629629629`50.*I)*CF^2*L - 
  (0.000601851851851851851851851851851851851851851851851851851851851851851851\
85185`50.*I)*CF*nf - (0.00046296296296296296296296296296296296296296296296296\
296296296296296296296296`50.*I)*CF*L*nf - 
  (0.002314814814814814814814814814814814814814814814814814814814814814814814\
81481`50.*I)*CA*CF*irrational[Pi^2] + 
  (0.003968253968253968253968253968253968253968253968253968253968253968253968\
25397`50.*I)*CF^2*irrational[Pi^2], 
 -0.0037225056689342403628117913832199546485260770975056689342403628117913832\
1996`50.*CA*CF + 0.0084197947035957240038872691933916423712342079689018464528\
6686103012633624879`50.*CF^2 - 0.00036375661375661375661375661375661375661375\
661375661375661375661375661375662`50.*CA*CF*L - 
  0.0009674981103552532123960695389266817838246409674981103552532123960695389\
2668`50.*CF^2*L + 0.000089758125472411186696900982615268329554043839758125472\
41118669690098261527`50.*CF*nf + 0.000066137566137566137566137566137566137566\
13756613756613756613756613756613757`50.*CF*L*nf + 
  0.0003968253968253968253968253968253968253968253968253968253968253968253968\
254`50.*CA*CF*irrational[Pi^2] - 0.000694444444444444444444444444444444444444\
44444444444444444444444444444444445`50.*CF^2*irrational[Pi^2], 
 (-0.000545191543052406147644242882338120433358528596623834719072814310909549\
00479`50.*I)*CA*CF + (0.00124359973840542977920151011609817354337384571700520\
302183189560362651821457`50.*I)*CF^2 - 
  (0.000045469576719576719576719576719576719576719576719576719576719576719576\
71957`50.*I)*CA*CF*L - (0.000128171060090702947845804988662131519274376417233\
56009070294784580498866214`50.*I)*CF^2*L + 
  (0.000011564232174351221970269589317208364827412446460065507684555303602922\
65055`50.*I)*CF*nf + 
  (
    8.2671957671957671957671957671957671957671957671957671957671957671957672`\
50.*^-6*I)*CF*L*nf + (0.00005787037037037037037037037037037037037037037037037\
037037037037037037037037`50.*I)*CA*CF*irrational[Pi^2] - 
  (0.000102880658436213991769547325102880658436213991769547325102880658436213\
99177`50.*I)*CF^2*irrational[Pi^2], 
 0.00006947062962579701682750309608460276134753333040055136301042070757364282\
182`50.*CA*CF - 0.00015923510329710792148853793264644024701133964592434400110\
556993063081918378`50.*CF^2 + 
  5.05217519106407995296884185773074661963550852439741328630217519106407996`5\
0.*^-6*CA*CF*L + 0.0000149410973237031438089639147840206041264242322443380644\
4388454970465552476`50.*CF^2*L - 
  1.31407587040303089685805735188451237833953883336599385982102031484747535`5\
0.*^-6*CF*nf - 
  9.1857730746619635508524397413286302175191064079952968841857730746619636`50.\
*^-7*CF*L*nf - 
  7.34861845972957084068195179306290417401528512639623750734861845972957084`5\
0.*^-6*CA*CF*irrational[Pi^2] + 0.0000132275132275132275132275132275132275132\
2751322751322751322751322751322751`50.*CF^2*irrational[Pi^2], 
 (
    7.83564551843420103687173478052792741631239993547879665289592223328680875`\
50.*^-6*I)*CA*CF - (0.0000180085765403881847990355590926683561268259345020913\
8459747345276865727021`50.*I)*CF^2 + 
  (
    5.0521751910640799529688418577307466196355085243974132863021751910640799`\
50.*^-7*I)*CA*CF*L + 
  (
    1.55611370062428263486464544665602866661067719268777469835670893871952073`\
50.*^-6*I)*CF^2*L - 
  (
    1.3370403030896858057351884512378339538833365993859821020314847475341303`\
50.*^-7*I)*CF*nf - 
  (
    9.185773074661963550852439741328630217519106407995296884185773074661963`50.\
*^-8*I)*CF*L*nf - 
  (
    8.2671957671957671957671957671957671957671957671957671957671957671957672`\
50.*^-7*I)*CA*CF*irrational[Pi^2] + 
  (
    1.50312650312650312650312650312650312650312650312650312650312650312650312`\
50.*^-6*I)*CF^2*irrational[Pi^2], 
 -7.9325623398962611190712307702313581208348992005664551225985676309015521`50.\
*^-7*CA*CF + 
  1.8254440195528009913533534266390208481359807720369290166069198057465255`50.\
*^-6*CF^2 - 
  4.592886537330981775426219870664315108759553203997648442092886537330982`50.\
*^-8*CA*CF*L - 
  1.4652591387199371807356415341023325631310239294847279455264063248671234`50.\
*^-7*CF^2*L + 
  1.23236129128385020640912896805152697408589664481920374176266432158688`50.*^\
-8*CF*nf + 
  8.35070279514723959168403612848057292501736946181390625835070279514724`50.*^\
-9*CF*L*nf + 
  8.35070279514723959168403612848057292501736946181390625835070279514724`50.*^\
-8*CA*CF*irrational[Pi^2] - 
  1.5309621791103272584754066235547717029198510679992161473642955124436606`50.\
*^-7*CF^2*irrational[Pi^2], 
 (
    -7.28481636966349652864588056771926204472885696815597994176421432097365`50.\
*^-8*I)*CA*CF + 
  (
    1.6769705879631454842323463485494940936689788732051067723696806619299835`\
50.*^-7*I)*CF^2 - 
  (
    3.82740544777581814618851655888692925729962766999804036841073878110915`50.\
*^-9*I)*CA*CF*L - 
  (
    1.259323336744372498741586444007479761848849551270587024956112658533694`50.\
*^-8*I)*CF^2*L + 
  (
    1.03856594106313522699605752355471771857854910604630021016104068853788`50.\
*^-9*I)*CF*nf + 
  (
    6.9589189959560329930700301070671441041811412181782552152922523292893`50.*^\
-10*I)*CF*L*nf + 
  (
    7.65481089555163629237703311777385851459925533999608073682147756221831`50.\
*^-9*I)*CA*CF*irrational[Pi^2] - 
  (
    1.413195857640302084746529190973635418079862524306968751413195857640302`50.\
*^-8*I)*CF^2*irrational[Pi^2], 
 6.12317467347162741065686676183994233019833752986193690341946197753761`50.*^\
-9*CA*CF - 
  1.409156938915963306802641956921426145210313309425723482452483496428856`50.\
*^-8*CF^2 + 
  2.944158036750629343221935814528407120999713592306184898777491370084`50.*^-\
10*CA*CF*L + 
  9.9566250043858854800999076476685287627431902909511720453864729342338`50.*^\
-10*CF^2*L - 
  8.063836114643332117216257767064984538868679419486636960521101071908`50.*^-\
11*CF*nf - 
  5.353014612273871533130792390051649310908570167829427088686347945607`50.*^-\
11*CF*L*nf - 
  6.4236175347286458397569508680619791730902842013953125064236175347286`50.*^\
-10*CA*CF*irrational[Pi^2] + 
  1.19295754216389137024057658978293898928819563740198660833581468502103`50.*^\
-9*CF^2*irrational[Pi^2], 
 (
    4.7448402565813197040781817463000383446686013513558008937315008574629`50.*^\
-10*I)*CA*CF - 
  (
    1.09117967499862610777709641367882156928648209413153023188049743064246`50.\
*^-9*I)*CF^2 + 
  (
    2.102970026250449530872811296091719372142652565932989213412493835774`50.*^\
-11*I)*CA*CF*L + 
  (
    7.289398446907163939690496026576172180127307891959466134849834043057`50.*^\
-11*I)*CF^2*L - 
  (
    5.80540177076797422941578609543801318516902756296519499806512617335`50.*^\
-12*I)*CF*nf - 
  (
    3.82358186590990823795056599289403522207755011987816220620453424686`50.*^\
-12*I)*CF*L*nf - 
  (
    4.970656425682880709335735790762245788700815155841610868065894520921`50.*^\
-11*I)*CA*CF*irrational[Pi^2] + 
  (
    9.278558661274710657426706809422858805574854957571006953723003105719`50.*^\
-11*I)*CF^2*irrational[Pi^2], 
 -3.410937636004995285473898119461979596101919534051323610518216165487`50.*^-\
11*CA*CF + 
  7.836287619205556763648589870874699808611582082385588409605844610881`50.*^-\
11*CF^2 - 
  1.40198001750029968724854086406114624809510171062199280894166255719`50.*^-12\
*CA*CF*L - 
  4.96940439254885537585788540007748195210350926474896567120627598656`50.*^-12\
*CF^2*L + 
  3.896411996689144585340100583234873988212360598352031962513192042`50.*^-13*
   CF*nf + 
  2.5490545772732721586337106619293568147183667465854414708030228313`50.*^-13*
   CF*L*nf + 
  3.56867640818258102208719492670109954060571344521961805912423196374`50.*^-12\
*CA*CF*irrational[Pi^2] - 
  6.69126826534233941641349048756456163863571270978678386085793493201`50.*^-12\
*CF^2*irrational[Pi^2], 
 (
    -2.28670886832398242770133215301352794801661180948109703206974091808`50.*^\
-12*I)*CA*CF + 
  (
    5.24714193139224167488206816358399098426903090248579611085466798292`50.*^\
-12*I)*CF^2 - 
  (8.762375109376873045303380400382164050594385691387455055885390982`50.*^-14*
    I)*CA*CF*L - 
  (
    3.1698886024732228058590115110901790418628665625642781350095787569`50.*^-13\
*I)*CF^2*L + 
  (2.449482132848534964937081339197741314143430545546947663349779752`50.*^-14*
    I)*CF*nf + 
  (1.59315911079579509914606916370584800919897921661590091925188927`50.*^-14*
    I)*CF*L*nf + 
  (
    2.3897386661936926487191037455587720137984688249238513788778339043`50.*^-13\
*I)*CA*CF*irrational[Pi^2] - 
  (
    4.4983316069528332211183129328165120259735883763272496543582755845`50.*^-13\
*I)*CF^2*irrational[Pi^2], 
 1.4363081874452114558668542853961105151863373985111240342208734052`50.*^-13*
   CA*CF - 
  3.2913511344608057594232741624621438878563225868278728214495635111`50.*^-13*
   CF^2 + 
  5.15433829963345473253140023551892002976140334787497356228552411`50.*^-15*
   CA*CF*L + 
  1.899921386607408185572895500114352471887753573087436155137856332`50.*^-14*
   CF^2*L - 
  1.44822205789611996829814966510458069463661533459677844519653429`50.*^-15*
   CF*nf - 
  9.3715241811517358773298186100344000541116424506817701132464075`50.*^-16*CF*
   L*nf - 
  1.499443868984277740372770977605504008657862792109083218119425195`50.*^-14*
   CA*CF*irrational[Pi^2] + 
  2.832282863636969065148567402143729794131518607317157189781136479`50.*^-14*
   CF^2*irrational[Pi^2], 
 (8.48625851613763278424395307224394190027578141370171277656818366`50.*^-15*
    I)*CA*CF - 
  (1.941864364484568346735809051398690076370462489581678124351433887`50.*^-14*
    I)*CF^2 + 
  (2.8635212775741415180730001308438444609785574154860964234919579`50.*^-16*
    I)*CA*CF*L + 
  (1.07395122300869662044728070797679128078485128153718560608644668`50.*^-15*
    I)*CF^2*L - 
  (8.081833671109430903652258242132062501276380109066522882701604`50.*^-17*I)*
   CF*nf - 
  (5.20640232286207548740545478335244447450646802815653895180356`50.*^-17*I)*
   CF*L*nf - 
  (8.8508839488655283285892731316991556066609956478661162180660515`50.*^-16*
    I)*CA*CF*irrational[Pi^2] + 
  (1.67700959031136326225902017232194527284103075433252728342304134`50.*^-15*
    I)*CF^2*irrational[Pi^2], 
 -4.7333730502013500910045937191843429225270181341444235938339181`50.*^-16*CA*
   CF + 
  1.08149358912239462515983551156405149213281482900250245951329402`50.*^-15*
   CF^2 - 
  1.507116461881127114775263226759918137357135481834787591311557`50.*^-17*CA*
   CF*L - 
  5.743998037159850903224206613044227207527683712024116226721038`50.*^-17*
   CF^2*L + 4.270563924415952962122356724418056178688746474311226933381502092\
496039406576139`50.*^-18*CF*nf + 2.740211748874776572318660412290760249740246\
330608704711475557739122727604583418`50.*^-18*CF*L*nf + 
  4.932381147974597830173588742123368449532443395095668480656004`50.*^-17*CA*
   CF*irrational[Pi^2] - 
  9.371524181151735877329818610034400054111642450681770113246408`50.*^-17*
   CF^2*irrational[Pi^2], 
 (-2.500193625901851591595462733154232297628717950208223984118194`50.*^-17*I)*
   CA*CF + 
  (5.703793135705666284589628300518850611807314975949393963068985`50.*^-17*I)*
   CF^2 - (7.5355823094056355738763161337995906867856774091739379565577837825\
875009126044`50.*^-19*I)*CA*CF*L - (2.915385704603776080673815429716717307718\
062422913362604625548829522431694579666`50.*^-18*I)*CF^2*L + 
  (2.142893661510406415984285752243169090038096143629526535333736600375361104\
81239`50.*^-19*I)*CF*nf + (1.370105874437388286159330206145380124870123165304\
35235573777886956136380229171`50.*^-19*I)*CF*L*nf + 
  (2.603201161431037743702727391676222237253234014078269475901779852166591224\
354247`50.*^-18*I)*CA*CF*irrational[Pi^2] - 
  (4.958478402725786178481385507954709023339493360149084716003388921623152102\
058911`50.*^-18*I)*CF^2*irrational[Pi^2], 
 1.25418308690699596184250785106739820873008513143729595260913272127586137446\
2771`50.*^-18*CA*CF - 2.85680857485216434081129689517613452232818520489114449\
1246890217914595117950167`50.*^-18*CF^2 + 3.588372528288397892322055301809328\
8984693701948447323602656113250416671012402`50.*^-20*CA*CF*L + 
  1.4079009030077041599507868706656101769637765660891322443184715710874646279\
5654`50.*^-19*CF^2*L - 1.0236958857757810437403612311222284606455908910834106\
603528302438105881470638`50.*^-20*CF*nf - 
  6.5243136877970870769491914578351434517624912633540588368465660455303038204\
37`50.*^-21*CF*L*nf - 1.30486273755941741538983829156702869035249825267081176\
736931320910606076408734`50.*^-19*CA*CF*irrational[Pi^2] + 
  2.4911015898861605202896912839006911361274966641897315558868706719297523678\
0311`50.*^-19*CF^2*irrational[Pi^2], 
 (5.9900835886766145158929360556437268352653105503243430227662480375236994226\
975`50.*^-20*I)*CA*CF - (1.36233152644762157066000330715917559289708068391447\
497775620244044343194806925`50.*^-19*I)*CF^2 + 
  (1.631078421949271769237297864458785862940622815838514709211641511382575955\
109`50.*^-21*I)*CA*CF*L + 
  (6.484473476962956199331634342249388002203330868502523777216468641486080775\
978`50.*^-21*I)*CF^2*L - 
  (4.666643104120899552284594834559375530727401759600945271927836988489306254\
88`50.*^-22*I)*CF*nf - 
  (2.965597130816857762249632480834156114437496028797299471293893657059229009\
29`50.*^-22*I)*CF*L*nf - 
  (6.227753974715401300724228209751727840318741660474328889717176679824380919\
508`50.*^-21*I)*CA*CF*irrational[Pi^2] + 
  (1.191396412554250683616808874909026195539237535047262918032851190922925045\
471`50.*^-20*I)*CF^2*irrational[Pi^2], 
 -2.7302122640985171780767607922649323005230429402720357128250089937797594088\
38`50.*^-21*CA*CF + 
  6.1998229181687910913922359663313591054478700802237890537537004352479403320\
09`50.*^-21*CF^2 - 
  7.0916453128229207358143385411251559258287948514718030835288761364459824135`\
50.*^-23*CA*CF*L - 
  2.8545742834637594443594153713686787881670571222133795457886702224421269580\
7`50.*^-22*CF^2*L + 
  2.0343143519236908806174800342549704686022234602078055318064029640421760547`\
50.*^-23*CF*nf + 
  1.2893900568768946792389706438409374410597808820857823788234320248083604388`\
50.*^-23*CF*L*nf + 
  2.8366581251291682943257354164500623703315179405887212334115504545783929654\
1`50.*^-22*CA*CF*irrational[Pi^2] - 
  5.4369280731642392307909928815292862098020760527950490307054717046085865170\
3`50.*^-22*CF^2*irrational[Pi^2], 
 (
    -1.1900323736598879808842119870292527322810342036468634937712280512210439\
1225`50.*^-22*I)*CA*CF + 
  (2.698245140257758281524127171457389121358612704298674897393297684918945215\
92`50.*^-22*I)*CF^2 - 
  (
    2.954852213676216973255974392135481635761997854779917951470365056852492673`\
50.*^-24*I)*CA*CF*L - 
  (1.203447604524752314705862619134838491823572551058592327181329892196810612\
3`50.*^-23*I)*CF^2*L + 
  (
    8.49666002153931955748506470465835134394013217135332138219245288087030996`\
50.*^-25*I)*CF*nf + 
  (
    5.37245857032039449682904434933723933774908700869075991176430010336816849`\
50.*^-25*I)*CF*L*nf + 
  (1.235665471173690734270680200347565047682290011998874779705789023774678753\
9`50.*^-23*I)*CA*CF*irrational[Pi^2] - 
  (2.372477704653486209799705984667324891549996823037839577035114925647383207\
4`50.*^-23*I)*CF^2*irrational[Pi^2], 
 4.970000224004496478364509514122439132815737618530525118257269196494839887`5\
0.*^-24*CA*CF - 
  1.1251940024502597257913839090670983114285644614181109826445130225204830782`\
50.*^-23*CF^2 + 
  1.18194088547048678930238975685419265430479914191196718058814602274099707`5\
0.*^-25*CA*CF*L + 
  4.86760843786430573239168577297793222570374192800838457323273238373576532`5\
0.*^-25*CF^2*L - 
  3.4061387335831301109896141174798097401329211635099417840585662655354188`50.\
*^-26*CF*nf - 
  2.1489834281281577987316177397348957350996348034763039647057200413472674`50.\
*^-26*CF*L*nf - 
  5.15756022750757871695588257536374976423912352834312951529372809923344175`5\
0.*^-25*CA*CF*irrational[Pi^2] + 
  9.91838505289918984029977418339182646969062216989063368325716942160277261`5\
0.*^-25*CF^2*irrational[Pi^2], 
 (
    1.99227986097434964841699676349635404953012016884627720844573275397655347`\
50.*^-25*I)*CA*CF - 
  (
    4.5038123769368308721579397257321768258715542271196590977665084517734913`\
50.*^-25*I)*CF^2 + 
  (
    4.545926482578795343470729834054587131941535161199873771492869318234604`50.\
*^-27*I)*CA*CF*L + 
  (
    1.8920256512877521844140693962242684571410438147986788296152680030025435`\
50.*^-26*I)*CF^2*L - 
  (
    1.312702500377298757923435925041217375069737472656038141754164687978794`50.\
*^-27*I)*CF*nf - 
  (
    8.26532087741599153358314515282652205807551847490886140271430785133564`50.\
*^-28*I)*CF*L*nf - 
  (
    2.0663302193539978833957862882066305145188796187272153506785769628339109`\
50.*^-26*I)*CA*CF*irrational[Pi^2] + 
  (
    3.9795989409780699976511439624720291390733977842153777124180000765690137`\
50.*^-26*I)*CF^2*irrational[Pi^2], 
 -7.677973235460911848243522756302077841344557318513889626975863737932824`50.\
*^-27*CA*CF + 
  1.7331928186813707713658593882311392513852755537070891784666379499900068`50.\
*^-26*CF^2 - 
  1.68367647502918346054471475335355078960797598562958287833069234008689`50.*^\
-28*CA*CF*L - 
  7.07825083779424785334368476757086739632813379319597275049953482729657`50.*^\
-28*CF^2*L + 
  4.870931423485102111961788084682507723367286132992085146582189442831`50.*^-\
29*CF*nf + 
  3.0612299545985153828085722788246377992872290647810597787830769819761`50.*^\
-29*CF*L*nf + 
  7.95919788195613999530228792494405827814679556843075542483600015313803`50.*^\
-28*CA*CF*irrational[Pi^2] - 
  1.534988162948684141951155528382068382214024859625931403361228600962334`50.\
*^-27*CF^2*irrational[Pi^2], 
 (
    -2.8490019927858816606567550431351274462136892486367044807072840125203`50.*^\
-28*I)*CA*CF + 
  (
    6.42208118295044279368323108035799233958754275962918131042569495626405`50.\
*^-28*I)*CF^2 - 
  (
    6.013130267961369501945409833405538534314199948677081708323901214596`50.*^\
-30*I)*CA*CF*L - 
  (
    2.5522755765201669870661800341976798454058744663933091300922032973803`50.*^\
-29*I)*CF^2*L + 
  (
    1.742621927102801887889422522668031249121840052466542438318975700719`50.*^\
-30*I)*CF*nf + 
  (
    1.093296412356612636717347242437370642602581808850378492422527493563`50.*^\
-30*I)*CF*L*nf + 
  (
    2.9519003133628541191368375545809007350269708838960219295408242326199`50.*^\
-29*I)*CA*CF*irrational[Pi^2] - 
  (
    5.7002212947696493335056173467769117641900127413164561398029709319556`50.*^\
-29*I)*CF^2*irrational[Pi^2], 
 1.019278335837795269944996020329808396194493427917945223478067478285`50.*^-29\
*CA*CF - 
  2.2944112401361397647921516700979886490296351009876496972998991309414`50.*^\
-29*CF^2 + 
  2.07349319584874810411910683910535811528075860299209714080134524641`50.*^-31\
*CA*CF*L + 
  8.88183888731616613013462985180662855396363712324238079682429930744`50.*^-31\
*CF^2*L - 
  6.0186707259708772778916304652043123677615093350024375134918880902`50.*^-32*
   CF*nf - 
  3.7699876288159056438529215256461056641468338236219948014569913571`50.*^-32*
   CF*L*nf - 
  1.055596536068453580278818027180909585961113470614158544407957579992`50.*^-\
30*CA*CF*irrational[Pi^2] + 
  2.040819969732343588539048185883091866191486043187373185855384654651`50.*^-\
30*CF^2*irrational[Pi^2], 
 (
    3.52050137648954306965863655306515141139515040506617244485064122138`50.*^-31\
*I)*CA*CF - 
  (
    7.91391811753304193217963285051418039133724921939198644322171312929`50.*^\
-31*I)*CF^2 + 
  (6.911643986162493680397022797017860384269195343306990469337817488`50.*^-33*
    I)*CA*CF*L + 
  (
    2.9866438293995937728238610754221469142403214651010407059038742333`50.*^-32\
*I)*CF^2*L - 
  (2.009215628997289176474871203897981984225381551210036309895277769`50.*^-33*
    I)*CF*nf - 
  (1.256662542938635214617640508548701888048944607873998267152330452`50.*^-33*
    I)*CF*L*nf - 
  (
    3.6443213745220421223911574747912354753419393628345949747417583119`50.*^-32\
*I)*CA*CF*irrational[Pi^2] + 
  (
    7.0535252410104041078538531770152944684037536054863128543388870552`50.*^-32\
*I)*CF^2*irrational[Pi^2], 
 -1.1753049085448990958862206682057512453518788505558666669416489595`50.*^-32*
   CA*CF + 
  2.6385130196529464855919730179447243563323592477098063600144972445`50.*^-32*
   CF^2 - 
  2.22956257618144957432162025710253560782877269138935176430252177`50.*^-34*
   CA*CF*L - 
  9.71550011985765630496884938805980376004496035045235768565906521`50.*^-34*
   CF^2*L + 
  6.49035909273544167383165701432194627577134415929373367946521`50.*^-35*CF*
   nf + 
  4.0537501385117264987665822856409738324159503479806395714591305`50.*^-35*CF*
   L*nf + 
  1.216125041553517949629974685692292149724785104394191871437739147`50.*^-33*
   CA*CF*irrational[Pi^2] - 
  2.356242268009941027408075953528816040091771139763746750910619598`50.*^-33*
   CF^2*irrational[Pi^2], 
 (-3.79678832505138349274849504535798205447552914072073355015552628`50.*^-34*
    I)*CA*CF + 
  (8.51255548107979833072378094337507948908408924931747656884073855`50.*^-34*
    I)*CF^2 - 
  (6.967383050567029919755063303445423774464914660591724263445381`50.*^-36*I)*
   CA*CF*L - 
  (3.0606379777472878143382662249512805087650060588889008054237769`50.*^-35*
    I)*CF^2*L + 
  (2.030876376726252428345027310651155720184024184120425003720547`50.*^-36*I)*
   CF*nf + 
  (1.266796918284914530864556964262804322629984483743949866080978`50.*^-36*I)*
   CF*L*nf + 
  (3.9270704466832350456801265892146934001529518996062445848510326`50.*^-35*
    I)*CA*CF*irrational[Pi^2] - 
  (7.6161366238705164522281242942345568972663309568121107100141239`50.*^-35*
    I)*CF^2*irrational[Pi^2], 
 1.1881157007327106413920471486784070081597092840356158056978752`50.*^-35*CA*
   CF - 
  2.6604198856824501327818872922172283757730170446938719198053199`50.*^-35*
   CF^2 + 2.11132819714152421810759494043800720438330747290658311013496524594\
2622571082949`50.*^-37*CA*CF*L + 
  9.34670799510218250854778234497172843822713024773017376515086`50.*^-37*CF^2*
   L - 6.16167578194711354974582201109232474419715249066229058484635612438861\
54643525`50.*^-38*CF*nf - 3.8387785402573167601956271644327403716060135871028\
7838206357054121202237779129`50.*^-38*CF*L*nf - 
  1.228409132882341363262600692618476918913924347872921082260342`50.*^-36*CA*
   CF*irrational[Pi^2] + 
  2.38455890500689794045093075625939637200938255763567033615243`50.*^-36*CF^2*
   irrational[Pi^2], (3.60498954644266160236178946335975851200027253234669314\
8772247387478687649460276`50.*^-37*I)*CA*CF - 
  (8.06225030875432802793331052774758027635666846027251216780765`50.*^-37*I)*
   CF^2 + (6.2097888151221300532576321777588447187744337438428915003969523460\
782714934859`50.*^-39*I)*CA*CF*L + (2.769578858609501903425567854991622188621\
57136098482538074421314514386191892051`50.*^-38*I)*CF^2*L - 
  (1.814333047101798814782613971236298335431907963077091780135424579481303435\
8702`50.*^-39*I)*CF*nf - (1.1290525118403872824104785777743354034135334079714\
348182539913356505948169974`50.*^-39*I)*CF*L*nf - 
  (3.725873289073278031954579306655306831264660246305734900238171407646962896\
09155`50.*^-38*I)*CA*CF*irrational[Pi^2] + 
  (7.238839533056654462083182652930310415028482764251142091891304449142670769\
54929`50.*^-38*I)*CF^2*irrational[Pi^2], 
 -1.0615849734308544210543768100197907994938520176938464904438426865383661376\
8782`50.*^-38*CA*CF + 2.37126709145656863540829098794743900259630227891425189\
239722433987305428026377`50.*^-38*CF^2 - 
  1.7742253757491800152164663365025270625069810696693975715419863845937918552\
82`50.*^-40*CA*CF*L - 
  7.9700587580346780433338395436040075945270278378728276686504578995384852210\
76`50.*^-40*CF^2*L + 
  5.1893946182467740399226718464649925744729270604081233783374727816257431244\
6`50.*^-41*CF*nf + 
  3.2258643195439636640299387936409582954672383084898137664399752447159851914\
2`50.*^-41*CF*L*nf + 1.096793868644947645770179189837925820458861024886536680\
5895915832034349650832`50.*^-39*CA*CF*irrational[Pi^2] - 
  2.1326547445873982001086817580181890953366742150571546567019836340066790987\
729`50.*^-39*CF^2*irrational[Pi^2], 
 (-3.036606353801081478301836287762652726700421400902556798740208095136343369\
163`50.*^-40*I)*CA*CF + 
  (6.774856508638657139730695816964876609587124559939819400162521742896243345\
649`50.*^-40*I)*CF^2 - 
  (
    4.928403821525500042267962045840352951408280749081659920949962179427199598`\
50.*^-42*I)*CA*CF*L - 
  (2.229279019277611919477407479129848724561068917491518508424881978298416303\
47`50.*^-41*I)*CF^2*L + 
  (1.442962677326874399099811687014441001213189269824918900376258767973706779\
8`50.*^-42*I)*CF*nf + 
  (
    8.960734220955454622305385537891550820742328634693927128999931235322181087`\
50.*^-43*I)*CF*L*nf + 
  (3.136256977334409117806884938262042787259815022142874495149975932362763380\
55`50.*^-41*I)*CA*CF*irrational[Pi^2] - 
  (6.102986550488579904921505825807218396829910313359107125697250462976188199\
99`50.*^-41*I)*CF^2*irrational[Pi^2], 
 8.4442818215978062210970759037119844506082934185725037529630773333477973692`\
50.*^-42*CA*CF - 
  1.8817950095278167231308443080404547704428889631569825607151039151420354018\
3`50.*^-41*CF^2 + 
  1.332001032844729741153503255632527824704940742995043221878368156601945837`\
50.*^-43*CA*CF*L + 
  6.065473266997331144124850919826776266470599348852040803524704191515694509`\
50.*^-43*CF^2*L - 
  3.90363939055096199052221060584635167846233657549871389212784115782743341`5\
0.*^-44*CF*nf - 
  2.42182005971769043846091501024095968128171044180916949432430573927626516`5\
0.*^-44*CF*L*nf - 
  8.718552214983685578459294036867454852614157590513010179567500661394554571`\
50.*^-43*CA*CF*irrational[Pi^2] + 
  1.6978233260757703494894414703373464712985464781525335612841974972189395744`\
50.*^-42*CF^2*irrational[Pi^2], 
 (
    2.284620086912428316917939380295094248589212451765272537639351715126398818`\
50.*^-43*I)*CA*CF - 
  (
    5.085497311929133450843343593781470792552126442822746413909085731884635676`\
50.*^-43*I)*CF^2 + 
  (
    3.5052658759071835293513243569277048018551072184080084786272846226366996`\
50.*^-45*I)*CA*CF*L + 
  (
    1.60651966654703018869202607947645029960299974627534537203674109753104863`\
50.*^-44*I)*CF^2*L - 
  (
    1.0282052797770759048767516810592280346835641459229491657855369566379042`\
50.*^-45*I)*CF*nf - 
  (
    6.373210683467606417002407921686736003372922215287288142958699313884908`50.\
*^-46*I)*CF*L*nf - 
  (
    2.35808795288301437429089093102409232124798121965629661289471874613741608`\
50.*^-44*I)*CA*CF*irrational[Pi^2] + 
  (
    4.59524831843869467810532591686746195935504032548406519435893909503701594`\
50.*^-44*I)*CF^2*irrational[Pi^2], 
 -6.0181352958742227306688719590736831951876375380814216363572901968444559`50.\
*^-45*CA*CF + 
  1.33814358979226284007973230520465119911131128877052328468935082052652894`5\
0.*^-44*CF^2 - 
  8.98786122027482956243929322289155077398745440617438071442893492983769`50.*^\
-47*CA*CF*L - 
  4.145101549808395445587645259601548661824224632667303496659315951761751`50.\
*^-46*CF^2*L + 
  2.6386887375926471773913910786872139617411334062047961047268361289537`50.*^\
-47*CF*nf + 
  1.63415658550451446589805331325300923163408261930443285716889725997049`50.*^\
-47*CF*L*nf + 
  6.209795024917154970412602590361435080209513953356844857241809587887859`50.\
*^-46*CA*CF*irrational[Pi^2] - 
  1.2109100298588452192304575051204798406408552209045847471621528696381326`50.\
*^-45*CF^2*irrational[Pi^2], 
 (
    -1.544573318341272268945191161440208214404622597350597987744904820021776`50.\
*^-46*I)*CA*CF + 
  (
    3.430692951974184515219531451029618346974395333010003059053556940532428`50.\
*^-46*I)*CF^2 - 
  (
    2.2469653050687073906098233057228876934968636015435951786072337324594`50.*^\
-48*I)*CA*CF*L - 
  (
    1.04256474010025768351895316482310433914359522614243832956906454647388`50.\
*^-47*I)*CF^2*L + 
  (
    6.602097359065514372642616029985314539983208787286018001478830116003`50.*^\
-49*I)*CF*nf + 
  (
    4.085391463761286164745133283132523079085206548261082142922243149926`50.*^\
-49*I)*CF*L*nf + 
  (
    1.59330267086690160425060198042168400084323055382182203573967482847123`50.\
*^-47*I)*CA*CF*irrational[Pi^2] - 
  (
    3.10888326022810069122068679106670048945020595867672592339448747018776`50.\
*^-47*I)*CF^2*irrational[Pi^2], 
 3.8649263483174800092162737372001205052666961323777154693640888122751`50.*^-\
48*CA*CF - 
  8.5754703073199355406680683648556135528148802190644614715796731438391`50.*^\
-48*CF^2 + 
  5.48040318309440826978005684322655534999235024766730531367617983527`50.*^-50\
*CA*CF*L + 
  2.557796731087019513327223463493436284385688101279130990594651525148`50.*^-\
49*CF^2*L - 
  1.61151397368374747238137148194950853362487549596041198746937778822`50.*^-50\
*CF*nf - 
  9.9643694238080150359637397149573733636224549957587369339566906096`50.*^-51*
   CF*L*nf - 
  3.985747769523206014385495885982949345448981998303494773582676243831`50.*^-\
49*CA*CF*irrational[Pi^2] + 
  7.781698026211973647133587205966710626828964853830632653185225047479`50.*^-\
49*CF^2*irrational[Pi^2], 
 (
    9.43479425617434773911186508931887992073329346508118770634316646516`50.*^-50\
*I)*CA*CF - 
  (
    2.091236419794409050068594517930539272771960479221452486432684646537`50.*^\
-49*I)*CF^2 + 
  (
    1.3048579007367638737571563912444179404743691065874536461133761513`50.*^-51\
*I)*CA*CF*L + 
  (6.124731940205159437894283189296723492407124786619198635284223386`50.*^-51*
    I)*CF^2*L - 
  (3.839762400330863600634774429730960616726920810958962423944651392`50.*^-52*
    I)*CF*nf - 
  (2.372468910430479770467557074989850800862489284704461174751593002`50.*^-52*
    I)*CF*L*nf - 
  (
    9.7271225327649670589169840074583882835362060672882908164815313093`50.*^-51\
*I)*CA*CF*irrational[Pi^2] + 
  (
    1.90018207616804007662564338750349910655125885965631727577778751159`50.*^\
-50*I)*CF^2*irrational[Pi^2], 
 -2.2482371898587690972015570133246308700337104832330043858042153846`50.*^-51*
   CA*CF + 
  4.9782536330449995731244155852831905382571301906191431312630202185`50.*^-51*
   CF^2 - 
  3.03455325752735784594687532847539055924271885252896196770552593`50.*^-53*
   CA*CF*L - 
  1.432242692440811009144482014143421989116792957140207576357665445`50.*^-52*
   CF^2*L + 
  8.935939070036768045298107657093040758869377472714400237127417`50.*^-54*CF*
   nf + 
  5.5173695591406506289943187790461646531685797318708399412827744`50.*^-54*CF*
   L*nf + 
  2.317295214839073264177613887199389154330803487385752775338765258`50.*^-52*
   CA*CF*irrational[Pi^2] - 
  4.529258829003643198165336234071533347101115907163062242707586641`50.*^-52*
   CF^2*irrational[Pi^2], 
 (-5.23259723204765038305075550841335504720337704231830403652915481`50.*^-53*
    I)*CA*CF + 
  (1.157514200308671305367509583729478988011956302518790726468445019`50.*^-52*
    I)*CF^2 - 
  (6.896711948925813286242898473807705816460724664838549926603468`50.*^-55*I)*
   CA*CF*L - 
  (3.2726034399513006979557852525912324634654273914100383315592721`50.*^-54*
    I)*CF^2*L + 
  (2.032252329366665270681927832037833487270875975137735305747495`50.*^-55*I)*
   CF*nf + 
  (1.253947627077420597498708813419582875720131757243372713927903`50.*^-55*I)*
   CF*L*nf + 
  (5.3919747964329085692444478977042063655965665561465026698899841`50.*^-54*
    I)*CA*CF*irrational[Pi^2] - 
  (1.05443062685799100909669203332882257816110634875753829988959689`50.*^-53*
    I)*CF^2*irrational[Pi^2], 
 1.1901294178442941711431196052406426657056073042961553375538443`50.*^-54*CA*
   CF - 
  2.6301888972262245226179008247906964726176321245218132321407991`50.*^-54*
   CF^2 + 1.53260265531684739694286632751282351476904992551967776146743746517\
09005729475278`50.*^-56*CA*CF*L + 
  7.31047013914511714535562489398600264682700371032977227816812`50.*^-56*CF^2*
   L - 4.51899644281211844957166554420906915144482948654149246287597915395510\
0685326382`50.*^-57*CF*nf - 2.78655028239426799444157514093240639048918168276\
3050475395340618134879899391539`50.*^-57*CF*L*nf - 
  1.22608212425347791755429306201025881181523994041574220917395`50.*^-55*CA*
   CF*irrational[Pi^2] + 
  2.398856330061152447388834251759202023116773796465582583166424`50.*^-55*
   CF^2*irrational[Pi^2], 
 (2.64665770240773375195750708216829840726030719813609915140286`50.*^-56*I)*
   CA*CF - 
  (5.84364174741124223845684880685230554388718727817818105901188`50.*^-56*I)*
   CF^2 + (3.3317449028627117324844920163322250321066302728688646988422550869\
0039987970727`50.*^-58*I)*CA*CF*L + (1.59731358687643520558189844842679630625\
11882856957876625975192793850336177063`50.*^-57*I)*CF^2*L - 
  (9.829891197818048932292849084637631868990927612267471693817421903292440224\
8017`50.*^-59*I)*CF*nf - 
  (6.057718005204930422699076393331318240193873223397935816076827430727999781\
286`50.*^-59*I)*CF*L*nf - (2.725973102342218690214584376999093208087242950529\
071117234572343827599901578681`50.*^-57*I)*CA*CF*irrational[Pi^2] + 
  (5.335947349265619563824292823062054790298433009546266867778311821960408317\
983801`50.*^-57*I)*CF^2*irrational[Pi^2], 
 -5.7576286798380285246680543413976651770559149202585723478433842947152824040\
1344`50.*^-58*CA*CF + 1.27008131550395060186879479259012543559017943953197349\
5247538871770272723295147`50.*^-57*CF^2 - 
  7.0888189422610887925201957794302660257587878146146057422175640146817018717\
18`50.*^-60*CA*CF*L - 3.41535892353304770159686602209976221122096304445769247\
94991452337489617029778`50.*^-59*CF^2*L + 
  2.0926850077355850664096146035707714943308887527179214832308234978446725089\
3`50.*^-60*CF*nf + 
  1.2888761713201979622763992326236847319561432390208374076759207299421276130\
4`50.*^-60*CF*L*nf + 
  5.9288303880729106264714364700689497669982588994958520753092353577337870199\
82`50.*^-59*CA*CF*irrational[Pi^2] - 1.16106261766427833101732297538850266270\
38257011512710314147252575561999580798`50.*^-58*CF^2*irrational[Pi^2], 
 (-1.225850845158780597479033888713291971323839168512550486379504635116175642\
6666`50.*^-59*I)*CA*CF + (2.7016950171418556599649592915234507342460322770000\
721666676083548497820389199`50.*^-59*I)*CF^2 - 
  (1.476837279637726831775040787381305422033080794711376196295325836392021223\
27`50.*^-61*I)*CA*CF*L - 
  (7.149625237009547580448062570912838609428828541575117574002277363283208256\
78`50.*^-61*I)*CF^2*L + 
  (4.362192641741029044532176406957192433713121464069305093022541255945162623\
5`50.*^-62*I)*CF*nf + 
  (2.685158690250412421409165067966009858241965081293411265991501520712765860\
5`50.*^-62*I)*CF*L*nf + 
  (1.262024584417693838062307581944024633373723588207903295016005714734999954\
435`50.*^-60*I)*CA*CF*irrational[Pi^2] - 
  (2.472537961308134866407786282992374791915866621795075843296664257439999910\
729`50.*^-60*I)*CF^2*irrational[Pi^2], 
 2.55550807954540104163731414755799506867835733362120844074359128784143332768`\
50.*^-61*CA*CF - 
  5.6272371828188133830072235188050569484711439631458277871788370401073541287\
1`50.*^-61*CF^2 + 
  3.013953631913728228112328137512868208230777132064033053663930278351063721`\
50.*^-63*CA*CF*L + 
  1.4659600601799073041825189907369879927186332579145875404209061837211229604`\
50.*^-62*CF^2*L - 
  8.90719289951003634514025237299914591841856909081694369523593495217696088`5\
0.*^-64*CF*nf - 
  5.47991569438859677838605115911430583314686751284369646120714596063829767`5\
0.*^-64*CF*L*nf - 
  2.6303595333065264536253045563748667999104964061649743013794300611063828837`\
50.*^-62*CA*CF*irrational[Pi^2] + 
  5.1555046852807918491055969304947389278245729560833496307036829197685104521`\
50.*^-62*CF^2*irrational[Pi^2], 
 (
    5.218570018216988171932937025691267479632954197876536748462625005818363523`\
50.*^-63*I)*CA*CF - 
  (1.148145569507101522344524863318589994076377285724142820374388494337361193\
3`50.*^-62*I)*CF^2 + 
  (
    6.0279072638274564562246562750257364164615542641280661073278605567021275`\
50.*^-65*I)*CA*CF*L + 
  (
    2.94534591381106667047208380681380603472847634123564213717176987504580976`\
50.*^-64*I)*CF^2*L - 
  (
    1.7823518991844053684911148164596815679892382960821960217907215147621652`\
50.*^-65*I)*CF*nf - 
  (
    1.0959831388777193556772102318228611666293735025687392922414291921276595`\
50.*^-65*I)*CF*L*nf - 
  (
    5.37031738050082484281833013593201971648393016258682253198300304142553172`\
50.*^-64*I)*CA*CF*irrational[Pi^2] + 
  (
    1.053003407941338204474182379594513669898809835801337751369216282632457201`\
50.*^-63*I)*CF^2*irrational[Pi^2], 
 -1.04434041533906097276756505474839846279882792412089510645996586346398397`5\
0.*^-64*CA*CF + 
  2.2957412294677634286130160257615615294272331787566385546542621552163196`50.\
*^-64*CF^2 - 
  1.181942600750481658083265936279556160090500836103542373985855011118065`50.\
*^-66*CA*CF*L - 
  5.800986224121167831979892929864013931678823358225589749279708584220596`50.\
*^-66*CF^2*L + 
  3.49652752264794894786985409598850517519820889054801947213355610775676`50.*^\
-67*CF*nf + 
  2.14898654681905756015139261141737483652818333837007704361064547476011`50.*^\
-67*CF*L*nf + 
  1.0744932734095287800756963057086874182640916691850385218053227373800584`50.\
*^-65*CA*CF*irrational[Pi^2] - 
  2.1076598824571526070715581381208868589026413510937294081565946002454991`50.\
*^-65*CF^2*irrational[Pi^2], 
 (
    -2.048911032926799852407346957363366988513768821991457824756820815257496`50.\
*^-66*I)*CA*CF + 
  (
    4.500357936220102774739515958500816662689556307614106576347492066988685`50.\
*^-66*I)*CF^2 - 
  (
    2.272966539904772419390896031306838769404809300199119949972798098304`50.*^\
-68*I)*CA*CF*L - 
  (
    1.1204381043674333967816830052925893411510875104689835581110745614276`50.*^\
-67*I)*CF^2*L + 
  (
    6.727270363889279126909706682539162873660058788536679572214842582188`50.*^\
-69*I)*CF*nf + 
  (
    4.132666436190495307983447329648797762554198727634763545405087451462`50.*^\
-69*I)*CF*L*nf + 
  (
    2.10765988245715260707155813812088685890264135109372940815659460024551`50.\
*^-67*I)*CA*CF*irrational[Pi^2] - 
  (
    4.13578542972724285161211408235041949671461699082543129147709129104778`50.\
*^-67*I)*CF^2*irrational[Pi^2], 
 3.942413949919006211809053536041859751459118777430312665562189810891`50.*^-68\
*CA*CF - 
  8.6524028160997709791861537426257923631290632968500666577485166924598`50.*^\
-68*CF^2 + 
  4.28861611302787248941678496472988447057511188716815084900527943076`50.*^-70\
*CA*CF*L + 
  2.123034584484106978871692193142750708961083520635969132714802150223`50.*^-\
69*CF^2*L - 
  1.26987324541320981373965363834472213564440958703257138544786224074`50.*^-70\
*CF*nf - 
  7.797483841868859071666881754054335401045657976669365180009598965`50.*^-71*
   CF*L*nf - 
  4.054691597771806717266778512108254408543742147868069893604991461811`50.*^-\
69*CA*CF*irrational[Pi^2] + 
  7.959209432663176148708861523768054950104382734703989050409798054667`50.*^-\
69*CF^2*irrational[Pi^2], 
 (
    7.44252699792844842683625933746123253330475276696639253378651822522`50.*^-70\
*I)*CA*CF - 
  (
    1.632122313936012604206310341270123689106536922697183944196320678216`50.*^\
-69*I)*CF^2 + 
  (7.941881690792356461882935119870156426990947939200279350009776724`50.*^-72*
    I)*CA*CF*L + 
  (
    3.9478982746705941809905642359942075401881184171623469359604799531`50.*^-71\
*I)*CF^2*L - 
  (2.352645595843006046741638171904868777019172240676634432951882909`50.*^-72*
    I)*CF*nf - 
  (1.443978489234973902160533658158210259452899625309141700001777586`50.*^-72*
    I)*CF*L*nf - 
  (
    7.6530859929453616814508283882385143751003680141384510100094212064`50.*^-71\
*I)*CA*CF*irrational[Pi^2] + 
  (
    1.50278779497836193017579902896319918638334499186718674378366816416`50.*^\
-70*I)*CF^2*irrational[Pi^2], 
 -1.3789638777819948944558922451715554933296345120224586913178019786`50.*^-71*
   CA*CF + 
  3.021690229809538383480781072631178658268531847383202096671492344`50.*^-71*
   CF^2 - 
  1.44397848923497390216053365815821025945289962530914170000177758`50.*^-73*
   CA*CF*L - 
  7.20717815294931869141899020018552377486645197809964603736463849`50.*^-73*
   CF^2*L + 
  4.2793387611793747538164330818144449746014613321833822893839028`50.*^-74*CF*
   nf + 
  2.6254154349726798221100611966512913808234538641984394545486865`50.*^-74*CF*
   L*nf + 
  1.417724334885247103939433046191697345644665086667157305456290721`50.*^-72*
   CA*CF*irrational[Pi^2] - 
  2.784815657810306811309600626447976928944877848810487564289142487`50.*^-72*
   CF^2*irrational[Pi^2], 
 (-2.50846981693404546244182706274576343721580712583468016903140802`50.*^-73*
    I)*CA*CF + 
  (5.49259380596702064193804115379813569201274787752648474104270293`50.*^-73*
    I)*CF^2 - 
  (2.578533016491024825286667246711089749023035045194895892860317`50.*^-75*I)*
   CA*CF*L - 
  (1.2921122356784319584384837009194607727916740338773076175707892`50.*^-74*
    I)*CF^2*L + (7.6447770483019029993298338068075539646851769039652688740114\
97613679462974651527`50.*^-76*I)*CF*nf + 
  (4.688241848165499682339394994020163180041881900354356168836940214659808952\
170542`50.*^-76*I)*CF*L*nf + 
  (2.5785330164910248252866672467110897490230350451948958928603171`50.*^-74*
    I)*CA*CF*irrational[Pi^2] - 
  (5.0665911902981540426685391514323166998347355274004971929886933`50.*^-74*
    I)*CF^2*irrational[Pi^2], 
 4.481593590516943878467631926681870836509225223514016057235774`50.*^-75*CA*
   CF - 
  9.805713379549956629300316720563719956971151330474746167314977`50.*^-75*
   CF^2 + 4.52374213419478039523976709949313991056672814946472963659704757554\
89384626207`50.*^-77*CA*CF*L + 2.27567886704256989207157825879986416574993078\
6754274052330348589684406903523621`50.*^-76*CF^2*L - 
  1.3417136758232069673053923038881738160355977144146073831032596676853111514\
5056`50.*^-77*CF*nf - 8.22498569853596435498139472635116347375768754448132661\
19946319555435244774922`50.*^-78*CF*L*nf - 4.60599199118014003878958104675665\
154530430502490954290271699389510437370739562`50.*^-76*CA*CF*
   irrational[Pi^2] + 9.05315667231958559348296964362514269249466849723599811\
9133396365227918838128412`50.*^-76*CF^2*irrational[Pi^2], 
 (7.8661534996497805906156761136862845711810193416840851941957953027330677531\
3612`50.*^-77*I)*CA*CF - (1.7198621575596057038673132656340121185888536371623\
92044796733966651480581471282`50.*^-76*I)*CF^2 + 
  (7.799555403784104129723736378436448121666772671490913166546633750946445625\
208`50.*^-79*I)*CA*CF*L + (3.938516228152741213448340917777560615251840117409\
1261779036403625482591283536`50.*^-78*I)*CF^2*L - 
  (2.314172655965200559855885044363671430258606311537891246412533085099052639\
718`50.*^-79*I)*CF*nf - 
  (1.418100982506200750858861159715717840303049576634711484826660681990262840\
947`50.*^-79*I)*CF*L*nf - (8.083175600285344279895508610379591689727382586817\
8554635119658873444981933975`50.*^-78*I)*CA*CF*irrational[Pi^2] + 
  (1.589234524801864299098099997972936671200637932323510565707437360901630153\
27815`50.*^-77*I)*CF^2*irrational[Pi^2], 
 -1.3568531176322767803180372489923874859490157484139573190909883429390684292\
749`50.*^-78*CA*CF + 2.964522409827751306330834952296086413693495072881341004\
6140676611332019364776`50.*^-78*CF^2 - 
  1.3219585430142549372413112505824488341808089273713412146689209747366856991\
9`50.*^-80*CA*CF*L - 
  6.7003230516885571735066344490865416420641802063904702197704381837156375691\
2`50.*^-80*CF^2*L + 
  3.9237559503348916092356295713141809701992768386051586732260855100883969383`\
50.*^-81*CF*nf + 
  2.403560987298645340438747728331725153056016231584256753943492681339428544`\
50.*^-81*CF*L*nf + 
  1.3940653726332142974544736824324005887724894143188689172872257551768685555\
07`50.*^-79*CA*CF*irrational[Pi^2] - 
  2.7416618995119881183271315754503878245858958481604422039982106518478414924\
97`50.*^-79*CF^2*irrational[Pi^2], 
 (
    -2.3007692567546915259602546636375618430135304408107694589956251075850389\
8987`50.*^-80*I)*CA*CF + 
  (5.023329240635786222182892773635799664461999485266758801285032206794602218\
52`50.*^-80*I)*CF^2 - 
  (
    2.203264238357091562068852084304081390301348212285568691114868291227809499`\
50.*^-82*I)*CA*CF*L - 
  (1.120795511438053209236332354042342336436854889503683862734230101544532304\
2`50.*^-81*I)*CF^2*L + 
  (
    6.54189551204023950709811705154694120047873344387409995035185084313711695`\
50.*^-83*I)*CF*nf + 
  (
    4.00593497883107556739791288055287525509336038597376125657248780223238091`\
50.*^-83*I)*CF*L*nf + 
  (2.363501637510334584764768599526196400505082627724519141377767803317104734\
9`50.*^-81*I)*CA*CF*irrational[Pi^2] - 
  (
    4.649511418053117215930692326936779804272293693884299950251346498328730626`\
50.*^-81*I)*CF^2*irrational[Pi^2], 
 3.836261963394841107058134537280071572175815593253096640349932680795608027`5\
0.*^-82*CA*CF - 
  8.370074549992629991214664878279749183220505822696792562429570362826872787`\
50.*^-82*CF^2 + 
  3.6119085874706419050309050562361990004940134627632273624833906413570648`50.\
*^-84*CA*CF*L + 
  1.84393862210784661134659109705718820790591960640854871458107902994311185`5\
0.*^-83*CF^2*L - 
  1.0728068278433665151604461664796936822629759808177514356824735541318376`50.\
*^-84*CF*nf - 
  6.567106522673894372783463738611270909989115386842231568151619347921936`50.\
*^-85*CF*L*nf - 
  3.94026391360433662367007824316676254599346923210533894089097160875316155`5\
0.*^-83*CA*CF*irrational[Pi^2] + 
  7.7534225396730494852862829946184682356645684889814733998177183269013824`50.\
*^-83*CF^2*irrational[Pi^2], 
 (
    6.2915731620748746171051565956249144122234406966303513063008992055190252`50.\
*^-84*I)*CA*CF - 
  (
    1.37179262558023581907247812615893391084167909028557842605888027139703718`\
50.*^-83*I)*CF^2 + 
  (
    5.82565901204942242746920170360677258144195719800520542336030748605978`50.\
*^-86*I)*CA*CF*L + 
  (
    2.984515818641248633200531719708661717369311957230161197442355583680962`50.\
*^-85*I)*CF^2*L - 
  (
    1.73090306142987262195257389527063074583778549762374427118124867552897`50.\
*^-86*I)*CF*nf - 
  (
    1.05921072946353135044894576429214046935308312691003734970187408837451`50.\
*^-86*I)*CF*L*nf - 
  (
    6.461185449727541237738569162182056863053807074151227833181431939084485`50.\
*^-85*I)*CA*CF*irrational[Pi^2] + 
  (
    1.2717253901051033547294961525564683349502731384043686528801548578515495`\
50.*^-84*I)*CF^2*irrational[Pi^2], 
 -1.015180132801648536284740231349467077568734619920605293248555284300244`50.\
*^-85*CA*CF + 
  2.212004181692117358237223944150947030908246267497525595026486319424182`50.\
*^-85*CF^2 - 
  9.24707779690384512296698683112186124038405904445270702120683727946`50.*^-88\
*CA*CF*L - 
  4.7536014481801014681925678852384895255071891354540983074482494348304`50.*^\
-87*CF^2*L + 
  2.748340163535402462884336960234282177528846855598870471089031142268`50.*^-\
88*CF*nf + 
  1.681286872164335476903088514749429316433465280809583094764879505356`50.*^-\
88*CF*L*nf + 
  1.04239786074188799567991487914464617618874847410194151875422529332094`50.*^\
-86*CA*CF*irrational[Pi^2] - 
  2.0522207883355919914948324183160221593715985583881973650473810462256`50.*^\
-86*CF^2*irrational[Pi^2], 
 (
    -1.6120295339590783140834567513075526019421001240306035344032074261204`50.*^\
-87*I)*CA*CF + 
  (
    3.5102235403454599089537636134704538147676492771423452631152239156595`50.*^\
-87*I)*CF^2 - 
  (
    1.44485590576622580046359169236279081881000922569573547206356832492`50.*^\
-89*I)*CA*CF*L - 
  (
    7.45252771789411168520627760934501593426069157836774836383913739711`50.*^\
-89*I)*CF^2*L + 
  (4.295605603678177625566585510348069926233040595694437214698370295`50.*^-90*
    I)*CF*nf + 
  (
    2.6270107377567741826610758042959833069272895012649735855701242271`50.*^-90\
*I)*CF*L*nf + 
  (
    1.655016764786767735076477756706469483364192385796933358909178263085`50.*^\
-88*I)*CA*CF*irrational[Pi^2] - 
  (
    3.259109936810865693689063890129662982624871159723191845236535656537`50.*^\
-88*I)*CF^2*irrational[Pi^2], 
 2.51975681736578255606891638722461036743742701759989101699061667753`50.*^-89*
   CA*CF - 
  5.48333175289588323656469117894547267653522751907047075975445009877`50.*^-89\
*CF^2 + 
  2.2228552396403473853286026036350627981692449626088238031747205`50.*^-91*CA*
   CF*L + 
  1.1503326088891236021239369633193502774409144333714475264621831657`50.*^-90*
   CF^2*L - 
  6.61059790308543286374020468356680316128041920479806531092738484`50.*^-92*
   CF*nf - 
  4.04155498116426797332473200660920508758044538656149782395403727`50.*^-92*
   CF*L*nf - 
  2.5865951879451315029278284842298912560514850473993586073305838544`50.*^-90*
   CA*CF*irrational[Pi^2] + 
  5.0948087035282893239487530749982706558589856994229790750450894101`50.*^-90*
   CF^2*irrational[Pi^2], 
 (3.877985709907594849502439726748200492844850021899763401037280712`50.*^-91*
    I)*CA*CF - 
  (8.433759953773053595539293234548409245102239979528976225652482288`50.*^-91*
    I)*CF^2 + 
  (3.3679624843035566444372766721743375729837044888012481866283644`50.*^-93*
    I)*CA*CF*L + 
  (1.74858205792807289531231210825826140372187295668638953214305069`50.*^-92*
    I)*CF^2*L - 
  (1.001895684565656456338429538545949371679280432587241408007819`50.*^-93*I)*
   CF*nf - 
  (6.123568153279193898976866676680613769061280888729542157506117`50.*^-94*I)*
   CF*L*nf - 
  (3.9803192996314760343349633398423989498898325776742024023789761`50.*^-92*
    I)*CA*CF*irrational[Pi^2] + 
  (7.84182309778141547063007702774920390127549104855215995692574396`50.*^-92*
    I)*CF^2*irrational[Pi^2], 
 -5.8778538184246813024086314987843140530460811282752945728749539`50.*^-93*CA*
   CF + 
  1.27752035288979622252518011019304012623919685839550385434336664`50.*^-92*
   CF^2 - 5.02680967806500991707056219727513070594582759522574356213188547546\
6230646693808`50.*^-95*CA*CF*L - 
  2.618134651254774257389882147301740543117103140561919015517148`50.*^-94*
   CF^2*L + 1.495786424906725741944807311446080379874592093526117600392601757\
311625971575669`50.*^-95*CF*nf + 9.139653960118199849219203995045692192628777\
44586498829478524937243610618530829`50.*^-96*CF*L*nf + 
  6.032171613678011900484674636730156847134993114270892274558265`50.*^-94*CA*
   CF*irrational[Pi^2] - 
  1.1886926415189023450955094137085897316413074666357346541041286`50.*^-93*
   CF^2*irrational[Pi^2], 
 (-8.77599167834441422190971863840415093685424652407764386030797`50.*^-95*I)*
   CA*CF + 
  (1.906268231461268702104384061118732463347104199391941611540453`50.*^-94*I)*
   CF^2 - (7.3923671736250145839272973489340157440379817576849170031351281688\
821447087052`50.*^-97*I)*CA*CF*L - (3.862237117198510416850048586148125471887\
09977593001919975686682399585184324806`50.*^-96*I)*CF^2*L + 
  (2.200284879211691559786272889328738689877482132495277861297103955872216296\
2897`50.*^-97*I)*CF*nf + (1.3440667588409117425322358816243664989159966832154\
394551154778488876626743101`50.*^-97*I)*CF*L*nf + 
  (9.005247284234108674965980406883255542737177777543444349273701587547339917\
87729`50.*^-96*I)*CA*CF*irrational[Pi^2] - 
  (1.774947290805563448978801935269743121467037938762186132610468718704982940\
335233`50.*^-95*I)*CF^2*irrational[Pi^2], 
 1.29102738597827709158129332954663207248755541411190764996427109861027990196\
747`50.*^-96*CA*CF - 2.802635587136421071863540694306733688091508555316258072\
58332002047167190480653`50.*^-96*CF^2 + 
  1.0713575613949296498445358476715964846431857619833213048021924882437890882\
18`50.*^-98*CA*CF*L + 
  5.6146363696857310348675932993297714984277838685588029262147695121015714459\
99`50.*^-98*CF^2*L - 
  3.1896613749504938772981356729678663068718887891644801925115263454921458439\
1`50.*^-99*CF*nf - 
  1.9479228388998720906264288139483572448057922945151296450948954331705256149\
4`50.*^-99*CF*L*nf - 1.324587530451913021625971593484882926467938760270288158\
6645288945559574181606`50.*^-97*CA*CF*irrational[Pi^2] + 
  2.6113297028909142426340582842987691978939364131042823699386426778388874815\
166`50.*^-97*CF^2*irrational[Pi^2], 
 (1.8716756376173203920506232780760168481332615143433125310299343320736338058\
67`50.*^-98*I)*CA*CF - 
  (4.060781488639039149059097496569983255463727515472420451706052038123013112\
688`50.*^-98*I)*CF^2 + 
  (1.530510801992756642635051210959423549490265374261887578288846411776841554\
6`50.*^-100*I)*CA*CF*L + 
  (8.045111982363305651417070305434326027146221793317175358970357607604063578\
4`50.*^-100*I)*CF^2*L - 
  (
    4.557828328464030792353054820214567927731033079535400953074746457205568808`\
50.*^-101*I)*CF*nf - 
  (
    2.782746912714102986609184019926224635436846135021613778706993475957893736`\
50.*^-101*I)*CF*L*nf - 
  (1.920095369772731060760336973749094998451423833164913507307825498410946677\
59`50.*^-99*I)*CA*CF*irrational[Pi^2] + 
  (3.786103546030737302907706708801032391312666713282928042578810841937077955\
8`50.*^-99*I)*CF^2*irrational[Pi^2], 
 -2.6746874063523349053822411394769111731924144560314157249904776792755288853`\
50.*^-100*CA*CF + 
  5.7996833356370049716993637468733183496565012428383586364192760257758667846`\
50.*^-100*CF^2 - 
  2.1556490168912065389226073393794697880144582736082923637871076222209036`50.\
*^-102*CA*CF*L - 
  1.136474502469081839401827137908560374255099146509685789922676822393835448`\
50.*^-101*CF^2*L + 
  6.4210765850376808885144234472315478948636268824376266776693711222474254`50.\
*^-103*CF*nf + 
  3.9193618488931027980411042534172177963899241338332588432492865858561884`50.\
*^-103*CF*L*nf + 
  2.743553294225171958628772977392052457472946893683281190274500610099331852`\
50.*^-101*CA*CF*irrational[Pi^2] - 
  5.410896774721866918406746705412103457793867484764249014152487314362571152`\
50.*^-101*CF^2*irrational[Pi^2], 
 (
    -3.76835264426602501718694624718747556578097245481011660616312270740438249`\
50.*^-102*I)*CA*CF + 
  (
    8.16656168531264143905946604611843490868512269842634447521379922027773497`\
50.*^-102*I)*CF^2 - 
  (
    2.993956967904453526281399082471485816686747602233739394148760586417922`50.\
*^-104*I)*CA*CF*L - 
  (
    1.583037911684429312308439120144042557886442012571358593442056091744014`50.\
*^-103*I)*CF^2*L + 
  (
    8.92032206577593085419664252164733130117544624552284638810078511609864`50.\
*^-105*I)*CF*nf + 
  (
    5.44355812346264277505708924085724693943045018587952617117956470257804`50.\
*^-105*I)*CF*L*nf + 
  (
    3.864926267658476370290533361008645326995619631974463581537490938830408`50.\
*^-103*I)*CA*CF*irrational[Pi^2] - 
  (
    7.6239641444221999633128329313047250285940990000592158320739547286517636`\
50.*^-103*I)*CF^2*irrational[Pi^2], 
 5.235431053580486044158097032289354278431932295893202240771544260356595`50.*^\
-104*CA*CF - 
  1.1339678517376004633225660273902799130151497192782412481451034473233091`50.\
*^-103*CF^2 + 
  4.1013109149376075702484918937965559132695172633338895810256994334492`50.*^\
-106*CA*CF*L + 
  2.17476039088636869811023038575191177804777169195403073347526355736863`50.*^\
-105*CF^2*L - 
  1.222249672484692445609891990627415566376673973419865045680655895225`50.*^-\
106*CF*nf - 
  7.456928936250195582269985261448283478671849569697981056410362606271`50.*^-\
107*CF*L*nf - 
  5.36898883410014081923438938824276410464373169018254636061546107651532`50.*^\
-105*CA*CF*irrational[Pi^2] + 
  1.059286986187325080551649798220869674699979495630610498175482861042213`50.\
*^-104*CF^2*irrational[Pi^2], 
 (
    7.1739712769062734780044041979721418892104709799444540079294133696235`50.*^\
-106*I)*CA*CF - 
  (
    1.55300387936876971410226752905266733311338957814659564613741970969207`50.\
*^-105*I)*CF^2 + 
  (
    5.54231204721298320303850255918453501793178008558633727165635058574`50.*^\
-108*I)*CA*CF*L + 
  (
    2.947149356632819038679300084898580024722808182129685320028630392692`50.*^\
-107*I)*CF^2*L - 
  (
    1.65206700977642119889973381906784143797953019750197339897274386268`50.*^\
-108*I)*CF*nf - 
  (
    1.00769309949326967327972773803355182144214183374297041302842737923`50.*^\
-108*I)*CF*L*nf - 
  (
    7.356159626300868614942012487644928296527635386323684015107519868349`50.*^\
-107*I)*CA*CF*irrational[Pi^2] + 
  (
    1.4516154995900380733485571308952658505147867162345403123145505873542`50.*^\
-106*I)*CF^2*irrational[Pi^2], 
 -9.69738798692798290623662788569786969373715582175283835207288964326`50.*^-1\
08*CA*CF + 
  2.09814839105519073249906145878944555194123306551857879365995144439`50.*^-1\
07*CF^2 - 
  7.389749396283977604051336745579380023909040114115116362208467448`50.*^-110*
   CA*CF*L - 
  3.9404284447323434789072238359545608124759588175532943716274492726`50.*^-109\
*CF^2*L + 
  2.203246822459638990154667181704109339806590469404149844798010229`50.*^-110*
   CF*nf + 
  1.343590799324359564372970317378069095256189111657293884037903172`50.*^-110*
   CF*L*nf + 
  9.942571915000260776359980348597711304895799426263974741880483475`50.*^-109*
   CA*CF*irrational[Pi^2] - 
  1.96234972006584094270262770038112723122943409728894238326588489639`50.*^-1\
08*CF^2*irrational[Pi^2], 
 (
    -1.2933535557103178173112013324965773633425231174084793259811105716`50.*^\
-109*I)*CA*CF + 
  (
    2.7968619051819948233028911469235461614109778075155488099633296054`50.*^-\
109*I)*CF^2 - 
  (9.7233544687947073737517588757623421367224212027830478450111414`50.*^-112*
    I)*CA*CF*L - 
  (5.1989198451992157449677628110940104249296532014917987223025568`50.*^-111*
    I)*CF^2*L + 
  (2.8996376691790022085232916660128273249192317647470084307179955`50.*^-112*
    I)*CF*nf + 
  (1.7678826306899467952275925228658803884949856732332814263656621`50.*^-112*
    I)*CF*L*nf + 
  (
    1.325911973017460096420694392149410291371239254924961069774246552`50.*^-110\
*I)*CA*CF*irrational[Pi^2] - 
  (
    2.617384674008492657869422696191043692057511256475247826047863323`50.*^-110\
*I)*CF^2*irrational[Pi^2], 
 1.70225439587297540595889841785955290755654159973109033007192097`50.*^-111*
   CA*CF - 
  3.67920741181863646045881299686026243471638932263018095105473197`50.*^-111*
   CF^2 + 
  1.262773307635676282305423230618485991782132623738058161689759`50.*^-113*CA*
   CF*L + 
  6.769973026139300050835151167281856265741073499817748974945643`50.*^-113*
   CF^2*L - 
  3.76655834143365776079439243408552528525002606684892117844474`50.*^-114*CF*
   nf - 2.2959514684285023314644058738517927123311502249782875667086522907697\
49975800855`50.*^-114*CF*L*nf - 
  1.7449231160056617719129484641273624613716741709834985506985755`50.*^-112*
   CA*CF*irrational[Pi^2] + 
  3.4451046136522040112127444035335105006568951580956253436869312`50.*^-112*
   CF^2*irrational[Pi^2], 
 (2.211320308170722128632455557606227019145354705874840418370997`50.*^-113*I)*
   CA*CF - 
  (4.77706471042905015052431984786095475958090311531839683746576`50.*^-113*I)*
   CF^2 + (1.6189401379944567721864400392544692202335033637667412329355879751\
0739922271439`50.*^-115*I)*CA*CF*L + 
  (8.702393044914003838598314749433111173099151970507978824755984992901665198\
57856`50.*^-115*I)*CF^2*L - (4.8299140435126605182385392143773784292680578966\
249613570006416294867009777648`50.*^-116*I)*CF*nf - 
  (2.943527523626285040338981889553580400424551570484984059882887227467998586\
7534`50.*^-116*I)*CF*L*nf - (2.2665161931922394810610160549562569083269047092\
7343772610982471113635957617357`50.*^-114*I)*CA*CF*irrational[Pi^2] + 
  (4.47565222959480201323441145029336807213920423603362386421687`50.*^-114*I)*
   CF^2*irrational[Pi^2], 
 -2.8357779413245652902154945853522167903173233341547980291906750387620361271\
6957`50.*^-115*CA*CF + 
  6.1230086975856690943992787371644242121615141130975449787289729340476555338\
11`50.*^-115*CF^2 - 
  2.0492913139170338888435949863980623040930422326161281429564404748194926869\
8`50.*^-117*CA*CF*L - 1.10443535273271631648444228204422623806753434972539641\
38487874660876094144256`50.*^-116*CF^2*L + 
  6.1150402931878562798015036727873488776645528601832061342888916000854296254`\
50.*^-118*CF*nf + 
  3.7259842071218797978974454298146587347146222411202329871935281360354412490\
5`50.*^-118*CF*L*nf + 2.90626768155506624236000743525543381307740534807378173\
00109519461076441742629`50.*^-116*CA*CF*irrational[Pi^2] - 
  5.7398786710712558286610146846294817808278755624457189167716300935625972441\
692`50.*^-116*CF^2*irrational[Pi^2], 
 (-3.590522233387895853335945615463013953380334907884124998813607906829558559\
285`50.*^-117*I)*CA*CF + 
  (7.748843681870718075852431853280727421957089086301236347121936093308278421\
571`50.*^-117*I)*CF^2 - 
  (2.561614142396292361054493732997577880116302790770160178695550593524365858\
7`50.*^-119*I)*CA*CF*L - 
  (1.384082084574100065125191051941765466334928215486655353921420495142526189\
41`50.*^-118*I)*CF^2*L + 
  (
    7.645293148619083923388857734185233636637868407857661607359188830289493539`\
50.*^-120*I)*CF*nf + 
  (
    4.657480258902349747371806787268323418393277801400291233991910170044301561`\
50.*^-120*I)*CF*L*nf + 
  (3.679409404532856300423727361941975500530689463106230074853609034334998233\
44`50.*^-118*I)*CA*CF*irrational[Pi^2] - 
  (7.267969194138975408244399727292791112159386593790084098476264759180243424\
08`50.*^-118*I)*CF^2*irrational[Pi^2], 
 4.4892890496279916154243289409082587070132805995145125371801384342213489793`\
50.*^-119*CA*CF - 
  9.6838225020439713361017325492018756434690795505147684664288215647422013794`\
50.*^-119*CF^2 + 
  3.16248659555097822352406633703404676557568245774093849221672912780785908`5\
0.*^-121*CA*CF*L + 
  1.713056469940788895549551958148214742559214187468688010215008694883505666`\
50.*^-120*CF^2*L - 
  9.4404306650019240516477389898162804542535593905459721152339453397159969`50.\
*^-122*CF*nf - 
  5.7499756282745058609528478855164486646830590140744336222122347778324711`50.\
*^-122*CF*L*nf - 
  4.599980502619604688762278308413158931746447211259546897769787822265976851`\
50.*^-120*CA*CF*irrational[Pi^2] + 
  9.087766358833853165603525438572338377352737173463982895593971063501076217`\
50.*^-120*CF^2*irrational[Pi^2], 
 (
    5.54370349184084390714067022574049080260676649559808767544169717652733929`\
50.*^-121*I)*CA*CF - 
  (
    1.195260271815468284747753227406017079869124373309456347608609572874456978`\
50.*^-120*I)*CF^2 + 
  (
    3.856690970184119784785446752480544836067905436269437185630157472936413`50.\
*^-123*I)*CA*CF*L + 
  (
    2.0942882444164539807572300130457872270409735158765234782894126449018558`\
50.*^-122*I)*CF^2*L - 
  (
    1.151485817847805822251098183167865717527377969214933929639706757474952`50.\
*^-123*I)*CF*nf - 
  (
    7.01216540033476324506444864087371788375982806594443124660028631442984`50.\
*^-124*I)*CF*L*nf - 
  (
    5.6798539742711582285022033991077114858454607334149893097462319146881726`\
50.*^-122*I)*CA*CF*irrational[Pi^2] + 
  (
    1.12228439973550596322212211741405383575741633768681716481732775181790399`\
50.*^-121*I)*CF^2*irrational[Pi^2], 
 -6.762249685176564310986167364819388342300464967050459186957052895808478`50.\
*^-123*CA*CF + 
  1.4573038690296186728587722287628581439205256780131823676663987513820106`50.\
*^-122*CF^2 - 
  4.6466156267278551623921045210608973928528981159872737176266957505258`50.*^\
-125*CA*CF*L - 
  2.52942151846681095605923461181090739027230085918368950075590082244949`50.*^\
-124*CF^2*L + 
  1.3875836386995309207634905485692409911871159878505883767496704511517`50.*^\
-125*CF*nf + 
  8.448392048596100295258371856474358896096178392704134032048537728229`50.*^-\
126*CF*L*nf + 
  6.92768147984880224211186492230897429479886628201738990627980093714756`50.*^\
-124*CA*CF*irrational[Pi^2] - 
  1.369041816255834728798297115599154443972156908112960386241008280436303`50.\
*^-123*CF^2*irrational[Pi^2], 
 (
    -8.1492163268447795326997460306373016100054833440306372751300311679042`50.*^\
-125*I)*CA*CF + 
  (
    1.75539273302222668185976086873564166610453029698657980242699566053151`50.\
*^-124*I)*CF^2 - 
  (
    5.53168526991411328856202919173916356292011680474675442574606636967`50.*^\
-127*I)*CA*CF*L - 
  (
    3.018487710096476004646865960469341506881907680447175188852636500836`50.*^\
-126*I)*CF^2*L + 
  (
    1.65217731696464662530383665396621916982538198937997648876205335972`50.*^\
-127*I)*CF*nf + 
  (
    1.00576095816620241610218712577075701144002123722668262286292115812`50.*^\
-127*I)*CF*L*nf + 
  (
    8.347815952779480053648153143897283194952176268981465769762245612417`50.*^\
-126*I)*CA*CF*irrational[Pi^2] - 
  (
    1.64992127066700311648575262138205126676701836845751323449418501516`50.*^\
-125*I)*CF^2*irrational[Pi^2], 
 9.70369354367909868866581075696133423414488500988590793078913725052`50.*^-127\
*CA*CF - 
  2.089286934533822531437116597808971210517270528491949699956186213156`50.*^-\
126*CF^2 + 
  6.507865023428368574778857872634310074023666829113828736171842788`50.*^-129*
   CA*CF*L + 
  3.5596149826192879167140850597823905422818086056465661836073942952`50.*^-128\
*CF^2*L - 
  1.944073455305276082269691410844743862448984863059188309244509492`50.*^-129*
   CF*nf - 
  1.183248186077885195414337795024420013458848514384332497485789598`50.*^-129*
   CF*L*nf - 
  9.9392847630542356414804374782051281130543275208283929788806326215`50.*^-128\
*CA*CF*irrational[Pi^2] + 
  1.96474233688281402215310973406380439444097171923351954233686923912`50.*^-1\
27*CF^2*irrational[Pi^2], 
 (
    1.1418695373279352143492401929900098296787788747816715583518311053`50.*^-128\
*I)*CA*CF - 
  (
    2.4574406089834166882532269324018170451994848895106349959950904234`50.*^-\
128*I)*CF^2 + 
  (7.5672849109632192729986719449236163651437986385044520188044684`50.*^-131*
    I)*CA*CF*L + 
  (4.14880055691810696504363389789433070291054795407820106552956419`50.*^-130*
    I)*CF^2*L - 
  (2.2609314458100695016461728713610443390182570288586406118779308`50.*^-131*
    I)*CF*nf - 
  (1.375869983811494413272485808167930248207963388818991276146267`50.*^-131*
    I)*CF*L*nf - 
  (
    1.169489486239770251281612936942740710976768880496142584724326928`50.*^-129\
*I)*CA*CF*irrational[Pi^2] + 
  (
    2.312094156703913600234912932806337957333382154544097983592922203`50.*^-129\
*I)*CF^2*irrational[Pi^2], 
 -1.32804960008084557996137385409498848227281329682479541134604761`50.*^-130*
   CA*CF + 
  2.85686195871513882626541819037533357159166652244573645818622077`50.*^-130*
   CF^2 - 
  8.69802863329105663563065740795817973005034326264879542391318`50.*^-133*CA*
   CF*L - 
  4.779771204459999241211836662334761876824358339553963431246691`50.*^-132*
   CF^2*L + 
  2.59919948734125837642706602866666025468224517267605252187943`50.*^-133*CF*
   nf + 1.5814597515074648428419377105378508600091533204815991679842157365258\
00135948498`50.*^-133*CF*L*nf + 
  1.3600553862964197648440664310625517396078718556141752844664248`50.*^-131*
   CA*CF*irrational[Pi^2] - 
  2.68920042290428453503258589778277275786101935087348294883134`50.*^-131*
   CF^2*irrational[Pi^2], 
 (-1.52682502774673193155899890800644982340981069323304501426242`50.*^-132*I)*
   CA*CF + 
  (3.283034682996981428803527550875406675339357311141462252233849`50.*^-132*
    I)*CF^2 - (9.884123446921655267762110690861567875057208253009994799901343\
20528550292070872`50.*^-135*I)*CA*CF*L - 
  (5.443953709756084819197988091161282207785655769068556410400810631672254512\
415782`50.*^-134*I)*CF^2*L + (2.954110705317493862087635675987765548294741281\
08983529392890672172789147566066`50.*^-135*I)*CF*nf + 
  (1.797113353985755503229474671065739613646765136910908145436607855506455076\
4925`50.*^-135*I)*CF*L*nf + (1.5634886179676072878096429638271934638726856691\
124900865298488017753039266115451`50.*^-133*I)*CA*CF*irrational[Pi^2] - 
  (3.09184266025054924330895687228748370383811997487413769920509`50.*^-133*I)*
   CF^2*irrational[Pi^2], 1.7353971370058699774438348712274385205471599603921\
04846186945457135308130326692`50.*^-134*CA*CF - 
  3.7299161793643146723200958625637718435362236730305563116024503770680523445\
56828`50.*^-134*CF^2 + 1.1105756681934444121081023248159065028154166576415724\
494271172140770228000796`50.*^-136*CA*CF*L + 6.130571166088661835281528376118\
4918290075532984670065511600226976753207344472`50.*^-136*CF^2*L - 
  3.3197470739038415974342932418139762510645316857055980243383872583790907345\
37`50.*^-137*CF*nf - 
  2.0192284876244443856510951360289209142098484684392226353220312983218596365\
09`50.*^-137*CF*L*nf - 1.7769210691095110593729637197054504045046666522265159\
1908338754252323648012742`50.*^-135*CA*CF*irrational[Pi^2] + 
  3.5143550033499218729820838011952241333536740455146648177426998063237343718\
0755`50.*^-135*CF^2*irrational[Pi^2], 
 (1.9502902250371258676925358283834781960052428847831780444674304141657880818\
988`50.*^-136*I)*CA*CF - (4.1900203037499331817972460192467683877466369581200\
293291159143976062201291224`50.*^-136*I)*CF^2 + 
  (1.233972964659382680120113694239896114239351841823969388252352460085580888\
98`50.*^-138*I)*CA*CF*L + 
  (6.826872956882905031653124750157463476789930980930604148977774444012195219\
06`50.*^-138*I)*CF^2*L - 
  (3.689174422319539048884807051829229762943253457873907799948186188125567106\
7`50.*^-139*I)*CF*nf - 
  (2.243587208471604872945661262254356571344276076043580705913368109246510707\
3`50.*^-139*I)*CF*L*nf - 
  (1.996792615539728336921638523406377348496405707678786828262897617229394529\
436`50.*^-137*I)*CA*CF*irrational[Pi^2] + 
  (3.949699679089572534570274002342284865157725575628369550410127154959241926\
357`50.*^-137*I)*CF^2*irrational[Pi^2], 
 -2.1674309983471079095023870412436924112109143570144298823815106627644716740\
9`50.*^-138*CA*CF + 
  4.6545905251710716965890568060111019614384363265365107763803047660990094252\
6`50.*^-138*CF^2 - 
  1.356014246878442505626498565098786938724562463542823503574013692401737241`\
50.*^-140*CA*CF*L - 
  7.51849676015518324939013269304540812301806923967866286038438025857948555`5\
0.*^-140*CF^2*L + 
  4.05464666249433724237613701261306721671242797679171712057684325074014849`5\
0.*^-141*CF*nf + 
  2.46548044886989546477545193654324897949920447916877000649820671345770408`5\
0.*^-141*CF*L*nf + 
  2.2189324039829059182979067428889240815492840312518930058483860421119336665`\
50.*^-139*CA*CF*irrational[Pi^2] - 
  4.3896271470096617079371633391933063352388010183461361637435463006996948619`\
50.*^-139*CF^2*irrational[Pi^2], 
 (
    -2.382268160191152287920406608238634372886950957532216595792086147496702481`\
50.*^-140*I)*CA*CF + 
  (
    5.113858833594814003466405879942513674471869952968502044637418529949258324`\
50.*^-140*I)*CF^2 - 
  (
    1.4739285292156983756809767011943336290484374603726342430152322743497144`\
50.*^-142*I)*CA*CF*L - 
  (
    8.189950693997218756212854228910843395934450465908152610577802802404029`50.\
*^-142*I)*CF^2*L + 
  (
    4.407871944753052425672648257759567718485861958726338387207159542317179`50.\
*^-143*I)*CF*nf + 
  (
    2.679870053119451592147230365807879325542613564313880441845876862454026`50.\
*^-143*I)*CF*L*nf + 
  (
    2.43868174833870094885397963288517018624377834352563120207974794483316381`\
50.*^-141*I)*CA*CF*irrational[Pi^2] - 
  (
    4.82491872789592445794765862850399262654683027106146388368466260053013056`\
50.*^-141*I)*CF^2*irrational[Pi^2], 
 2.5899290065065938135744923744426010349524906728086234485925597089889289`50.\
*^-142*CA*CF - 
  5.5573832581278501684694214307457476220672129647382661208289566568645777`50.\
*^-142*CF^2 + 
  1.58486938625343911363545881848853078392305103265874649786584115521474`50.*^\
-144*CA*CF*L + 
  8.82519373391710863629231257827749413939275283831718101739638801151537`50.*^\
-144*CF^2*L - 
  4.7403282356915201505416895894908561315221520856542685531602945853304`50.*^\
-145*CF*nf - 
  2.8815807022789802066099251245246014253146382411977209052106202822086`50.*^\
-145*CF*L*nf - 
  2.65105424609666179008113111456263331128946718190190323279377065963194`50.*^\
-143*CA*CF*irrational[Pi^2] + 
  5.245703082701905244203089226687763786168520168444191503187673858420646`50.\
*^-143*CF^2*irrational[Pi^2], 
 (
    2.78540449368888295641667586686777920667986372537326300323189372911732`50.*^\
-144*I)*CA*CF - 
  (
    5.97444567708800354407545822979685878614025381113334837492183705842159`50.\
*^-144*I)*CF^2 + 
  (
    1.686031261971743737910062572860139131833033013466751593474299101292`50.*^\
-146*I)*CA*CF*L + 
  (
    9.408283752005422798800454784637481311261376798426621118270454383172`50.*^\
-146*I)*CF^2*L - 
  (
    5.04361133107455963527389821040481294755818594303202682326508266756`50.*^\
-147*I)*CF*nf - 
  (
    3.06551138540317043256375013247298023969642366084863926086236200235`50.*^\
-147*I)*CF*L*nf - 
  (
    2.8509255884249485022842876231998716229176740045892345126019966621851`50.*^\
-145*I)*CA*CF*irrational[Pi^2] + 
  (
    5.6418316907777928255731165595955354221949759248713272459913197104295`50.*^\
-145*I)*CF^2*irrational[Pi^2], 
 -2.963754070097795493299598681863595188040389344009293124059549875421`50.*^-\
146*CA*CF + 
  6.354490938479064286170122619352273934675123660356765375345946438692`50.*^-\
146*CF^2 - 
  1.7747697494439407767474342872211990861400347510176332562887358961`50.*^-148\
*CA*CF*L - 
  9.9240558533469930288980565966393975480908041948674304749926550135`50.*^-148\
*CF^2*L + 
  5.30979502967438605051797792144776675925963907354238873643329224`50.*^-149*
   CF*nf + 
  3.226854089898074139540789613129452883890972274577515011434065266`50.*^-149*
   CF*L*nf + 
  3.03324284450418969116834223634168571085751393810286411074802134969`50.*^-1\
47*CA*CF*irrational[Pi^2] - 
  6.0032931297478754304373440094262529694054963358285852191887922546`50.*^-147\
*CF^2*irrational[Pi^2], 
 (
    -3.1203170363547248077628247917720714789261067332274879243773162099`50.*^\
-148*I)*CA*CF + 
  (
    6.6875790518822814014212768743943681592950651640387537058426331081`50.*^-\
148*I)*CF^2 - 
  (1.84871848900410497577857738252208238139586953231003464196743323`50.*^-150*
    I)*CA*CF*L - 
  (
    1.035878983633083251592164964446918198327067663015922943470022769`50.*^-149\
*I)*CF^2*L + 
  (5.5317814596217327714235781368169725802174254008056838000975289`50.*^-151*
    I)*CF*nf + 
  (3.3613063436438272286883225136765134207197627860182448035771513`50.*^-151*
    I)*CF*L*nf + 
  (
    3.193241026461635867253906387992687749683774646717332563398293753`50.*^-149\
*I)*CA*CF*irrational[Pi^2] - 
  (
    6.320642031759114293945876561799959257106028166698225280128581449`50.*^-149\
*I)*CF^2*irrational[Pi^2], 
 3.25091887127022151058144814182716581678956451322494124021338659`50.*^-150*
   CA*CF - 
  6.96482549196316982062348700735136965642235349573015806780579169`50.*^-150*
   CF^2 + 
  1.905895349488768016266574621156785960201927352896942929863333`50.*^-152*CA*
   CF*L + 
  1.0700825031709002699832797137183467021930038259381213971108137`50.*^-151*
   CF^2*L - 5.703619576228980667236369341313272885819849370870713114264153673\
209895943273948`50.*^-153*CF*nf - 3.46526427179776002957559022028506538218532\
2459812623508842424039552367843077749`50.*^-153*CF*L*nf - 
  3.3266537009258496283925666114736627668979095614201185684887271`50.*^-151*
   CA*CF*irrational[Pi^2] + 
  6.5854165099960696725322237002641895589611679073010510437429903`50.*^-151*
   CF^2*irrational[Pi^2], 
 (3.352058195498699088749687279606200539103457192776351400019955`50.*^-152*I)*
   CA*CF - 
  (7.178799208878261454585489943295557703808776667872217329163586`50.*^-152*
    I)*CF^2 + (1.944791172947722465578137368527332612450946278466268295778911\
45076918603438037`50.*^-154*I)*CA*CF*L + 
  (1.094108360654164573720891629545009984420130780050625127208281123878341703\
722673`50.*^-153*I)*CF^2*L - (5.820771673012313189536793907867798295909420719\
4562263798520231596222760989223`50.*^-155*I)*CF*nf - 
  (3.535983950814040846505704306413332022638084142665942355961657183216701880\
6916`50.*^-155*I)*CF*L*nf - (3.4299044322896196211105331772209320619589416183\
85964085282807467720200824270833`50.*^-153*I)*CA*CF*irrational[Pi^2] + 
  (6.790517865947125714521863663992956405494470274784332936519495892917786084\
196203`50.*^-153*I)*CF^2*irrational[Pi^2], 
 -3.4210639423106702637762190774411792239887683286479378716321408439532606308\
3389`50.*^-154*CA*CF + 7.3238559634288078019508536422874280441766516710672180\
6423931417089479910136092`50.*^-154*CF^2 - 
  1.9644355282300226925031690591185177903544911903699679755342539906759454892\
73`50.*^-156*CA*CF*L - 1.1073469436626736974681918487007365409462350060623972\
556591824920917000461669`50.*^-155*CF^2*L + 
  5.8803112183838669566449503160173318838350645197390413360335524058894843237\
9`50.*^-157*CF*nf + 
  3.5717009604182230772784891983973050733718021643090326827895527103199008895\
9`50.*^-157*CF*L*nf + 3.50026694120985861573291941442935897190436612102285202\
91337616561135028717957`50.*^-155*CA*CF*irrational[Pi^2] - 
  6.9305285435955200591511804405701307643706449196252470176848480791047356861\
555`50.*^-155*CF^2*irrational[Pi^2], 
 (-3.456211483757350444682290576452595914685024735565936740769518185784875294\
343`50.*^-156*I)*CA*CF + 
  (7.396383313972741226226202153822947273364777644319121309950459165917883294\
91`50.*^-156*I)*CF^2 - 
  (1.964435528230022692503169059118517790354491190369967975534253990675945489\
2`50.*^-158*I)*CA*CF*L - 
  (1.109511831795825151047685137051601846266217506557907016285281465877342924\
87`50.*^-157*I)*CF^2*L + 
  (
    5.881040136947217614415823477078229293033711826303186036581060477871182263`\
50.*^-159*I)*CF*nf + 
  (
    3.57170096041822307727848919839730507337180216430903268278955271031990089`\
50.*^-159*I)*CF*L*nf + 
  (3.535983950814040846505704306413332022638084142665942355961657183216701880\
69`50.*^-157*I)*CA*CF*irrational[Pi^2] - 
  (7.001948417453546230704364963194716876511057708249390803884469669736043328\
1`50.*^-157*I)*CF^2*irrational[Pi^2], 
 3.4567921389394799844151102381204151210786069596464693205932846275269702889`\
50.*^-158*CA*CF - 
  7.3949453816298251359729217683305287638779224367496080925316704464051992132`\
50.*^-158*CF^2 + 
  1.9449856715148739529734347119985324656975160300692752233012415749266787`50.\
*^-160*CA*CF*L + 
  1.100648580886699068301827669952079434800523583156173681916039791461271999`\
50.*^-159*CF^2*L - 
  5.8235193550301629541863469441698634527998174228842859776214852003670259`50.\
*^-161*CF*nf - 
  3.5363375845724980963153358399973317558136655092168640423658937725939612`50.\
*^-161*CF*L*nf - 
  3.536337584572498096315335839997331755813665509216864042365893772593961277`\
50.*^-159*CA*CF*irrational[Pi^2] + 
  7.003335216506319759369586663524127594846670910409868005469711196705688019`\
50.*^-159*CF^2*irrational[Pi^2], 
 (
    3.42313101303659328905131703125670632105055205503543010269848102522222843`\
50.*^-160*I)*CA*CF - 
  (
    7.32031705743597790387886797953290828294645300244530997206551575860936092`\
50.*^-160*I)*CF^2 + 
  (
    1.90684869756360191467983795293973771146815297065615217970709958326145`50.\
*^-162*I)*CA*CF*L + 
  (
    1.0811270406388734943427828881873888951754682200287221983506673576669448`\
50.*^-161*I)*CF^2*L - 
  (
    5.71001250446720560639113509248487138428198433722012213570010388612926`50.\
*^-163*I)*CF*nf - 
  (
    3.46699763193382166305425082352679583903300540119300396310381742411173`50.\
*^-163*I)*CF*L*nf - 
  (
    3.501667608253159879684793331762063797423335455204934002734855598352844`50.\
*^-161*I)*CA*CF*irrational[Pi^2] + 
  (
    6.9353416707149962665601732007714661618869944938039469568729178841163124`\
50.*^-161*I)*CF^2*irrational[Pi^2]}

